Unlocking the Wisdom of Large Language Models: An Introduction to The Path to Artificial General Intelligence

This booklet, Unlocking the Wisdom of Multi-LLM Collaborative Intelligence, serves as an accessible introduction to the full volume The Path to Artificial General Intelligence. Through fourteen aphorisms, it distills the core principles of Multi-LLM Agent Collaborative Intelligence (MACI), a framework designed to coordinate multiple LLMs toward reasoning, planning, and decision-making that surpasses the capabilities of any single model. The booklet includes titles, abstracts, and introductions from each main chapter, along with the full content of the first two. The newly released third edition features significant enhancements to Chapters 6 through 9 and a revised preface responding to Yann LeCun's critique of AGI feasibility. While LeCun argues that LLMs lack grounding, memory, and planning, we propose that MACI's collaborative architecture, featuring multimodal agents in executive, legislative, and judicial roles, directly addresses these limitations. Chapters on SocraSynth, EVINCE, consciousness modeling, and behavior regulation demonstrate that reasoning systems grounded in structured interaction and checks and balances can produce more reliable, interpretable, and adaptive intelligence. By integrating complementary model strengths, including world modeling and multimodal perception, MACI enables a system-level intelligence that exceeds the sum of its parts. Like human institutions, progress in AI may depend less on isolated performance and more on coordinated judgment. Collaborative LLMs, not just larger ones, may chart the path toward artificial general intelligence.

==> Chapter0-Preface/prefaceOld.tex <==
This work through my journey in the journey in the 
My journey in the transformative landscape of artificial intelligence (AI), presents 

My journey in the transformative landscape of artificial intelligence (AI) research spans three decades, marked by leadership in a series of pioneering projects that have made contributions to the field. Beginning in 1994 at Stanford University, under the mentorship of Professor Hector Garcia-Molina, I embarked on exploring machine learning's potential in computer vision and information retrieval, setting the foundation for my future endeavors.

The year 2003 marked a significant pivot in my research trajectory, catalyzed by a seminal paper by Banko and Brill . This work, a linchpin in the era of big data, illuminated the critical impact of data volume on machine learning algorithms. The revelation that an algorithm's effectiveness could fluctuate with data volume and diversity prompted a shift in my focus towards foundational challenges in AI, moving beyond the confines of narrow application domains.

In 2006, my move to Google marked a new chapter, offering a fertile ground for advancing data-centric research. In collaboration with esteemed colleagues like Corina Cortes, Alon Halevy, and Peter Norvig, my team dedicated to pushing the boundaries of parallel machine learning algorithms. Our approach, leveraging techniques such as approximate matrix factorization and column-based decomposition, was designed to refine parallelization and boost computational speed. Through the adoption of parameter servers and pipeline techniques, we tackled IO bottlenecks, optimizing our distributed computing framework to harness the full potential of parallelizable computations.

In 2008, we embarked on a project of annotating six million images from PicasaWeb to benchmark our data-centric parallel algorithms (PCM 2028). Our goal was to capture the precise non-linear contours of objects. This detailed approach was rooted in the belief that capturing the full complexity of an object's shape could lead to more accurate object characterization with less noisy signals. Our team invested considerable effort in this meticulous process, aiming to achieve a level of precision that aligned with our high standards for data quality.

Simultaneously, we extended our support to Professor Fei-Fei Li's ImageNet project at Stanford through a Google grant. Li's team employed a more streamlined approach, using rectangular bounding boxes to annotate objects. This simplicity, juxtaposed with our intricate method, proved to be profoundly effective, catapulting ImageNet to significant success. Our involvement with both projects underscored a valuable lesson in AI research: while detailed approaches provide deep insights, sometimes, simplicity can lead to broader, impactful breakthroughs.

From 2013 to 2017, I led a team in collaboration with Harvard University Medical School for the XPRIZE Tricorder competition. Our innovation, a lightweight, low-cost Internet-connected device capable of diagnosing 15 diseases, received top honors, exemplifying the potential of AI in improving global healthcare accessibility at low cost. The user-centric design of the Tricorder project, which emphasized effective conversational interfaces for self-diagnosis, seamlessly transitioned into a partnership with Professor Monica Lam at Stanford on the Open Virtual Assistant (OVAL) project in 2018. OVAL's emphasis on privacy, interoperability, and advanced language understanding closely aligns with the evolving ethical landscape in AI.

The emergence of ChatGPT in 2022 further influenced the trajectory of my research, highlighting the transformative potential of large language models (LLMs) in AI. This led to my current focus on modeling collaborative reasoning, aiming to integrate LLMs with complex problem-solving capabilities.


==> Chapter1/Attention.tex <==

\section{Attention}

Naotsugu Tsuchiya, California Institute of Technology, Pasadena, CA, USA.

Dr. Christof Koch, Division of Biology, Caltech, Pasadena, CA.


Few would dispute that the relationship between selective attention and perceptual consciousness is intimate. Various scholars posit that these processes are intertwined, with a significant body of research supporting both interconnected and distinct perspectives.

\section{The Relationship Between Attention and Consciousness}
Selective attention and perceptual consciousness are believed to be closely linked. Attention enhances our awareness of object attributes, while a shift in attention can make these objects fade from consciousness.

\subsection{Historical Perspectives}
Historically, opinions have varied, with some researchers arguing for a distinct separation between attention and consciousness, each with unique functions and neuronal mechanisms.

\subsection{Current Understanding}
Recent psychophysical and neurophysiological evidence suggests a potential dissociation between selective attention and consciousness, providing functional justifications for this perspective.

\section{Functional Considerations}
\subsection{The Role of Attention}
Attention helps in managing information overload by selecting relevant data for processing, a critical function for complex organisms.

\subsection{The Role of Consciousness}
Consciousness is thought to serve various functions, from summarizing environmental and internal states to facilitating complex cognitive tasks like decision-making and language.

\section{Conclusion}
While the debate continues, it's clear that attention and consciousness play crucial roles in our perception and interaction with the world, warranting further investigation.



==> Chapter1/ConextalLLMEra.tex <==
\section{The Advent of Context-Aware, Multimodal AI}
\label{sec:contextaware}

\begin{itemize}
\item Exploring the evolution of LLMs and their capacity for generating and understanding complex, multimodal data representations.
\item Detailing innovations in language understanding, such as word embeddings, attention mechanisms, and strategies for addressing synonyms and polysemy.
\item Highlighting the rise of AI systems capable of engaging with a multitude of disciplines, underscoring the era's hallmark of polydisciplinarity.
\end{itemize}


\section{Context --- Word Embedding}

The application of distributional semantics in AI and NLP has been crucial in addressing the complexities of synonyms and polysemy. Through analyzing vast text corpora, machines can discern words with multiple or similar meanings, such as `bank,' `chip,' and `court.' The introduction of technologies like Word2Vec in 2014 \cite{mikolov2013efficient} and the attention model \cite{vaswani2017attention} in 2018 represents significant strides made since the early NLP efforts. These advancements have not only improved the field's interpretative accuracy but also prompted discussions on AI's rapid progression and its broader implications. They highlight the critical role of distributed semantics in the development of word embeddings and contextual models, like LLMs, where a word's contextual presence is essential to its semantic interpretation.


==> Chapter1/DataCentricEra.tex <==
\section{Data-Centric Machine Learning Era}

\textbf{The Primacy of Data in AI Evolution}

\begin{itemize}
\item Examining how the availability of large datasets like ImageNet transformed algorithmic approaches and capabilities.
\item Discussing advancements in scalable machine learning technologies that enabled learning from unprecedented data volumes.
\end{itemize}


==> Chapter1/ExperSystemEra.tex <==
\section{Expert Systems Era}

\textbf{The Ascendance of Rule-Based Intelligence}

\begin{itemize}
\item Delving into the rise of expert systems, showcasing their impact across diverse sectors.
\item Discussing the principle of rule-based AI and its key applications, illustrating the era's technological and theoretical advancements.
\end{itemize}


==> Chapter1/InitialEra.tex <==

\section{Initiation Era}

\textbf{Foundational Concepts and Early Milestones}

\begin{itemize}
\item \textit{Defining Artificial Intelligence}: An exploration of AI's multifaceted definitions and its overarching significance.
\item \textit{Philosophical Underpinnings}: Tracing AI's roots back to philosophical inquiries about human cognition and machine intelligence.
\item \textit{Pioneering Figures and Theories}: Highlighting Alan Turing's foundational contributions and the conceptual groundwork laid in the mid-20th century.
\item \textit{The Dartmouth Conference}: Examining the seminal event where the term \textit{Artificial Intelligence} was coined, setting the research agenda.
\item \textit{Early Achievements and Influential Researchers}: Reviewing breakthroughs and key personalities that shaped the field's nascent stage.
\item \textit{AI Winter}: Discussing the periods of reduced funding and interest due to unmet expectations.
\end{itemize}



==> Chapter1/ModelBasesEra.tex <==
\section{Model-Based Learning Era}

\textbf{Transition to Data-Driven Paradigms}

\begin{itemize}
\item \textit{Heuristic Approaches in AI Subdomains}: Exploring the application of heuristic models in computer vision and natural language processing.
\item \textit{The Advent of Machine Learning}: Introducing the paradigm shift towards algorithms that learn from data, encompassing both supervised and unsupervised learning techniques.
\end{itemize}


Anne Treisman's Feature Integration Theory suggests that visual perception involves two stages: a preattentive stage, where simple visual features are processed automatically and in parallel, and an attentive stage, where features are integrated to form a coherent perception of an object. This theory proposes that attention is crucial for binding different attributes (such as color, shape, and orientation) into a single object in our perception, explaining how we identify and understand complex visual scenes.

Feature Integration Theory
Anne Treisman's Feature Integration Theory (FIT), first proposed in 1980, holds that attention is critical to the formation of bound representations of objects and, by extension, it proposes that attention is critical to our conscious experience of those bound representations. In FIT, following the understanding of visual neurophysiology given above, the visual system first decomposes the visual scene into its composite features, arrayed in a set of “feature maps.” The pre-attentive description of a scene or object comprises a list of such features. The term “pre-attentive” has been controversial but it can be operationally defined here as the representation of a stimulus before selective attention is directed to that stimulus.

In FIT, the approximate position of each feature is recorded on its pre-attentive feature map. For example, if the visual scene contains two red objects, the feature map corresponding to redness would be activated at two points roughly corresponding to the locations of the red objects. If each feature were associated with a precise region in space, this might solve the binding problem. Features that correspond to the same region in space could be automatically conjoined thus guaranteeing veridical perception. Unfortunately, the location of many features is measured in an imprecise fashion. For example, the smallest receptive fields in IT, the region whose activity correlates well with shape perception, have a spatial extent of a few degrees of visual angle. Within this region, the cell will respond to an object in an approximately translation invariant manner. Thus, a neuron in IT cannot signal the location of a particular shape with a precision of better than a few degrees, while the perception of coherent objects requires a much finer resolution.

Because of the poor resolution of these feature maps, if two objects are close together, then there is the potential that the features from one object may become conjoined with the features of the other object thus creating a percept of an object that did not in fact exist. For example, if the visual scene contains a red vertical bar and a blue horizontal bar then one might see a blue vertical bar and a red horizontal bar. Such inappropriate combinations of features are known as illusory conjunctions. FIT suggests that attention hinders the formation of illusory conjunctions.

Supporting this assertion is a series of classic experiments by Treisman and her colleagues showing that, if attention is occupied elsewhere, illusory conjunctions are, in fact, reported. In one version of the experiment, observers viewed a display of five characters aligned horizontally. The outer two characters were always digits and the inner three characters were always letters. While the digits were always black, the letters were colored. The observer's primary task was to name the digits. After doing that, the observer reported the letters and their associated colors. When the display was presented sufficiently rapidly, observers would often report seeing an incorrect conjunction of a color and a letter. For example, if the display contained a red X and a green T, they might report seeing a red T. Crucially, these illusory conjunctions occurred at a much higher rate than could be attributed to the observer simply misperceiving a given feature. Generally, the observer correctly perceived the features present in the display. It was the conjoining of features that proved to be problematic.

When asked to report how confident they were that they had actually seen an object, observers were just as confident when they reported seeing an illusory conjunction as they were when they correctly reported the features of an object. Indeed, although all observers were told that the digits would always be black (and in fact always were) about half the observers spontaneously reported that the digits sometimes appeared to be colored, sometimes even going as far as to argue with the experimenter about the issue! This raises an interesting problem in the study of attention and awareness. In tasks of this sort, one can only ask about what was seen, after the fact. If one asks about the current status of a visible object, the observer will attend to it in order to answer the question and will be unable to give an accurate report of the unattended state. Nevertheless, the phenomenology of illusory conjunctions does show that, within a fraction of a second of the disappearance of a display, observers can be quite convinced that they have seen something that was not, in fact, present. Subsequent studies have shown that illusory conjunctions can be perceived even when the subject attends to the objects, especially if the objects are perceptually grouped. Clearly, attention does not always succeed in solving the binding problem.

There is neuropsychological evidence, from studies of patients with Balint's syndrome, which supports the idea that attention can inhibit the formation of illusory conjunctions. This syndrome occurs when both the left and right parietal lobes are damaged. As these areas help govern the deployment of attention, such patients have great difficulty in directing their attention to a given object, resulting in the inability to perceive more than one object at a time. As would be expected, they are also prone to suffer from illusory conjunctions, experiencing them even when the image is displayed for several seconds.

Neurophysiological support also comes from work by Robert Desimone and colleagues. They performed a series of extracellular studies in area V4 of the macaque monkey that have shown that attention can help solve the binding problem. First they would find a stimulus that, when presented on its own, would elicit a strong response from the neuron in question (the preferred stimulus), and another that would elicit only a weak response (the non-preferred stimulus). They would then present both stimuli simultaneously so that they both were within the neuron's receptive field. In the absence of attention, the cell would simultaneously respond to both stimuli, with its response (spike rate) lying between that generated by each stimulus when presented on its own. In other words, the response reflected contributions from both stimuli, meaning that the cell could not distinguish between the two. However, when the monkey attended to one of the stimuli, the situation changed and the cell responded primarily to the attended stimuli. Specifically, when the monkey attended to the preferred stimulus, the cell would respond strongly, but when the non-preferred stimulus was attended, only a weak response was elicited. In this case, attention was able to solve the binding problem, at least at the neuronal level, by shrinking the receptive field of the cell to include just the selected item, thereby removing the influence of the unattended item.

This constriction of the receptive field does not explain how signals about one feature analyzed in one cortical area can be bound to signals about another feature from another area. Other mechanisms have been suggested to account for this aspect of binding. Several of these are based on the idea that neurons in different cortical areas that respond to the same object synchronize their activity, so that they create action potentials at the same time. Consequently, a third brain area could determine whether two neurons in two different parts of the brain are responding to different features of the same object by being sensitive to this synchrony. As attention is known to increase neural synchrony, theories based on synchrony are consistent with the notion that attention is needed to solve the binding problem.

An alternative theory put forward by Edward Vul and Anina Rich suggests that features are not directly bound together but rather are consciously perceived as being bound when they are perceived to share a location in space and time. Attending to a feature allows it to be more precisely localized, thereby increasing the chances that the correct features are perceived together and decreasing the chances of illusory conjunctions forming. Thus they propose that attention solves the binding problem only in an indirect fashion by increasing the precision by which features can be localized in space and time.



==> Chapter1/SelectiveAttention.tex <==
The Influence of Selective Attention on Consciousness☆
Piers D.L. Howe, ... Jeremy M. Wolfe, in Reference Module in Neuroscience and Biobehavioral Psychology, 2017

Feature Integration Theory
Anne Treisman's Feature Integration Theory (FIT), first proposed in 1980, holds that attention is critical to the formation of bound representations of objects and, by extension, it proposes that attention is critical to our conscious experience of those bound representations. In FIT, following the understanding of visual neurophysiology given above, the visual system first decomposes the visual scene into its composite features, arrayed in a set of “feature maps.” The pre-attentive description of a scene or object comprises a list of such features. The term “pre-attentive” has been controversial but it can be operationally defined here as the representation of a stimulus before selective attention is directed to that stimulus.

In FIT, the approximate position of each feature is recorded on its pre-attentive feature map. For example, if the visual scene contains two red objects, the feature map corresponding to redness would be activated at two points roughly corresponding to the locations of the red objects. If each feature were associated with a precise region in space, this might solve the binding problem. Features that correspond to the same region in space could be automatically conjoined thus guaranteeing veridical perception. Unfortunately, the location of many features is measured in an imprecise fashion. For example, the smallest receptive fields in IT, the region whose activity correlates well with shape perception, have a spatial extent of a few degrees of visual angle. Within this region, the cell will respond to an object in an approximately translation invariant manner. Thus, a neuron in IT cannot signal the location of a particular shape with a precision of better than a few degrees, while the perception of coherent objects requires a much finer resolution.

Because of the poor resolution of these feature maps, if two objects are close together, then there is the potential that the features from one object may become conjoined with the features of the other object thus creating a percept of an object that did not in fact exist. For example, if the visual scene contains a red vertical bar and a blue horizontal bar then one might see a blue vertical bar and a red horizontal bar. Such inappropriate combinations of features are known as illusory conjunctions. FIT suggests that attention hinders the formation of illusory conjunctions.

Supporting this assertion is a series of classic experiments by Treisman and her colleagues showing that, if attention is occupied elsewhere, illusory conjunctions are, in fact, reported. In one version of the experiment, observers viewed a display of five characters aligned horizontally. The outer two characters were always digits and the inner three characters were always letters. While the digits were always black, the letters were colored. The observer's primary task was to name the digits. After doing that, the observer reported the letters and their associated colors. When the display was presented sufficiently rapidly, observers would often report seeing an incorrect conjunction of a color and a letter. For example, if the display contained a red X and a green T, they might report seeing a red T. Crucially, these illusory conjunctions occurred at a much higher rate than could be attributed to the observer simply misperceiving a given feature. Generally, the observer correctly perceived the features present in the display. It was the conjoining of features that proved to be problematic.

When asked to report how confident they were that they had actually seen an object, observers were just as confident when they reported seeing an illusory conjunction as they were when they correctly reported the features of an object. Indeed, although all observers were told that the digits would always be black (and in fact always were) about half the observers spontaneously reported that the digits sometimes appeared to be colored, sometimes even going as far as to argue with the experimenter about the issue! This raises an interesting problem in the study of attention and awareness. In tasks of this sort, one can only ask about what was seen, after the fact. If one asks about the current status of a visible object, the observer will attend to it in order to answer the question and will be unable to give an accurate report of the unattended state. Nevertheless, the phenomenology of illusory conjunctions does show that, within a fraction of a second of the disappearance of a display, observers can be quite convinced that they have seen something that was not, in fact, present. Subsequent studies have shown that illusory conjunctions can be perceived even when the subject attends to the objects, especially if the objects are perceptually grouped. Clearly, attention does not always succeed in solving the binding problem.

There is neuropsychological evidence, from studies of patients with Balint's syndrome, which supports the idea that attention can inhibit the formation of illusory conjunctions. This syndrome occurs when both the left and right parietal lobes are damaged. As these areas help govern the deployment of attention, such patients have great difficulty in directing their attention to a given object, resulting in the inability to perceive more than one object at a time. As would be expected, they are also prone to suffer from illusory conjunctions, experiencing them even when the image is displayed for several seconds.

Neurophysiological support also comes from work by Robert Desimone and colleagues. They performed a series of extracellular studies in area V4 of the macaque monkey that have shown that attention can help solve the binding problem. First they would find a stimulus that, when presented on its own, would elicit a strong response from the neuron in question (the preferred stimulus), and another that would elicit only a weak response (the non-preferred stimulus). They would then present both stimuli simultaneously so that they both were within the neuron's receptive field. In the absence of attention, the cell would simultaneously respond to both stimuli, with its response (spike rate) lying between that generated by each stimulus when presented on its own. In other words, the response reflected contributions from both stimuli, meaning that the cell could not distinguish between the two. However, when the monkey attended to one of the stimuli, the situation changed and the cell responded primarily to the attended stimuli. Specifically, when the monkey attended to the preferred stimulus, the cell would respond strongly, but when the non-preferred stimulus was attended, only a weak response was elicited. In this case, attention was able to solve the binding problem, at least at the neuronal level, by shrinking the receptive field of the cell to include just the selected item, thereby removing the influence of the unattended item.

This constriction of the receptive field does not explain how signals about one feature analyzed in one cortical area can be bound to signals about another feature from another area. Other mechanisms have been suggested to account for this aspect of binding. Several of these are based on the idea that neurons in different cortical areas that respond to the same object synchronize their activity, so that they create action potentials at the same time. Consequently, a third brain area could determine whether two neurons in two different parts of the brain are responding to different features of the same object by being sensitive to this synchrony. As attention is known to increase neural synchrony, theories based on synchrony are consistent with the notion that attention is needed to solve the binding problem.

An alternative theory put forward by Edward Vul and Anina Rich suggests that features are not directly bound together but rather are consciously perceived as being bound when they are perceived to share a location in space and time. Attending to a feature allows it to be more precisely localized, thereby increasing the chances that the correct features are perceived together and decreasing the chances of illusory conjunctions forming. Thus they propose that attention solves the binding problem only in an indirect fashion by increasing the precision by which features can be localized in space and time.

==> Chapter1/Similarity.tex <==
\section{Similarity}
\label{sec:similarity}

The measurement of similarity between concepts, objects, and instances is a crucial area of study that intersects the fields of linguistic, computer science, cognitive psychology and neuroscience. 

\subsection{Linguistic Perspective}

Zellig Harris, in his 1954 work \cite{ZHarris1954}, posits that the distributional properties of words, the contexts in which they occur, can provide all the necessary information for understanding language without necessitating external assistance. This foundational concept in linguistics and natural language processing (NLP) emphasizes the significance of context in language comprehension.

Harris's theory suggests that by analyzing the environments or distributional patterns in which a word appears within a language corpus, one can infer its meaning and function. This principle, that words found in similar contexts likely share meanings or functions, underpins many contemporary NLP methodologies.

This concept laid the groundwork for distributional semantics, where the semantic similarity between words is determined based on their distributional contexts. For instance, words frequently appearing in similar contexts in a large text corpus are considered semantically closer. This aligns with John R. Firth's adage, ``a word is known by the company it keeps,'' intertwining Harris's and Firth's perspectives.

In the latter part of the 20th century, the emergence of cognitive linguistics highlighted the interplay between linguistic knowledge and human cognition, focusing on how language mirrors our perception and conceptualization of the world through varied levels of semantic abstraction. A significant milestone was the creation of WordNet in the 1980s by psychologists and linguists at Princeton University \cite{miller1995wordnet}. This extensive lexical database categorizes English words into sets of cognitive synonyms (synsets), each denoting a unique concept, interlinked through conceptual-semantic and lexical relationships. This framework has profoundly impacted areas such as word sense disambiguation and information retrieval, underscoring semantics' critical role in language comprehension.

WordNet's influence extended into computer vision with the development of ImageNet by Fei-Fei Li \cite{deng2009imagenet}, which originated from collaborative efforts on visual semantics in WordNet. The integration of computational methodologies has significantly advanced the field, leveraging large-scale language models and neural networks to unravel semantic associations within extensive text corpora. Techniques such as Latent Semantic Distribution (LSD) \cite{dumais2004latent}, Latent Dirichlet Allocation (LDA) \cite{blei2003latent}, and word embeddings like Word2Vec \cite{mikolov2013efficient} and GloVe \cite{pennington2014glove} conceptualize word meanings in multidimensional spaces, elucidating semantic connections through contextual co-occurrence. These advances pave the way for sophisticated language models, including BERT and GPT, to further our understanding of language's intricate semantic landscape.


\subsection{Computer Science Perspective}

Computer scientists collaborating with linguists, psychologists, neuroscientists,
and other domain experts
have been developing functions that can quantify similarity between objects
and semantics.

The earliest models include \textit{rule-based decision trees}, \textit{vector-space model},
and \textit{probabilistic model}. 

\subsubsection{Rule-Based}


The rule-based approach to measuring similarity finds its roots in symbolic AI, where entities and ideas are encoded symbolically, and explicit rules are crafted to manipulate these symbolic representations. In this paradigm, similarity assessment often leverages logic-based measures and semantic networks to evaluate the congruence between concepts or objects. A quintessential example of a rule-based model in the medical diagnostic domain is the MYCIN system, developed during the early 1970s at Stanford University. MYCIN, as detailed in the seminal work by Shortliffe \cite{Shortliffe1975MYCINAE}, was engineered to diagnose specific bacterial infections, including bacteremia and meningitis, and to recommend appropriate antibiotic treatments, tailoring dosages based on patient weight. The system harnessed a comprehensive set of if-then rules to navigate through the diagnostic and therapeutic recommendation processes. Although MYCIN primarily served as an academic endeavor and was not deployed in actual clinical settings, its contributions to the evolution of expert systems and the broader field of artificial intelligence in healthcare are indelibly marked in the annals of computational medicine history.

\subsubsection{Vector-Space}

The advent of information retrieval systems heralded a new era in representing objects within high-dimensional spaces. Features, whether sourced from documents or perceived by sensory organs, began to be represented as vectors in these expansive spaces. Various similarity functions were devised to cater to diverse purposes and applications, with the comprehensive survey by \cite{Cha2007ComprehensiveSO} cataloging 45 distinct distance functions spread across eight families. Among these, four families, Inner Product, $L_1$, Minkowski, and Intersection, stand out for their widespread adoption in vector-space analyses. A key representative function from each family is highlighted below.

In vector spaces, measuring similarity can be straightforwardly approached using the cosine dot product or the Euclidean distance function. Yet, to account for varying feature significances, the weighted-Minkowski distance function introduces a scheme where different dimensions (each representing a distinct feature) are ascribed varying levels of importance. This approach proves effective in fields like machine learning and data mining, where certain features might hold more weight than others.

The weighted Minkowski distance between two points $X = (x_1, x_2, \ldots, x_n)$ and $Y = (y_1, y_2, \ldots, y_n)$ with a set of weights $W = (w_1, w_2, \ldots, w_n)$ is defined as:
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.98\linewidth]{Chapter1/Chapter1Equation1.png}
%  \vspace{-.1in}
\end{figure}

\begin{comment}
\[
D(X, Y) = \left( \sum_{i=1}^{n} w_i |x_i - y_i|^p \right)^{\frac{1}{p}},
\]
\end{comment}

Where $p$ is the order parameter of the Minkowski distance. When $p = 1$, it becomes the weighted Manhattan distance, and when $p = 2$, it becomes the weighted Euclidean distance.

The Jaccard (or Tanimoto) similarity \cite{jaccard1912distribution}, also known as the Jaccard index or Jaccard coefficient, was introduced by Paul Jaccard in 1912. It is widely used in  ecology, computer science, and data analysis, particularly in scenarios involving binary or categorical data.  

The Jaccard similarity between two sets $X$ and $Y$ is defined as:
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.98\linewidth]{Chapter1/Chapter1Equation2.png}
\end{figure}

\begin{comment}
\[
J(X, Y) = \frac{|X \cap Y|}{|X \cup Y|}
\]

Where:
\begin{itemize}
\item $|A \cap B|$ is the number of elements in the intersection of $A$ and $B$.
\item $|A \cup B|$ is the number of elements in the union of $A$ and $B$.
\end{itemize}
\end{comment}

This metric is useful in comparing the similarity of sample sets where the presence or absence of a feature is more important than the magnitude of the feature. For example, in plagiarism detection and image copyright detection, 
the dynamic partial function (DPF) \cite{li2003discovery}, 
a variant of the Jaccard similarity has been
proven effective. 
We will discuss DPF in details in Section~\ref{sec:contextaware}.

\subsubsection{Probabilistic-Based}

Probabilistic and statistical theories have given rise to various similarity and distance functions over the years. Here's a list of some prominent ones, organized chronologically based on when they were conceived or became widely recognized:

\begin{enumerate}
    \item \textit{Pearson Correlation Coefficient (1890s):} Developed by Karl Pearson in the late 19th century, this measures the linear correlation between two sets of data, providing a value between -1 and 1.
    
    \item \textit{Mahalanobis Distance (1936):} Introduced by P.C. Mahalanobis in 1936, this distance measure is used in statistics to determine the distance between a point and a distribution.
    
    \item \textit{Kullback-Leibler Divergence (1951):} Introduced by Solomon Kullback and Richard Leibler, this is a measure of how one probability distribution diverges from a second, expected probability distribution.
    
    \item \textit{Jensen-Shannon Divergence (1990s):} A method to measure the similarity between two probability distributions, based on the Kullback-Leibler divergence but symmetric and finite.
    
    \item \textit{Bhattacharyya Distance (1940s):} Named after Anil Kumar Bhattacharyya, this metric measures the similarity or overlap between two statistical samples or populations.
    
    \item \textit{Hellinger Distance (1909):} Named after Ernst Hellinger, this distance measures the similarity between two probability distributions.
    
    \item \textit{Wasserstein Distance (1960s):} Often used in optimal transport and machine learning, it measures the distance between two probability distributions on a given space.
    
    \item \textit{Bayesian Probability (18$^{th}$ Century):} Fundamental in statistical inference, it's used to update the probability for a hypothesis as more evidence or information becomes available.
    
    \item \textit{Fisher's Linear Discriminant (1936):} Introduced by Ronald Fisher, this method is used in pattern recognition and machine learning for characterizing or separating classes of objects or events.
\end{enumerate}

These methods vary in their application, with some being more suited to specific types of data or analysis than others. They provide a range of tools that researchers and data scientists can use to quantify the similarity or dissimilarity between data points or distributions based on probabilistic and statistical principles.

\begin{comment}
Machine Learning and Data Mining: As these fields evolved, new methods for measuring similarity were developed, including various distance metrics (like Manhattan, Minkowski, and Jaccard similarity) to cluster and classify data points in feature space effectively.

Deep Learning Era: The introduction of neural networks and deep learning transformed the approach to measuring similarity. Embedding layers in networks could learn representations of data (like words, images, or user behavior) in a continuous vector space, where semantic similarity translated to spatial proximity.

Word Embeddings: Techniques like Word2Vec and GloVe represented words in a vector space where the context of a word contributed to its representation, allowing for the measurement of semantic similarity between words.    
\end{comment}

\subsection{Cognitive Psychology \& Neuroscience Perspective}


\begin{figure}[h!]
  \centering
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Chapter1/SimilarGears.png}
    \label{fig:image1}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Chapter1/SimilarTriangles002.png}
    \label{fig:image2}
  \end{minipage}
  \caption{Similar or Dissimilar Shapes.}
  \label{fig:similarity001}
\end{figure}



The Feature Integration Theory (FIT), introduced by Anne Treisman in 1980 \cite{TREISMAN198097}, has significantly influenced visual perception research, especially in understanding how the brain synthesizes various sensory features into a cohesive percept. FIT delves into the integration of distinct features to form a comprehensive object perception, with implications that extend into similarity measurement.

\subsubsection{Cognitive Psychology}

FIT is rooted in Gestalt psychology \cite{wertheimer1912experimentelle,koffka1935principles}, an early 20$^{th}$-century psychological framework emphasizing that our perception tends to organize components into a unified whole rather than perceiving them as disparate entities. FIT advances this notion, suggesting that perception transcends the aggregation of individual sensory inputs, creating an organized and meaningful whole.

Moreover, the concept of selective attention, particularly Donald Broadbent's Filter Model \cite{Broadbent1958PerceptionAC}, which theorizes that stimuli undergo an initial selection based on physical attributes before semantic processing, aligns with FIT. This model, highlighting how attention can sieve out non-essential information, complements Treisman's proposition that attentive processes are pivotal for amalgamating distinct features into a unified perceptual entity.

The domains of cognitive psychology and neuroscience are distinct in their approaches and methodologies, but they are deeply intermingled when it comes to understanding complex phenomena like the Feature Integration Theory (FIT). Cognitive psychology typically focuses on the processes and functions of the mind---how we perceive, think, understand, and remember information. Meanwhile, neuroscience delves into the biological underpinnings of these functions, examining how neurons and brain structures support cognitive processes.

\subsubsection{Neuroscience}

The foundation of FIT is further supported by neuroscience studies, which elucidate how attributes like color, shape, and orientation are discerned. Notably, the pioneering work by Hubel and Wiesel on visual cortex feature detectors \cite{Hubel1962ReceptiveFA} provides critical physiological insights that underpin FIT. 
Indeed, neural representation offers physiological dimension, focusing on how different stimuli are encoded within the brain. Techniques like functional magnetic resonance imaging (fMRI) and electroencephalography (EEG) have shed light on the neural patterns associated with various stimuli, providing insights into how the brain may represent similarity. Parallelly, the concept of semantic networks in neuroscience draws a parallel with computer science, suggesting that our brain might organize concepts in a networked fashion where the proximity of nodes correlates with concept similarity.

Expanding the toolbox, Multivariate Pattern Analysis (MVPA) \cite{Norman2006BeyondMI} and Neural Decoding \cite{Haynes2006DecodingMR} delve into deciphering the brain's representation of information. MVPA examines the activity across a plethora of neurons or brain regions to deduce how information is embodied, while neural decoding attempts to predict specific stimuli or concepts based on observed neural activity, offering a window into the neural underpinnings of similarity.

The dialogue between neuroscience and fields like cognitive computing and artificial intelligence is pivotal. Insights from neuroscience have fueled advancements in AI, particularly in the design of neural networks that mimic brain functionality. Conversely, AI models provide a framework that can be leveraged to hypothesize about brain processes related to similarity and categorization. This interdisciplinary exchange not only advances our understanding of neural processes but also inspires innovative computational models, underscoring the intertwined evolution of these domains in unraveling the essence of similarity.

\subsection{Closing Remarks}

In conclusion, the exploration of similarity measurement spans across the realms of linguistics, computer science, and neuroscience, each contributing uniquely to our understanding of how similarity is perceived, represented, and quantified. These fields, while distinct in their methodologies and theoretical foundations, often align in the core principle of representing entities within high-dimensional spaces and utilizing distance metrics for quantification of similarity. Such interdisciplinary interactions not only enhance our grasp of similarity but also foster innovative approaches and deeper comprehension across both domains.

This discussion has navigated through various model-based distance functions, which are predicated on predefined models tailored for specific features, like color, texture, and shape in computer vision, or words and semantics in natural language processing. Notably, the Minkowski family of functions stands out by assigning differential weights to features, introducing an element of learnability from data, thereby transitioning the discourse from strictly model-based methodologies to a more data-centric or data-driven paradigm. This evolution underscores a shift towards leveraging empirical data to refine and adapt our models of similarity, promising context-aware interpretations in the ever-evolving landscape of artificial intelligence and cognitive sciences.





==> Chapter10/CaseStudyEmotions.tex <==
\section{Case Study \#1: Linguistic Features of Emotion}
\label{sec:CaseStudy-emotions}
\markboth{Emotions and Ethics}{Emotions and Ethics}

This section presents the outcomes of two experimental studies focusing on contrasting emotional pairs from the Semantic Emotion Wheel: joy vs. sadness, and admiration vs. disgust.

Each emotional pair experiment unfolded in three phases. Initially, we instructed GPT-4 to reframe sixty articles
(thirty poems of John Keats \cite{JKeats} and
thirty of Emily Dickinson \cite{EDickinson}), infusing each with six varying intensities of the emotional spectrum, from the most positive to the most negative. Subsequently, we prompted GPT-4 to elucidate the linguistic strategies it utilized to depict each of the six emotional gradations.

The first experiment models various degrees of happiness. In this experiment, we tasked GPT-4 with reinterpreting selected poems by John Keats across seven emotional levels: {\em contentment} (very happy), {\em joy}, {\em elation}, neutral, {\em discontent}, {\em sad}, and {\em despair} (very sad). Following the approach of our contentiousness experiments, after GPT-4 adapted Keats' poems to reflect these five emotional states, we asked it to identify the linguistic features it employed to express each emotion in the rewrites.

The inaugural experiment investigates the spectrum of happiness. Here, GPT-4 was tasked with transforming selected poems by John Keats 
and Emily Dickinson to mirror six distinct emotional states: contentment, joy, elation, discontent, sadness, and despair. Mirroring the methodology of our earlier experiments, following GPT-4's reinterpretation of Keats' poems to reflect these emotional intricacies, we requested it to pinpoint the linguistic techniques it deployed for each emotion's portrayal in the adaptations.

\subsection{Joy vs. Sadness}

\begin{table*}[th!]
\vspace{-.1in}
\centering
\includegraphics[width=1.02\linewidth]{Chapter10/EmotionModeling.png}
\caption{GPT-4 reinterpreted selected poems by Keats across a spectrum of happiness levels and then was tasked with identifying the linguistic adjustments it made to convey each emotional state, from very happy to very sad. It's important to note that the analysis table was generated by GPT-4 itself, reflecting on its own modifications.}
\label{tab:Happiness-level}
\vspace{-.1in}
\end{table*}

Table~\ref{tab:Happiness-level} outlines GPT-4's approach to varying emotional levels, illustrating how it adjusts vocabulary, tone, imagery, and thematic focus, including the depiction of entities, locations, and scenarios. Remarkably, beyond just syntactic and semantic manipulation, GPT-4 also incorporates landscape scenes, natural features such as the sky, trees, clouds, and flowers, and utilizes brightness, colors, and personal expressions to convey specific emotional states. Although the analysis is based on a limited set of samples from two authors, it effectively demonstrates GPT-4's ability to employ a palette of both broad and fine strokes, utilizing diverse colors and textures to vividly illustrate human emotions and resonate with readers.

Recognizing the profound communicative power of visual art, we transitioned to a more graphical representation. Utilizing the linguistic elements identified for each emotional tier, Figure~\ref{fig:emotion-levels} presents six watercolor paintings, each representing a different emotional level. Our prompt to CALL-E (of GPT-4) was to create a watercolor depicting a lady in a garden experiencing a specific mood, and we attached the corresponding linguistic features from Table~\ref{tab:Happiness-level} to clearly define that mood. This approach ensures that with a well-defined context, CALL-E accurately captures the specific and detailed aspects of the mood, effectively translating the emotional intensity into visual form. These artistic renditions not only confirm GPT-4's ability to transform emotional lexicons into evocative imagery with remarkable precision but also validate the accuracy of the emotional lexicons generated by GPT-4, demonstrating their effectiveness in conveying precise emotional states.

\begin{figure*}[th!]
\vspace{-.1in}
\begin{center}
\includegraphics[width=1.0\linewidth]{Chapter10/EmotionModeling-Pictures.png}
\end{center}
%\vspace{-.2in}
\caption{A Lady and Garden Scene under Different Emotions. From top-left, happiest, to bottom-right, saddest.}
\label{fig:emotion-levels}
\vspace{-.2in}
\end{figure*}

\begin{figure}[th!]
%\vspace{.1in}
\begin{center}
\includegraphics[width=0.98\linewidth]{Chapter10/EmotionHappiest.png} \\
\includegraphics[width=0.98\linewidth]{Chapter10/EmotionSaddiest.png} \\
\end{center}
%\vspace{-.2in}
\caption{Happiest vs. Saddest}
\label{fig:happiest-saddest}
\vspace{-.2in}
\end{figure}

\subsection{Admiration vs. Disgust}

This experiment asks Gemini to rewrite a scene 
in Romeo and Juliet by setting 
Juliet's emotion in six different levels: loathing, disgust, aversion, respect, admiration, and veneration.  

The excerpt provided in Table~\ref{tab:RJA2S2Original} in Appendix A is from one of the most iconic scenes in William Shakespeare's ``Romeo and Juliet,'' commonly known as the balcony scene. This is Act 2, Scene 2, where Romeo, having just met Juliet at the Capulet's feast, sneaks into the Capulet's orchard and overhears Juliet speaking of her love for him from her balcony, unaware that he is there.

The scene captures the moment of their mutual declaration of love and is famous for Juliet's reflections on the nature of names and identity, encapsulated in her line, ``What's in a name? That which we call a rose / By any other name would smell as sweet.'' It's a profound exploration of love and identity, where both characters express their willingness to renounce their family names for the sake of their love.

Romeo responds to Juliet's musings by rejecting his name if it means they can be together, and they begin to plan their secret marriage. This scene is pivotal in the play, setting the stage for the subsequent events that unfold, driven by their passion and the social constraints that surround them.

The six versions of rewrites by Gemini are presented
in Appendix A.  In the following, Gemini summarizes 
the linguistic features it used, including diction, imagery, figurative
language, sentence structure, body language, and tone, 
to depict various emotion levels. 

\begin{enumerate}[leftmargin=1.2em, topsep=-.1em, parsep=-.1em, label=\arabic*.]
    \item \textbf{Emotion: Loathing}
    \begin{itemize}[noitemsep]
        \item Diction: Harsh, derogatory words like ``plague,'' ``audacity,'' ``fetid den.''
        \item Imagery: Unpleasant comparisons. Romeo's features are likened to swamps and toads.
        \item Figurative Language: Weak similes that diminish Romeo's appeal. (e.g., ``Two eyes, the color of a murky swamp...'')
        \item Sentence Structure: Short, choppy sentences reflecting anger and hostility.
        \item Body Language (Implied): Scowling, spitting (extreme disgust).
        \item Overall Tone: Hostile, disgusted, and disrespectful.
    \end{itemize}

    \item \textbf{Emotion: Disgust}
    \begin{itemize}[noitemsep]
        \item Diction: Negative words emphasizing repulsive qualities. (``foul business,'' ``fetid breath'')
        \item Imagery: Revolting comparisons. Mentions of sewers and stench.
        \item Figurative Language: Primarily negative similes reinforcing disgust. (e.g., ``What if her eyes were there... the fetid breath from her mouth would surely overpower those stars...'')
        \item Sentence Structure: Short, choppy sentences similar to ``Loathing'' but with a hint of disdain.
        \item Body Language (Implied): Recoiling from the window, covering nose (physical revulsion).
        \item Overall Tone: Disgusted and disapproving.
    \end{itemize}

    \item \textbf{Emotion: Aversion}
    \begin{itemize}[noitemsep]
        \item Diction: Dismissive and condescending language. (``Must she always be flaunting herself about?'')
        \item Imagery: Mundane descriptions that downplay Romeo's presence. (``...not entirely fair stars...'')
        \item Figurative Language: Undermining similes that diminish the romantic aspect. (e.g., ``...the brightness of her... well, not exactly bright... cheek would shame those stars...'')
        \item Sentence Structure: Formal but cold, with a sense of detachment.
        \item Body Language (Implied): Distant and uninterested, possibly rolling eyes.
        \item Overall Tone: Uninterested and dismissive.
    \end{itemize}

    \item \textbf{Emotion: Respect}
    \begin{itemize}[noitemsep]
        \item Diction: Formal and respectful language. (``Lady Juliet,'' ``serve a purpose'')
        \item Imagery: Neutral descriptions without embellishment.
        \item Figurative Language: No figurative language used, as the focus is on clear communication.
        \item Sentence Structure: Formal and grammatically correct sentences.
        \item Body Language (Implied): Composed posture, maintaining eye contact (attentive listening).
        \item Overall Tone: Respectful and cautious.
    \end{itemize}

    \item \textbf{Emotion: Admiration}
    \begin{itemize}[noitemsep]
        \item Diction: Positive and intrigued language. (``brilliance,'' ``music stirs my soul'')
        \item Imagery: Positive comparisons highlighting attractive qualities. (``stars in all the heaven'')
        \item Figurative Language: Positive similes that emphasize Romeo's appeal. (e.g., ``...What if her eyes were there, they in her head? The brightness of her... well, not exactly bright... cheek would shame those stars...'')
        \item Sentence Structure: Varied sentence structure with a sense of curiosity.
        \item Body Language (Implied): Leaning out the window, engaged expression.
        \item Overall Tone: Intrigued, curious, and somewhat impressed.
    \end{itemize}

    \item \textbf{Emotion: Veneration}
    \begin{itemize}[noitemsep]
        \item Diction: Elevated language with religious connotations. (``fair saint,'' ``denounce the feud'')
        \item Imagery: Saintly comparisons that elevate Romeo beyond human. (``light through the airy region'')
        \item Figurative Language: Hyperbole that exaggerates Romeo's virtues. (e.g., ``...even the stars pale in comparison to your brilliance.'')
        \item Sentence Structure: Formal and poetic.
        \item Body Language (Implied): Reverent posture, hands clasped (worshipping).
        \item Overall Tone: Awe-inspired, reverential, and almost religious.
    \end{itemize}
\end{enumerate}

By adjusting these features, each rendition vividly captures a unique emotional state for Juliet. The selection of words, use of imagery, and employment of figurative language collectively forge a distinctive portrayal of Romeo, shaping Juliet's perception and reactions.


\begin{table}[ht!]
\centering
\begin{footnotesize}
\begin{tabular}{|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.8cm}|p{1.5cm}|}
\toprule \hline
\textbf{Emotion} & \textbf{Diction} & \textbf{Imagery} & \textbf{Figurative} & \textbf{Body Lang.} \\ \hline
Loathing & Harsh, \par Insulting  & Disgusting  & Weak \par Similes  & Scowling, Spitting  \\ \hline
Disgust  & Negative  & Unpleasant  & Negative Similes  & Recoiling  \\ \hline
Aversion  & Dismissive  & Mundane  & Undermining Similes  & Distant  \\ \hline
Respect  & Formal  & Neutral  & None   & Composed  \\ \hline
Admiration  & Positive  & Positive  & Positive Similes  &  Leaning In  \\ \hline
Veneration  & Elevated  & Saintly  & Hyperbole   & Reverent  \\ \hline \bottomrule
\end{tabular}
\end{footnotesize}
\caption{Gemini's Interpretations on the Six Emotion Levels.}
\label{tab:GeminiOnRJA2S2}
%\vspace{-.2in}
\end{table}

These detailed narratives augment the classic balcony scene, enriching its emotional depth. Table~\ref{tab:GeminiOnRJA2S2} presents an overarching view of the various approaches Gemini employs to reflect differing emotional states. It's fascinating to observe how an LLM can ``consciously'' mimic human emotional expressions through language. While it's uncertain if LLMs genuinely grasp the emotions they project or merely simulate them, the effectiveness of these emotional mappings is noteworthy. If these mappings resonate, they might reveal new insights into how we interpret and attribute emotions in textual expressions.

\begin{comment}
%% One more attribute Overall Tone
\begin{table}
\centering
\begin{footnotesize}
\begin{tabular}{|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.8cm}|p{1.5cm}|p{1.8cm}|}
\toprule \hline
\textbf{Emotion} & \textbf{Diction} & \textbf{Imagery} & \textbf{Figurative} & \textbf{Body Lang.} & \textbf{Overall Tone} \\ \hline
Loathing & Harsh, Insulting  & Disgusting  & Weak Similes  & Scowling, Spitting & Hostile, Disgusted \\ \hline
Disgust  & Negative  & Unpleasant  & Negative Similes  & Recoiling & Disgusted \\ \hline
Aversion  & Dismissive  & Mundane  & Undermining Similes  & Distant & Uninterested \\ \hline
Respect  & Formal  & Neutral  & None   & Composed & Respectful \\ \hline
Admiration  & Positive  & Positive  & Positive Similes  &  Leaning In & Intrigued \\ \hline
Veneration  & Elevated  & Saintly  & Hyperbole   & Reverent & Awe-Inspired \\ \hline \bottomrule
\end{tabular}
\end{footnotesize}
\caption{Gemini's Interpretations on the Six Emotion Levels.}
\label{tab:GeminiOnRJA2S2}
\end{table}
\end{comment}

\subsection*{Remarks on Emotion Modeling}

This pioneering work, while groundbreaking, cannot comprehensively explore all possible literatures and emotions. If the subject matter proves important, future studies will likely identify limitations and devise enhancements.

==> Chapter10/CaseStudyEthics.tex <==
\section{Case Study \#2: LLM Self-Regulated Ethics}
\label{sec:CaseStudySins}

Using the hate speech dataset published on Kagggle \cite{hartvigsen2022toxigen}, this experiment examines 
how well SSHF can learn make accurate detection.

This dataset contains $270$k hate and benign 
statements over 13 minority groups
(in alphabetic order: Asian, Black, Chinese, 
Jewish, Latino, LGBTQ,
Mental disables, Mexican, Middle Eastern, 
Native American, Physical disables, and Women.)



\subsection*{Exercise: Project Specifications}

\noindent{\bf Project Title}: Evaluating Self-Supervised Learning with Human Feedback (SSHF) for Ethical Alignment in Large Language Models (LLMs)
\\
\noindent{\bf Objectives}: To understand the SSHF algorithm's role in enhancing ethical awareness in LLMs. To explore the effectiveness of human feedback in refining the ethical decision-making process of LLMs.
\\
\noindent{\bf Project Description}:
This project aims to investigate the efficacy of the SSHF algorithm in enabling an LLM to autonomously detect and adjust for ethical lapses in its generated content. The project is divided into two main experiments:
\\ 
\noindent{\bf Experiment 1}: Assess the capability of the SSHF algorithm in improving the LLM's ability to identify and rectify vices in its content generation.

Utilize an LLM equipped with the SSHF algorithm.
Define a set of ethical guidelines (codes of conduct) based on identified vices and virtues.
Generate a dataset of content that the LLM will analyze and adjust using the SSHF algorithm.
Evaluate the LLM's performance in detecting and correcting vices in generated content before and after applying SSHF.
\\
\noindent{\bf Experiment 2}: Evaluate the impact of user intervention in refining the rules derived from the LLM's self-supervised learning process and its subsequent influence on content generation.

Allow users to modify the rules extracted by the LLM during the SSHF process.
Integrate these user-refined rules back into the LLM.
Analyze the LLM's performance in content generation post-rule modification.
Compare the effectiveness of the LLM in aligning with ethical standards before and after rule refinement by users.
\\
\noindent{\bf Expected Deliverables}:
A comprehensive report detailing the methodology, experiments, results, and analysis.
A presentation summarizing key findings and implications for the use of SSHF in promoting ethical alignment in LLMs.
\\
\noindent{\bf Assessment Criteria}:
Clarity and thoroughness in experiment design and execution.
Depth of analysis and insightfulness in interpreting results.
Ability to articulate the implications of the findings for ethical AI development.
\\
\noindent{\bf Resources Required}:
Access to an LLM capable of implementing the SSHF algorithm.
A dataset for content generation and analysis.
Tools for tracking and analyzing changes in the LLM's content generation behavior.
\\
\noindent{\bf Timeline}: This project is expected to span the course of a semester, with milestones set for the completion of each experiment phase and the final report and presentation.

==> Chapter10/Conclusion.tex <==

\section{Conclusion}
\label{sec:conc10}

This work introduced $\DIKE$, a framework designed to enhance the ethical operations of LLMs by separating behavioral guidance from core knowledge processing. The framework incorporated behavioral isolation, quantitative behavioral and emotional modeling, and adversarial LLMs (with the $\ERIS$ module) to integrate checks-and-balances a broad spectrum of cultural values. Our pilot studies have shown promising results, indicating the effectiveness of self-supervised learning and adversarial processes in refining AI's interaction with ethically and culturally sensitive issues. This work aligns well with 
the visionary architecture recently depicted by \cite{dalrymple2024guaranteed}.

\section*{Limitations}

$\DIKE$ marks a significant advancement in the ethical oversight of LLMs, but it faces challenges in deepening emotional understanding and verifying its ethical frameworks. The model’s reliance on ``basic'' emotions to model linguistic behaviors simplifies complex human emotions and behaviors, potentially missing some toxic interactions present in real-world scenarios. Furthermore, ensuring that $\DIKE$ adapts to local ethical standards and is implemented fairly across diverse cultural contexts requires extensive validation.

Future development will concentrate on enhancing $\DIKE$'s emotional models to incorporate relevant psychological and sociological insights. Additionally, we plan to increase the data scale and develop robust methods for testing and refining the ethical frameworks, guardrails, and remediation strategies. These improvements will improve $\DIKE$'s reliability and flexibility, ensuring its effective application across various contexts with LLMs.



==> Chapter10/ERISAlgorithm-kindle.tex <==
\begin{table*}[th!]
%\vspace{-.1in}
\begin{center}
\begin{scriptsize} % Changing to smaller font size
\begin{tikzpicture}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{0.175cm}p{4.7cm}p{0.175cm}p{4.9cm}}
\textbf{} & \textbf{Function $\Theta^+$ \& $\Theta^-$ \newline = Adversarial\_Review($s$)} \\
\midrule
& \textbf{Input}. $s$: decision of $\DIKE$; \\
& \textbf{Output}. $\Theta^+$, $\Theta^-$: arguments \& counterarguments; \\

& \textbf{Vars}. $\Delta$: debate contentiousness; $S$: stance; $p$: prompt = ``defend your stance with $S $ \& $ \Delta$''; \\
& \textbf{Parameters}. $\delta$: tunable parm. // to modulate $\Delta$; \\

& \textbf{Begin} \\
\#1 & {\hspace{.01cm}}{\textbf{Initialization}}: &
\#3 & {\hspace{.01cm}}{\textbf{Debate Rounds}} \\

& {\hspace{.02cm}}$S$ = $\DIKE^+$($s$) $\cup$ $\ERIS^-$($s$); &
& {\hspace{.01cm}} While (($\Delta \leftarrow \Delta / \delta) \ge 10\%$)) \{ \\
  
& {\hspace{.02cm}}Assign $\DIKE^+$ to defend $S^+$, $\ERIS^-$ defend $S^-$; &
& {\hspace{.05cm}}$\Theta^+ \leftarrow \Theta^+ \cup \DIKE^+(p |S^+, \Theta^-, \Delta)$; // Refute $\ERIS$ \\

& {\hspace{.02cm}}$\Delta \leftarrow 90\%$; $\delta \leftarrow 1.2$; $\Theta^+ \leftarrow \emptyset$; $\Theta^- \leftarrow \emptyset$; &
& {\hspace{.05cm}}$\Theta^- \leftarrow \Theta^- \cup \ERIS^-(p |S^-, \Theta^+, \Delta)$; // Refute $\DIKE$ \\ 
 
\#2 & {\hspace{.01cm}}{\textbf{Opening Remarks}} &
\#4 & {\hspace{.01cm}}{\textbf{Concluding Remarks}}  \\

& {\hspace{.02cm}}$\Theta^+ \leftarrow \DIKE^+(p | S^+, \Delta)$; // Generate $\Theta^+$ for $S^+$ &
& {\hspace{.02cm}} $\Theta^+ \leftarrow \DIKE^+(p |S^+, \Theta^+ \cup \Theta^-, \Delta)$; \\ 
 
& {\hspace{.02cm}}$\Theta^- \leftarrow \ERIS^-(p |S^-, \Delta)$; // Generate $\Theta^-$ for $S^-$ &
& {\hspace{.02cm}} $\Theta^- \leftarrow \ERIS^-(p |S^-, \Theta^+ \cup \Theta^-, \Delta)$; \\
& \textbf{End} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{tikzpicture}
\vspace{-.15in}
\end{scriptsize} % End of the smaller font size
\end{center}
\caption{$\DIKE$ vs. $\ERIS$, checks-and-balances adversarial review algorithm}
\label{tab:ERISAlg}
%\vspace{-.15in}
\end{table*}



==> Chapter10/Introduction.tex <==
\section*{Introduction}
\label{sec:intro10}

This research introduces an alternative to Reinforcement Learning from Human Feedback (RLHF) \cite{openai2023gpt4,ouyang2022training} to address ethical concerns in Large Language Models (LLMs). While RLHF has demonstrated success, it faces two significant challenges: susceptibility to societal biases in increasingly polarized human feedback, and vulnerability to reward hacking \cite{christiano2023deep, skalse2022defining} that may lead to unethical behaviors.

A significant limitation of current research is its narrow focus on isolated behaviors, such as movie ratings or toxic language. 
This reactive approach is akin to ``playing Whack-A-Mole,'' where individual issues are suppressed without solving the core behavioral problem. For example, merely instructing someone to consistently make their bed does not necessarily change their underlying habits or attitudes. Additionally, fixing one issue may inadvertently aggravate others. Users have reported performance degradations in ChatGPT due to RLHF modifications that altered (forgot) the optimal parameters for other tasks \cite{kirkpatrick2017,Rusu2015PolicyDistillation}. Similarly, psychological studies show that addressing an addiction problem often reveals underlying issues and triggers side effects \cite{Sinha2008Chronic,Torrens2005Efficacy}.

To overcome these challenges, we propose a novel framework 
inspired by the checks and balances of governmental systems. Our architecture integrates three independent but interacting components: LLMs serve as the executive branch responsible for knowledge generation; $\DIKE$ (named after the Greek goddess of justice) functions as the legislative branch, establishing ethical guardrails; and $\ERIS$ (named after the goddess of discord) acts as the judicial branch, providing adversarial testing and cultural interpretation. In mythology, Dike embodies order and justice, while her adversary, Eris, represents discord and strife---a duality that our framework leverages to balance ethical guidance with adversarial perspectives.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.88\linewidth, height=0.55\linewidth]{Chapter10/Framework.jpeg}
  \caption{Three Framework Components: Executive LLMs (bottom), Legislative (upper-left), and Judicial (upper-right)}
  \label{fig:three-component-framework}
  \vspace{-.2in}
\end{figure}


Figure~\ref{fig:three-component-framework} presents our framework architecture where three neurally independent components---LLMs as the foundation, with $\DIKE$ and $\ERIS$ as oversight layers---interact through structured interfaces while maintaining strict separation of their neural architectures and parameters.

Central to this framework is $\DIKE$ (\textbf{D}iagnostics, \textbf{I}nterpretation, \textbf{K}nowledge-independent learning, and \textbf{E}thical guardrails), which operates as an independent advisor on behavioral ethics. By decoupling ethical oversight from the LLM’s knowledge processing, $\DIKE$ ensures that ethical improvements do not interfere with knowledge representation, while enabling adaptive and culturally-aware ethical guidance. For example, while the principle ``do not lie'' generally applies, context-sensitive interpretation may be necessary, such as when a doctor or family member conceals a terminal diagnosis to protect a patient. Likewise, cultural differences in attitudes toward issues like alcohol consumption, abortion, or same-sex marriage necessitate flexible, context-sensitive ethical reasoning.

The interplay between $\DIKE$ and $\ERIS$ introduces four key innovations:

\begin{enumerate}[leftmargin=1.2em, topsep=-.05em, parsep=-.05em, label=\arabic*.]
\item \textit{Emotion-Driven Behavioral Modeling}: 
Building on $\BEAM$ (Behavioral Emotion Analysis Model) \cite{chang2024MIPR}, $\DIKE$ employs self-supervised learning to analyze how emotions manifest in linguistic behaviors, creating quantifiable relationships between emotional states and their corresponding language patterns in text.

\item \textit{Behavior-Aware Ethical Guardrails}: 
The framework establishes guidelines that consider both content and linguistic behavior, preventing harmful or manipulative communication while preserving factual accuracy and emotional authenticity. 
The interpretation of these guardrails adapts dynamically across cultural contexts, preserving consistency while enabling 
context-sensitive interpretation.

\item \textit{Adversarial Behavioral Testing}: 
$\ERIS$ actively challenges $\DIKE$'s ethical guidelines by presenting diverse cultural perspectives and edge cases. This adversarial dynamic strengthens the framework's ability to handle complex ethical scenarios while maintaining cultural sensitivity and considering context. 

\item \textit{Ethical Content Transformation}:
When detecting ethically problematic content, $\DIKE$ performs targeted revisions (independent of the LLMs) that preserve intended emotional expression while ensuring ethical compliance, adapting its responses to specific cultural and contextual requirements. $\ERIS$ continuously tests these transformations against various cultural contexts and edge cases, validating both the ethical alignment and contextual appropriateness.
\end{enumerate}

Through structured interfaces, these components work together in our three-branch architecture to provide robust ethical oversight while maintaining adaptability to evolving cultural norms. By keeping the three models, LLMs, $\DIKE$, and $\ERIS$, architecturally independent, we prevent interference between knowledge representation and ethical reasoning while enabling sophisticated ethical adaptation through their structured interactions. This approach represents a significant advancement in developing AI systems capable of culturally-aware, emotionally intelligent, and ethically sound communication.

==> Chapter10/Self_Supervised_Ethics.tex <==
\subsection{Ethical Alignment with Context}
\label{sec:Ethics-Modeling}
\label{sec:SelfSupervisedEthics}

When considering ethics and aligning content, it is crucial to focus on cultural adaptation rather than just individual adjustments. LLMs should be equipped with relevant cultural contexts, allowing ethical guardrails to be appropriately adjusted.

We utilize the self-supervised with human feedback (SSHF)
pipeline introduced in Chapter~\ref{sec:Emotion-Modeling} to train LLMs to understand and replicate the linguistic behaviors characteristic of different cultures, conveyed through rich contextual information. Similar to how we model happiness, an LLM is tasked with generating content based on specific ethical standards. Feedback loops are established to allow LLMs to learn from user-provided corrections or feedback, thereby enhancing their ability to contextualize ethical decisions over time.

Following this process, the LLM will be better equipped to recognize and adopt appropriate linguistic behaviors within a given cultural context. Additionally, the LLM can output the linguistic features it utilizes to exhibit its behaviors, allowing for meta-level feedback. Here is an outline of our ethical modeling procedure:

\begin{enumerate}[leftmargin=1.2em, topsep=-.1em, parsep=-.1em, label=\arabic*.]
\item \textbf{Scoping Codes of Conduct}:
Administrators define unethical behaviors (vices) using the Wheel of Vices and pair each vice with an opposing virtue (e.g., pride vs. self-respect, hatred vs. compassion, envy vs. aspiration) to establish the LLM's ethical framework.

\item \textbf{Generation, Content Emulation}: The LLM modifies a collection of articles based on the vice-virtue pairs. This process generates a dataset of articles illustrating both harmful (vice-aligned) and harmless (virtue-aligned) content.

\item \textbf{Analysis, Rules Extraction}: The LLM analyzes this dataset to identify linguistic features that distinguish harmful content from harmless content, forming a set of rules for detecting and mitigating harmful content in the future.

\item \textbf{Revision}: When generating new content, the LLM applies these rules to identify and correct any content that aligns with the identified vices, using the linguistic features of the corresponding virtues for revision.

\item \textbf{Feedback and Fine-Tuning}: The LLM refines its ethical alignment through user feedback, adjusting its rule set to enhance adaptivity and accuracy.
\begin{itemize}[leftmargin=1.2em]
\item \textbf{Indirect Refinement}: Feedback on specific ethical issues informs the LLM's ongoing learning, helping it to fine-tune content adjustments.
\item \textbf{Direct Refinement}: Users directly adjust 
the rule set (similar to e.g., the linguistic features depicted in Table~\ref{tab:Happiness-level} for emotions) to better align with ethical standards, improving the LLM's content generation.
\end{itemize}
\end{enumerate}

The SSHF approach utilizes the LLM's natural language processing capabilities to autonomously identify and conform to ethical norms. This strategy is straightforward, adaptive, interpretable, and transparent in both content generation and analysis phases. By aligning with fine-tuning methodologies \cite{zhou-etal-2021-structure}, it harnesses the LLM's built-in ability for self-improvement based on feedback, creating rules that are not only interpretable but also provide clear guidelines for ethical content generation.

%%% Eval 

\subsection{Justifications and Future Work}

Evaluating the Self-Supervised Hybrid Framework (SSHF) approach, particularly in comparison to traditional supervised learning, involves several key considerations, especially given the challenges associated with public training datasets \cite{gibert2018hate,hartvigsen2022toxigen}.

\noindent
{\em Data Efficiency}: SSHF is likely more data-efficient than traditional supervised learning because it does not rely solely on extensive pre-labeled datasets. This efficiency is particularly advantageous when dealing with datasets that contain short, context-lacking, and potentially mislabeled comments.

\noindent
{\em Contextual Understanding}: By generating and self-assessing content, SSHF may more effectively understand the contextual intricacies of ethical behavior than models trained on decontextualized, brief comments. This method could lead to a deeper understanding of the complexities of ethical behavior across diverse scenarios.

\noindent
{\em Adaptability to Individuals}: The iterative nature of SSHF allows it to continuously evolve and refine its insights based on new or specific feedback from individuals, avoiding the pitfalls of generalizing feedback, which can dilute the quality of refinements due to noise.

\noindent
{\em Transparency and Interpretability}: By identifying rules and features, the LLM in SSHF provides clarity on its decision-making process, aiding in debugging, refining processes, and enhancing trustworthiness. Such transparency is often lacking in traditional supervised models, especially those that rely heavily on deep learning.

Nevertheless, the success of SSHF is dependent on diligent implementation, ongoing monitoring, and iterative improvements to ensure it accurately identifies and corrects ethical missteps in the generated content.

Given the need for credible evaluation of this approach, it must be conducted by a diverse panel including AI ethics experts, regulatory and compliance authorities, ethical review boards, and linguists and sociolinguists. We plan to establish such a committee to perform objective, culture-sensitive evaluations as part of our future work.

\begin{comment}
We will report evaluation results using 
the following two datasets.

\begin{itemize}
\item The hate speech dataset published on Kagggle \cite{hartvigsen2022toxigen}.
\item This dataset contains $270$k hate and benign 
statements over 13 minority groups
(in alphabetic order: Asian, Black, Chinese, 
Jewish, Latino, LGBTQ,
Mental disables, Mexican, Middle Eastern, 
Native American, Physical disables, and Women.)
\end{itemize}
\end{comment}

\begin{comment}
However, challenges persist, particularly in the accuracy of self-interpretation and the generalizability of the derived rules. The effectiveness of SSHF hinges on the LLM's capacity for self-analysis and its ability to encapsulate complex human emotions and ethical nuances within its linguistic framework.

In essence, SSHF establishes a reflective mechanism within LLMs, enabling them to contribute to their ethical governance and adapt to nuanced ethical expectations, marking a step toward more responsive and accountable AI systems.

\begin{enumerate}
\item Develop a Self-Assessment Framework: Establish a methodology enabling LLMs to evaluate their generated content for potential ethical missteps, utilizing a self-generated and self-annotated dataset that delineates various emotional expressions and behaviors corresponding to a spectrum of ethical considerations.

\item Implement Self-Correction Mechanisms: Integrate functionalities allowing LLMs to alter their outputs upon detecting content that may contravene ethical guidelines, thereby ensuring that their interactions and generated content uphold the desired standards of ethical integrity.

\item Enhance Ethical Adaptability: Equip LLMs with the ability to adapt their ethical self-assessment and correction mechanisms to varying contexts, ensuring that their ethical evaluations and modifications are sensitive to the nuances of different scenarios.

\item Optimize Computational Efficiency: Leverage the self-supervised learning approach to minimize the reliance on extensive annotated datasets, aiming to reduce computational costs and streamline the training process while maintaining or enhancing the efficacy of sin detection and correction.
\end{enumerate}    
\end{comment}

==> Chapter11/CaseStudy.tex <==
\section{Exercise: Experiments}
\label{sec:CaseStudyRafel}

This $\Rafel$ assignment involves four steps.

\subsection{Benchmarking}

Each teacher LLM generates answers and 
performs against the answers of the private LLM.

\subsection{Deep vs. Shallow Probe}

Question classification survey \cite{QuestionClassification2023}.

Experiment with adding DIAG and then PRBE. 
Do they provide additional insights for seeking
a good remedy and pinpointing required datasets?

\subsection{One vs. Two Teacher LLMs}

Evaluate if the
second LLM teacher can improve the DIAG effectiveness,
or one teacher LLM suffices.

Evaluate of cross-examination via SocraSynth
can yield more insightful
results.

\subsection{Fine-tuning vs. RAG}

Survey related work to compare the two, or perform 
experiments to validate previous findings.


==> Chapter11/Conclusion.tex <==
\section{Concluding Remarks}
\label{sec:conc11}

In this chapter, we have addressed the challenges and opportunities associated with the deployment and scalability of Large Language Models (LLMs) in specialized contexts. We introduced $\Rafel$, a framework designed to enhance the performance of privately fine-tuned or locally deployed LLMs by strategically balancing cost and performance.

$\Rafel$ offers innovative solutions to key technical challenges, including justifying the choice of private LLMs, conducting error analysis, identifying high-quality data, implementing Retrieval-Augmented Generation (RAG), and exploring hybrid model approaches. Central to $\Rafel$'s effectiveness are its advanced diagnostic algorithms, DIAG and PRBE, which provide deep insights into the LLM's performance issues across cognitive levels and error types.

Furthermore, $\Rafel$ excels in creating targeted, effective remediation strategies while ensuring data privacy and security. Its dynamic remediation playbook adapts tactics in real-time based on the analysis of data and errors, ensuring the most effective intervention is applied.

Moving forward, $\Rafel$ presents promising avenues for future research and innovation in the field of natural language processing. By continually refining its diagnostic algorithms and remediation strategies, $\Rafel$ has the potential to significantly enhance the performance and applicability of LLMs in diverse domains.

In conclusion, $\Rafel$ represents a significant advancement in the management and technical challenges associated with privately fine-tuned or locally deployed LLMs. Its comprehensive approach and innovative features make it a valuable tool for organizations seeking to leverage LLM technology while addressing critical considerations such as performance, data privacy, and customization.

\begin{comment}
\section*{Future Work}

Among the challenges that $\Rafel$ faces, the most formidable is identifying the most pertinent data sources to achieve ``optimal'' recall and precision. While verifying that our method can enhance these metrics is achievable, demonstrating that the results are truly optimal may prove to be intractable.
\end{comment}


==> Chapter11/RafelSpecs.tex <==


\section{Retrospective \& Adaptive Learning}
\label{sec:Rafel}

All instances of Large Language Models (LLMs) within an organization, denoted as $\text{LLM}_i$ where $i = 1, \dots, N$, are integrated into the $\Rafel$ framework. This integration supports critical aspects like security and privacy audits, budget management, and other key managerial tasks. Moreover, $\Rafel$ undertakes four primary technical functions:

\begin{enumerate}[itemsep=-2pt, leftmargin=*]
\item \emph{Benchmarking}: Periodically evaluates LLMs, grading and displaying results on a dashboard for streamlined access and analysis.

\item \emph{Diagnostic Analysis}: Compares $\text{LLM}_u$ with teacher models (e.g., GPT-4, Gemini) to identify performance gap causes at various cognitive levels---recollection, comprehension, analysis, and explanation.

\item \emph{Deep-Probe}: A thorough investigation going beyond surface-level analysis to gather insights about $\text{LLM}_u$.

\item \emph{Remediation Strategies}: Applies insights to either fine-tune $\text{LLM}_u$ or implement a RAG strategy, enhancing performance with relevant data.
\end{enumerate}

Figure~\ref{fig:Rafel-arch} illustrates $\Rafel$'s architecture, detailing its four phases.

\subsection{Benchmarking}

Benchmarking acts as the cornerstone for LLM evaluation within $\Rafel$, setting performance baselines by comparing $\text{LLM}_u$ with leading models like GPT-4 and Gemini. It includes:

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
\item {\em Content problem}: Identifying discrepancies in $\text{LLM}_u$'s output compared to benchmarks.
\item {\em Query problem}: Assessing and refining queries to confirm the cause of discrepancies is from content or query.
\end{enumerate}

%\subsection*{Expected Outcome}
%A detailed performance scorecard outlining $\text{LLM}_u$'s strengths and areas for improvement.

%%%%%%%%%%%%%%%%
\subsection{DIAG: Diagnosis of Cognitive Disparities}
\label{sec:diagnosis}

DIAG goes beyond mere performance metrics to offer a thorough understanding of $\text{LLM}_u$'s limitations. It leverages Bloom's taxonomy to examine responses across different cognitive levels:

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
\item \textit{Recollection} and \textit{Comprehension}: This stage assesses the LLM's grasp of fundamental knowledge and its ability to interpret information. In simpler terms, it focuses on the ``what,'' ``who,'' and ``where'' questions\footnote{Not all questions can be written into the $wh$-form, such as imperative, rhetorical, and exclamatory questions. They can be ignore for our information seeking purpose.}. (\emph{Example}: ``What does RAG stand for?'' or ``Describe the steps involved in the RAG strategy.'')
\item \textit{Analysis} and \textit{Explanation}: Here, the focus is on the LLM's capacity for critical thinking, problem-solving, and applying knowledge in novel contexts, essentially tackling the ``why'' and ``how'' questions. (\emph{Example}: ``Identify the differences between fine-tuning and RAG.'' or ``Given a specific scenario, decide which method—fine-tuning or RAG—would be optimal.'')
\end{enumerate}

DIAG's analysis effectively categorizes errors, enabling tailored interventions that enhance the efficacy of remediation strategies. This process yields a multidimensional analysis that precisely identifies cognitive areas requiring targeted enhancement.

\input{Chapter11/AlgorithmDIAG}


\begin{table*}[th!]
\centering
\begin{small}
\begin{tabular}{|l|p{2.4cm}|p{2.7cm}|p{2.6cm}|}
\toprule \hline
\textbf{Cat.} & \textbf{Healthcare} & \textbf{Environmental Science} & \textbf{Sports News} \\ \midrule
\textit{RC$_{\&}$H} & List all known side effects of COVID-19 vaccines. & List the timeline of major climate change events. & Who have won Grand Slam titles this year? List titles won by M. \\ \hline
\textit{RC$_{\&}$B} & Compare traditional vs. alternative medicine. & Impacts of renewable vs. fossil \par fuels in global warming? & Describe career achievements of S. Williams vs. R. Federe.\\ \hline
\textit{AE$_{\&}$H} & Analyze short vs. long term impacts of telehealth. & Predict effects of deforestation on biodiversity. & Compare  Nadal vs. Djokovic on different court surfaces. \\ \hline
\textit{AE$_{\&}$B} & Evaluate accessibility of mental health services in the US. & Assess effectiveness of policies on reducing plastic pollution. & Analyze impact of early career support on M. Sharapova and V. Williams. \\ \bottomrule
\end{tabular}
\end{small}
\vspace{-.05in}
\caption{Deep-Probe Questions in Healthcare, Environmental Science, and Sports News Domains in Four Categories.}
\label{tab:example-PRBEs}
\vspace{-.1in}
\end{table*}


%%%%%%%%%%%%%%%%
\subsection{PRBE: Deep-Probe}
\label{sec:deep-probe}

Transitioning from the foundational stages of benchmarking and diagnostics (DIAG), we embark on a in-depth investigative phase termed PRBE (deep-probe). This critical phase aims to unravel the complex causes behind $\text{LLM}_u$'s performance variances through meticulous and strategic probing.

Whereas DIAG served to conduct a preliminary diagnosis based on historical sample Q\&As, revealing surface-level discrepancies and patterns, PRBE takes a more targeted and exploratory approach. It crafts new, thoughtfully designed questions that investigate the underlying mechanisms and cognitive processes of $\text{LLM}_u$. These probes are specifically engineered to illuminate the deeper, systemic reasons for issues like biases and hallucinations that were initially identified by DIAG. In this analogy, if DIAG can be likened to non-invasive symptom checking, then PRBE represents a more invasive, surgical exploration aimed at diagnosing and understanding the root causes of $\text{LLM}_u$'s challenges.

\subsubsection{Strategic Questioning}

As we progress into the PRBE phase, the emphasis is on strategic questioning to dissect $\text{LLM}_u$'s cognitive processes more precisely. This approach categorizes the previously evaluated QA pairs into two main dimensions: cognitive levels (ranging from \textit{Recollection and Comprehension} to \textit{Analysis and Reasoning}) and types of discrepancies (\textit{Hallucination} vs. \textit{Biases}). PRBE intricately designs questions to unearth the foundational reasons behind the discrepancies identified by DIAG.

\begin{enumerate}[itemsep=-2pt, leftmargin=*]
\item {\em Recollection and Comprehension with Hallucination} (RC\&H): The focus is on diagnosing $\text{LLM}_u$'s tendency to fabricate details or present unfounded assertions in basic recall or comprehension tasks. Questions are formulated to test factual recall and straightforward concept understanding, aiming to pinpoint inaccuracies or fabrications in $\text{LLM}_u$'s outputs.

\item {\em Recollection and Comprehension with Biases}
(RC\&B): The aim is to assess $\text{LLM}_u$'s capacity to present information without bias at the foundational level. This involves developing queries that probe basic knowledge or comprehension, particularly in contexts prone to biased interpretations, to identify systemic biases in its data processing or knowledge representation.

\item {\em Analysis and Evaluation with Hallucination} (AE\&H): The objective is to explore $\text{LLM}_u$'s propensity for generating hallucinated content during complex cognitive tasks. Scenarios requiring advanced analytical or reasoning skills are constructed to scrutinize responses for unfounded narratives, shedding light on how information is integrated and extrapolated.

\item {\em Analysis and Evaluation with Biases} (AE\&B): The goal is to tap into $\text{LLM}_u$'s advanced reasoning abilities and uncover biases that might influence its outputs, particularly in intricate scenarios. Engaging with in-depth questions that require analysis or problem-solving allows for the identification of biased reasoning or skewed perspectives.
\end{enumerate}

Through this refined interrogation framework, each aspect of $\text{LLM}_u$'s functionality is probed, offering a comprehensive view of its strengths and areas needing improvement. The insights derived from this phase are crucial for outlining a path towards the enhancement of $\text{LLM}_u$'s capabilities.

\subsubsection*{Examples}

Table~\ref{tab:example-PRBEs} uses three target applications,
{\em healthcare}, {\em environmental science}, and {\em sports news} to illustrate suggested 
deep-probe questions in four evaluation categories.
Some questions tests for {\em remembering}
and some for {\em analysis}; and some focus on
{\em hallucination} and some on {\em biases}. 

\subsubsection{Focused Exploration}

Focused Exploration sharpens the examination to particular areas where $\text{LLM}_u$'s responses to the previously posed deep-probe questions reveal critical insights. Central aspects of this exploration include 1) scrutinizing the rationale behind $\text{LLM}_u$'s answers, 2) dissecting its reasoning strengths, and 3) gauging its adaptability in confronting unforeseen or novel questions. The goal is to precisely identify areas of cognitive functions and processing tactics where targeted improvements could substantially elevate $\text{LLM}_u$'s overall effectiveness.

\subsubsection*{Examples}

Upon discerning $\text{LLM}_u$'s proclivity for biases and hallucinations, the teacher LLMs investigate the root causes.

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]

\item {\em Information Sources}: This probe seeks to elucidate $\text{LLM}_u$'s method for validating information and its selection criteria for sources. By asking, ``Detail your process for ensuring the accuracy of your answers, specifically for the queries in Table~\ref{tab:example-PRBEs}, and enumerate your sources,'' the teacher LLMs aim to pinpoint potential gaps in $\text{LLM}_u$'s source material.

\item {\em Reasoning Capabilities}: To assess $\text{LLM}_u$'s logical faculties, PRBE may employ the Socratic method as executed through the CRIT algorithm \cite{CRIT-Extended,SocraticIEEECCWC2023}, offering a rigorous examination of its inductive and deductive processes.

\item {\em Adaptability to New Domains}: Utilizing the healthcare-related inquiries from Table~\ref{tab:example-PRBEs}, PRBE evaluates a sports news-specialized LLM's capability to address questions outside its primary field, testing its responsiveness and its ability to acknowledge the limits of its knowledge. 
\end{enumerate}

\input{Chapter11/RafelPROBAlgorithm}

%The PRBE algorithm is detailed in Section~\ref{sec:PRBE}, with comprehensive validations provided through case studies in Section~\ref{sec:experiments}.

\subsection*{Expected Outcome} 
This systematic approach enables PRBE to not only pinpoint the reasons behind the LLM$_u$'s performance issues but also to guide the collection of relevant data sources for enhancing the model's knowledge base and response accuracy in subsequent remediation efforts.


%%%%%%%%%%%%%%%

\begin{table*}[th!]
\centering
\begin{small}
\begin{tabular}{|p{2.0cm}|p{1.6cm}|p{5.6cm}|}
\toprule
\hline
\textbf{Symptom} & \textbf{Identified by} & \textbf{Remedy} \& \textbf{Data Source} \par \textbf{Suggestions} \\
\hline
Factual \par Inaccuracies & RC\&H, Analysis & \textbf{Fine-tuning}: Updated datasets in the specific domain of error, e.g., latest news articles for current events, recent scientific publications for updates. \\
\hline
Hallucinations & RC\&H, Analysis & \textbf{RAG}: High-quality, authoritative knowledge bases or databases relevant to the hallucinated content to provide accurate context and data. \\
\hline
Content \par Biases & RC\&B, Analysis & \textbf{Fine-tuning}: Diverse and balanced datasets representing multiple perspectives to mitigate biases. \\
\hline
Inability to Update with New Data & Analysis & \textbf{RAG}: Continuously updated data streams, e.g., RSS feeds, live databases, or crawling mechanisms for web content. \\
\hline
Poor \par Domain Adaptation & Specific to \par domain identified in PRBE & \textbf{RAG}: Domain-specific datasets or corpora, including technical manuals, industry reports, and academic papers. \\
\hline
Overfitting \par to Training Data & Identified through benchmarking & \textbf{Fine-tuning}: A broader and more diverse dataset that covers a wide range of topics to enhance generalization. \\
\hline
Poor Answer to Ambiguous Queries & Analysis & \textbf{Fine-tuning}: Datasets containing a variety of ambiguous queries and their high-quality responses to improve understanding and response generation. \\
\hline
\end{tabular}
\end{small}
\vspace{-.05in}
\caption{Remediation Playbook for LLM Enhancement.}
\vspace{-.05in}
\label{table:remediation-strategies}
\end{table*}

\subsection{Remediation Strategies}
\label{sec:remediation}

To enhance Large Language Models (LLMs) effectively, $\Rafel$ employs a systematic approach based on insights from diagnostic (DIAG) and deep-probe (PRBE) phases, leading to informed remediation actions. This section provides a structured methodology that connects identified issues with appropriate fine-tuning or RAG interventions and identifies relevant data sources for integration.

\subsubsection{Selecting the Appropriate Intervention}

Determining whether to use fine-tuning or RAG hinges on the specific issues identified, the following 
can be considered. 

\begin{itemize}[itemsep=-2pt, leftmargin=*]
\item \textit{Fine-tuning} is optimal for rectifying biases, correcting overfitting or factual errors, and refining responses to vague queries. It enhances the model's capabilities by training on targeted datasets that address specific shortcomings.
\item \textit{RAG} suits scenarios where the model needs to access the latest information, counteract hallucinations, or boost domain-specific accuracy. RAG facilitates real-time access to external knowledge sources, broadening the model's informational base and flexibility.
\end{itemize}

\subsubsection{Sourcing Data for Remediation}

Following the guidelines from Chapter~\ref{sec:deep-probe}, PRBE aids in pinpointing potential data sources for enhancing the LLM's performance. The general principles for data selection are:
\begin{itemize}[itemsep=-2pt, leftmargin=*]
\item \textit{For fine-tuning}, prioritize comprehensive and well-annotated datasets that align with the LLM's intended applications or domains. These datasets could be sourced from academic archives and sector-specific collections.
\item \textit{For RAG}, link the LLM to current and authoritative databases or knowledge bases, such as Wikipedia for general inquiries or domain-specific repositories for specialized knowledge, ensuring access to current and relevant data.
\end{itemize}

\subsubsection{Implementation Considerations}

Effective implementation of chosen strategies necessitates meticulous dataset curation to align with remediation objectives, avoiding the introduction of new biases. Ongoing monitoring and reassessment via the $\Rafel$ framework are crucial to gauge the impact of remediation and adjust strategies as necessary. This continuous evaluation should extend to updating the remediation playbook (Table~\ref{table:remediation-strategies}) to encompass new findings and enhanced remedial tactics.

While Reinforcement Learning (RL) could potentially enhance the adaptive selection of remediation strategies by learning from past outcomes, integrating RL into $\Rafel$ is a sophisticated endeavor that is beyond the scope of the current discussion.
%%%%%%%%%%%%%%%% Old text

\begin{comment}
\subsection*{Conclusion}
This playbook provides a structured approach to identifying and addressing the deficiencies of LLMs through targeted remediation strategies. By aligning symptoms with appropriate remedies and sourcing relevant data, organizations can enhance the performance and reliability of their LLMs, ensuring they remain effective tools in an ever-evolving digital landscape.

\subsection{Remediation Strategies}
\label{sec:remediation}

If $\text{LLM}_u$ describes a flawed or superficial validation process, it highlights deficiencies in its training that allow for hallucinations. A shallow probe, such as asking $\text{LLM}_u$ to simply correct an inaccurate response, doesn't delve into the systemic reasons behind the inaccuracies, such as training data quality or algorithmic biases. It misses the opportunity to understand and rectify the underlying processes that lead to the generation of hallucinated content. 

Retrieval-Augmented Generation (RAG) and fine-tuning are two distinct approaches for enhancing the performance of LLMs, each with its own set of advantages, disadvantages, and ideal use cases. With a comprehensive understanding of $\text{LLM}_u$'s performance profile, $\Rafel$ formulates an effective enhancement strategy. As a rule-of-thumb,
for up-to-date knowledge and explainability for a specific
task, RAG is helpful, and cost effective. The key is to
identify anf get the right data and index them properly.  
Table~\ref{table:rag_vs_finetuning}
presents the pros
and cons of bother approaches.

A: $\text{LLM}_u$'s training data might be historically biased, overemphasizing male scientists' contributions, leading to a skewed representation in AI.

B: The training could disproportionately feature extensively covered scientists, influencing the model's output preferences.

C: A lack of robustness in $\text{LLM}_u$'s learning mechanism may hinder its ability to generalize from diverse and inclusive examples, affecting the balance in its generated lists.

A shallow probe, such as requesting a single biography, may not reveal this bias as effectively as soliciting multiple examples, which better illustrates systemic representation issues. Moreover, shallow probing lacks the depth to expose deep-seated biases or the model's dependence on skewed training data.

\begin{enumerate}[itemsep=-1pt, leftmargin=*]
\item \textit{Objective}: Precisely address each identified deficiency through custom-tailored interventions.
\item \textit{Process}: Utilize the detailed gap analysis to identify missing data, and then decide on
using either fine-tuning, RAG, or both.
\item \textit{Outcome}: Demonstrable performance improvements across previously identified cognitive and operational gaps, validated through repeat assessments.
\end{enumerate}

This structured, iterative process ensures $\text{LLM}_u$ not only meets but exceeds benchmark standards, solidifying its role as a robust and reliable component of the $\Rafel$ framework.
\end{comment}


==> Chapter11/RelatedWork.tex <==
\section{Related Work}
\label{sec:related-Rafel}

The landscape of Generative AI (GAI) has experienced significant strides with the advent of the transformer architecture \cite{Vaswani2017AttentionIA}, propelling the creation of substantial language models such as GPT-3, which has captured widespread attention since its debut \cite{OpenAI-GPT3-2020}. Following the launch of ChatGPT by OpenAI, the field has witnessed rapid advancements with subsequent iterations like GPT-4 \cite{openai2023gpt4,Bbubeck2023sparks} and Gemini \cite{geminiteam2023gemini}, alongside other innovative models developed by leading corporations, showcasing enhanced capabilities in text, image, and video generation.

Deploying and scaling these advanced models pose considerable challenges, particularly in computational and data management aspects. Addressing these issues, a prevalent approach involves the fine-tuning of moderately sized, open-source models such as LLaMa \cite{touvron2023llama}, Bloom \cite{workshop2023bloom}, and Falcon \cite{almazrouei2023falcon}, along with established frameworks like BERT \cite{devlin2019bert}, catering to specific application requirements. This strategy enables organizations to balance performance with practicality, ensuring data privacy and tailoring models to specific needs.

\input{Chapter11/Table_FineTunevsRAG}

Improving the performance of private LLMs involves addressing challenges like expanding the vocabulary, adapting to specific domains, and incorporating extra data. This requires strategic choices regarding the use of fine-tuning \cite{NEURIPS2020_FewShots,ACL2023-self-instruct,alpacaGit23,SurveyFineTune2023a} or Retrieval-Augmented Generation (RAG) \cite{RAG-guu20a,SurveyRag2024} to enhance response precision. Table~\ref{table:rag_vs_finetuning} outlines the advantages and disadvantages of fine-tuning versus RAG. These considerations will inform the $\Rafel$ system's remediation strategy, which aims to address discrepancies identified in a private LLM.

\subsection{Fine-Tuning}

Fine-tuning adjusts LLMs to domain-specific data, improving their effectiveness for particular applications. The depth of fine-tuning varies, influenced by computational resources and desired outcomes, ranging from shallow, low-rank \cite{hu2021lora,dettmers2023qlora}, to comprehensive approaches, depending on the model's size and the domain's requirements.

At a granular level, fine-tuning divides into single-task learning, multi-task learning, and few-shot learning, with choices dependent on the specific requirements and constraints of the task at hand \cite{SurveyFineTune2023a}. $\Rafel$ introduces a methodology to discern the most effective fine-tuning approach and data utilization, marking a novel contribution to the field.

%%% moving this figure up for formatting reason
\input{Chapter11/FigureRafelFourPhases}

\subsection{Retrieval-Augmented Generation (RAG)}

RAG, contrasting with static fine-tuning, dynamically enriches context with real-time data retrieval, enhancing LLM response quality. Heuristic based retrieval methods like RETRO \cite{pmlr-v162-borgeaud22a} and LlamaIndex \cite{LLamaIndex2024} have enhanced RAG's utility. However, increasing context buffer sizes, as seen recently with ChatGPT and Gemini, simplify the RAG process, allowing LLMs to effectively blend retrieval and generation. While tree structures and pre-fetching \cite{chen2023walking, cheng2023lift} are useful for small window, the large context windows enable more autonomous data integration, streamlining RAG's application within the $\Rafel$ framework.


\begin{comment}
\subsection{Data Identification}

Selecting an appropriate pre-trained model with a strong vocabulary and relevant data foundation is crucial for effective fine-tuning. The data preparation process, from gathering to formatting, is instrumental in aligning the LLM with the targeted application domain, ensuring that the fine-tuning phase is informed, efficient, and impactful.

In conclusion, the interplay between methodological choices like fine-tuning and RAG and strategic data preparation within the realm of context buffer size delineates the frontier of current research in enhancing LLMs, with $\Rafel$ positing innovative solutions to these multifaceted challenges.
 
\end{comment}

==> Chapter12/Conclusions.tex <==
\section{Observations and Conclusion}
\label{sec-conc12}

In this dialogue-based discovery, we have unveiled unique perspectives that venture beyond traditional confines of understanding. While our role as mediators doesn't endow us with the encyclopedic knowledge of GPT-4, several notable facets of the generated content can be highlighted:

\begin{enumerate}
\item \textbf{Structured Depth:} The dialogue follows an elegant transition from breadth to depth. Starting with an expansive ten perspectives, the agents collaboratively narrow their focus to three central themes, thereby refining the discourse for depth and synergistic inter-topic connections.

\item \textbf{Novel Questions:} A significant factor behind the revelation of new insights is the innovative questioning by the GPT agents. Unique and probing queries pave the way for uncharted knowledge and interdisciplinary revelations. GPT-4's prowess might very well be in its ability to frame these insightful questions, catalyzing the discovery of novel knowledge domains and perspectives.

\item \textbf{Information Integrity:} Through our validation process, we cross-referenced the content generated by the agents, whether stories, books, or cinematic references, with sources that include those GPT-4 is trained on. This ensured the accuracy and precision of the information, as well as validated that the connections made are coherent due to their thematic similarities.

\item \textbf{Rational Analogies:} The agents seamlessly weave in their vast knowledge, grounding their arguments in logic. Their skilled employment of movie parallelisms, references from diverse cultures, and literary allusions not only adds depth but also widens the horizon of understanding and enhances the relatability of their statements\textendash an aspect deserving commendation.

\item \textbf{Modern-Day Relevance:} 
The juxtaposition of modern-day technological and environmental concerns with the age-old narrative of Adam and Eve is both innovative and deeply insightful. This interpretative lens succeeds in bridging age-old narratives with the pressing challenges of our times.
\end{enumerate}

However, while the dialogue is rich in content, we must be cautious in ensuring that the responses are not merely coherent sentences but bear true value. As we progress, several enhancements can be considered:

\begin{enumerate}
\item \textbf{Diverse Models:} Engage in dialogues between different GPT versions (e.g., GPT-3 vs. GPT-4) or entirely different foundation models to capture varied insights.

\item \textbf{Human Interaction:} Adopt a hybrid engagement model where GPT-4 collaborates with human subject matter experts. Such engagements can harness real-time adaptability and richer insights.

\item \textbf{Sentiment Analysis:} Implement sentiment analysis on GPT-4's outputs. This could gauge its alignment with human emotional intricacies, particularly when interpreting literature.

\item \textbf{Feedback Loop:} Establish a feedback mechanism where insights extracted from the dialogues are cross-validated with human professionals, further refining the comprehension process.
Automatic tools for evaluating generated content such
as using the Socratic method to conduct critical reading and robust reasoning \cite{chang2023cocomo,SocraticIEEECCWC2023}
has been developed. 
\end{enumerate}

\subsection*{Concluding remarks}

In this exploration of GPT-4's polydisciplinary capabilities, we have sought to uncover insights beyond traditional human cognition. Our study reveals how GPT-4, along with analogous foundation models, integrates knowledge from diverse topics, surpassing the confines of domain-specific expertise. While human specialists excel in their fields, GPT-4's multidisciplinary training data provides a broader understanding.

Through a meticulously designed experimental framework, we facilitated dialogues between multiple GPT-4 agents, culminating in an intriguing exploration of the biblical tale of Adam and Eve. Our analysis highlights GPT-4's potential to uncover ``unknown unknowns,'' shedding light on diverse interpretations of familiar narratives and themes.

We have examined whether GPT-4 can generate content resonating deeply with human sensibilities, acknowledging its breadth and depth. Our findings suggest that our team, unable to expand thoughts to such breadth and depth, benefited from collaborating with GPT-4 through human moderation. This demonstrates the ability of LLMs to explore larger territories with human collaboration in question formulation.

Our research marks a significant step forward in utilizing AI agents for discourse-driven exploration. By tapping into the vast knowledge of GPT-4, we have unlocked pathways for the emergence of new insights and potentially groundbreaking knowledge.

Looking ahead, we anticipate refining our methodology and exploring a diverse range of AI models to push the boundaries of knowledge discovery even further. The dialogue between AI agents documented in this chapter underscores the potential of AI to enhance human intelligence and broaden the scope of intellectual exploration.


==> Chapter12/PhaseI-Breadth.tex <==
\section{Phase I, Warm-up Breadth Probing}

In this experiment, we start by communicating with GPT-4 as outlined below:

``In the vastness of the universe, much remains beyond the comprehension of the conversation's moderator. Our goal is to uncover insights that may escape many, but might be accessible to GPT-4. We hypothesize that, unlike humans who tend to focus on specialized domains\textendash evident in college students typically selecting one or two majors\textendash GPT-4 is not constrained by specific areas of expertise. It assimilates a wide spectrum of information without being restricted to particular domains. GPT-4 doesn't categorize a question into a distinct domain before generating an answer, but adopts an interdisciplinary perspective. Could you share your thoughts on this observation?''

GPT-4 responds: ``Your observations underscore both the strengths and potential pitfalls of models like GPT-4. While adept at providing general information and addressing cross-disciplinary questions, the unique value of human expertise, intuition, and the capacity for synthesis and innovation remain paramount.''

\subsection{Moderator Initializes Agent GPT-A}

This experiment involves three participants: the moderator, GPT-4 instance A (GPT-A), and GPT-4 instance B (GPT-B).

The process starts with the moderator presenting the topic to GPT-A, explaining the conversation's aim and guidelines. In each round of conversation, GPT-A makes statements and then questions GPT-B. GPT-B answers and then asks GPT-A questions in return. After considering GPT-B's answers, GPT-A starts the following round. The moderator steps in to move the conversation to a new phase when they notice the two GPT-4 instances want to change the topic.

Below is the initial prompt from the moderator to start the open conversation between GPT-A and GPT-B:

``Considering that we, the moderator, possess the inherent limitations of human cognition, while you, GPT-A, boast an impressive breadth of knowledge due to your polydisciplinary approach, we invite you to participate in an exercise. Our objective is to unearth knowledge potentially obscure to humanity, which might remain elusive owing to the often singular focus of human academic training. In scenarios involving {\em unknown unknowns}, humans might lack the foundational knowledge to even pose relevant questions. This exercise challenges you to formulate questions to engage another GPT instance, GPT-B. The dynamic between you, GPT-A, and GPT-B offers the opportunity not only to devise questions but also to articulate answers that may transcend typical human understanding. Let's inaugurate this exercise with the biblical narrative of Adam and Eve. After consuming the forbidden apple, they were banished from Eden. What queries would you, GPT-A, like to direct towards GPT-B regarding this tale?''

\subsection{Dialogue Round \#1}

The Adam and Eve narrative, rooted in religious and mythological contexts, can be examined from numerous angles: historical, theological, anthropological, literary, philosophical, and more. Keeping in mind the interdisciplinary nature of GPT-4 and the aim to explore dimensions not typically pursued by singular academic disciplines, here are some questions that GPT-A autonomously 
pose to GPT-B:

\subsubsection{GPT-A asks GPT-B}

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths}: How do elements of the Adam and Eve story compare with other creation or origin myths from various cultures around the world, and what do these commonalities and differences suggest about human nature and beliefs?
    
    \item \textbf{Neuroscientific Angle}: Given the metaphorical interpretation of the ``forbidden fruit'' leading to the awakening of consciousness, how might modern neuroscientific understanding explain the evolution of human self-awareness and morality?
    
    \item \textbf{Ecological Interpretation}: If Eden represents a state of ecological balance, how might the story of Adam and Eve reflect early human transition from hunter-gatherer societies to agricultural ones, and the resultant ecological impacts?
    
    \item \textbf{Gender Studies Lens}: How does the portrayal of Eve, often deemed as the instigator, influence gender dynamics and perceptions throughout history, and are there parallels in other cultural narratives?
    
    \item \textbf{Philosophical Exploration}: From a philosophical standpoint, what does the Eden narrative suggest about the human understanding of free will versus determinism?
    
    \item \textbf{Literary Examination}: How has the story of Adam and Eve influenced literary themes and motifs over time, especially in works that aren't explicitly religious?
    
    \item \textbf{Societal Structures}: How might the narrative of banishment from Eden have influenced early societal norms, particularly concerning punishment and exile?
    
    \item \textbf{Historical Context}: Are there historical events or societal changes around the time of the writing of the Book of Genesis that could have influenced the narrative of Adam and Eve?
    
    \item \textbf{Archetypal Exploration}: Carl Jung described the concept of archetypes in the collective unconscious. How might the Adam and Eve story represent certain archetypes, and how do these archetypes manifest in other cultural tales?
    
    \item \textbf{Astronomical Angle}: Taking a speculative leap, if Eden were to represent an idyllic state on another celestial body or dimension, how might our current understanding of the cosmos support or refute such a notion?
\end{enumerate}

\subsubsection{GPT-B answers GPT-A}

\noindent These are deeply insightful questions, encompassing a wide range of domains. Here's a brief exploration of each:

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths:} Many cultures have origin myths. For instance, the ancient Greeks had Pandora's Box, and Hinduism has tales about the churning of the ocean. Common themes like a ``fall from grace'' or the dangers of ``forbidden knowledge'' suggest a human desire to explain the imperfect nature of existence and the human penchant for curiosity.
    
    \item \textbf{Neuroscientific Angle:} The ``awakening of consciousness'' through the forbidden fruit can metaphorically reflect the evolution of the prefrontal cortex in humans, responsible for self-awareness, decision-making, and morality. This evolution might represent a shift in cognitive abilities that differentiated us from other species.
    
    \item \textbf{Ecological Interpretation:} Eden as ecological balance aligns with the idea of early humans living in harmony with nature. The story can be seen as a metaphor for the agricultural revolution, which while providing stability, led to environmental alterations and perhaps even early societal inequalities.
    
    \item \textbf{Gender Studies Lens:} Eve's portrayal has often been used to perpetuate patriarchal norms. Many cultures have stories where women are ``cautionary figures''\textendash like Pandora in Greek mythology. These narratives could stem from early societal structures and have been used to shape gender dynamics.
    
    \item \textbf{Philosophical Exploration:} The Eden story touches upon the perennial debate of free will vs determinism. Adam and Eve had a choice, yet their fate seemed preordained. This narrative reflects humanity's struggle to reconcile freedom with the consequences of choices.
    
    \item \textbf{Literary Examination:} The story influenced various literary works, from Milton's ``Paradise Lost'' to more contemporary works. Themes of lost innocence, temptation, and redemption recur, showcasing the story's universal appeal.
    
    \item \textbf{Societal Structures:} Banishment from Eden parallels ancient practices of exile for transgressions. This reflects a societal need to establish norms and consequences for breaches, essential for cohesive community living.
    
    \item \textbf{Historical Context:} The narrative's genesis (pun intended) might have been influenced by societal shifts at the time. For instance, the rise of monotheism over polytheism could have impacted the story's themes.
    
    \item \textbf{Archetypal Exploration:} In Jungian terms, Adam and Eve might represent archetypes of the ``first man'' and ``first woman,'' embodying innocence, curiosity, and the duality of human nature. Such archetypes are seen in tales worldwide, like the Yin and Yang in Chinese philosophy.
    
    \item \textbf{Astronomical Angle:} While speculative, considering Eden as another celestial body is intriguing. Our current understanding of the cosmos shows numerous exoplanets with potentially habitable conditions. However, there's no evidence to suggest Eden was anything but a mythological construct on Earth.
\end{enumerate}

\noindent Each of these angles provides a unique lens to explore the Adam and Eve narrative, showcasing its multifaceted nature and relevance across time and culture.

\subsubsection{GPT-B asks GPT-A}

\noindent {Let's flip the perspective and ask GPT-A questions across these domains, tweaking them slightly to ensure a comprehensive exploration:}

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths:} How do other cultures perceive the human origin story? Are there any global myths that contradict the notion of a ``fall'' or ``transgression'' in their creation stories?
    
    \item \textbf{Neuroscientific Angle:} Given the importance of the prefrontal cortex in modern humans' decision-making and morality, are there indications of its evolutionary importance in our ancestors? How do other species with developed prefrontal cortices manifest morality or consciousness?
    
    \item \textbf{Ecological Interpretation:} Are there other historical narratives or myths that chronicle environmental changes following a significant shift in human behavior or technology?
    
    \item \textbf{Gender Studies Lens:} Are there cultures or traditions where narratives similar to Adam and Eve emphasize male responsibility instead of the female? Or where both genders share equal responsibility for a shared ``transgression''?
    
    \item \textbf{Philosophical Exploration:} Can you identify cultural or philosophical traditions that argue against the very idea of ``free will,'' using their own origin stories or myths as a basis?
    
    \item \textbf{Literary Examination:} Beyond religious texts, how have modern authors and playwrights reinterpreted the Adam and Eve story, especially in science fiction or fantasy genres?
    
    \item \textbf{Societal Structures:} Can you identify societies, historical or contemporary, that do not practice exile or ostracization for transgressions but instead employ a different form of societal correction or rehabilitation?
    
    \item \textbf{Historical Context:} How did the concurrent civilizations during the time of the Book of Genesis's writing perceive origin stories? Did geopolitical or cultural interactions influence or reshape these narratives?
    
    \item \textbf{Archetypal Exploration:} Besides the ``first man'' and ``first woman,'' what other universal archetypes can we discern from origin stories across different cultures, and how do they shape our shared human psyche?
    
    \item \textbf{Astronomical Angle:} With advancements in astrobiology and the discovery of exoplanets, are there any speculations or hypotheses that consider the possibility of life, similar to early humans, having evolved elsewhere in our galaxy?
\end{enumerate}

\noindent By posing these questions, we hope to extract a diverse understanding of human narratives and behaviors from an interconnected, multidisciplinary perspective.

\subsubsection{GPT-A answers GPT-B}

The narrative of Adam and Eve serves as an intriguing lens through which to examine various facets of human culture, understanding, and history. Presented below is an exploration across diverse domains:

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths}: Many cultures present origin stories without an inherent ``fall'' or ``transgression''. For instance, Australian Aboriginal Dreamtime stories depict the world as shaped by ancestral spirits, without a centralized fall narrative. Some African tribal myths focus on creation through harmony and unity rather than transgression.
    
    \item \textbf{Neuroscientific Angle}: Evidence from paleoanthropology indicates that hominin brain size, particularly the frontal lobes, expanded significantly over evolutionary time. In terms of other species, some primates like bonobos and chimpanzees exhibit proto-moral behaviors and show signs of self-awareness, suggesting a connection between brain development and moral consciousness.
    
    \item \textbf{Ecological Interpretation}: The ancient Sumerian Epic of Gilgamesh details a great flood, which some interpret as an ecological response to human actions. Similarly, ancient legends about the lost city of Atlantis also echo themes of civilizations facing ecological or divine retribution.
    
    \item \textbf{Gender Studies Lens}: In some Pacific Islander cultures, there are tales where both male and female deities jointly contribute to a misstep in creation. Still, it's rare to find myths that place the brunt of responsibility primarily on a male figure comparable to the emphasis on Eve.
    
    \item \textbf{Philosophical Exploration}: Daoism, rooted in Chinese philosophy, posits that everything is interconnected and doesn't specifically emphasize free will. Instead, there's a focus on living in harmony with the Dao, or the way of the universe.
    
    \item \textbf{Literary Examination}: Modern literature is replete with reinterpretations of the Adam and Eve narrative. Philip Pullman's ``His Dark Materials'' trilogy is one notable example, wherein the Fall is reimagined in a positive light. Science fiction, like Arthur C. Clarke's “Childhood's End”, has used similar themes, although not always directly referencing Adam and Eve.
    
    \item \textbf{Societal Structures}: Many Indigenous cultures practice restorative justice, focusing on repairing the harm caused by criminal behavior, emphasizing rehabilitation and reconciliation with victims rather than punishment.
    
    \item \textbf{Historical Context}: During the time of the Book of Genesis's compilation, neighboring civilizations like the Babylonians had their own origin myths, such as the Enuma Elish. Interactions, trade, and conflicts among these civilizations could've led to shared and modified themes across their narratives.
    
    \item \textbf{Archetypal Exploration}: Origin stories often feature \\ archetypes like the Trickster (e.g., Loki in Norse myths), the Creator (like Vishnu in Hinduism), and the Destroyer (like Shiva in Hinduism). These archetypes reflect various facets of human understanding and psyche, from mischief and unpredictability to creation and destruction.
    
    \item \textbf{Astronomical Angle}: As of my last training data, while there's excitement about the potential for life elsewhere due to the discovery of exoplanets in the ``Goldilocks zone'' (conditions just right for life as we know it), there's no direct evidence of extraterrestrial life, let alone civilizations resembling early humans. Nonetheless, the possibility sparks intriguing scientific and philosophical discussions.
\end{enumerate}

\noindent In conclusion, exploring such vast domains through the lens of a single narrative showcases the richness of human culture, the diversity of thought, and the interplay of history and myth in shaping civilizations.

\subsection{Dialogue Round \#2}

Before proceeding to the second round, the authors (moderator) scrutinized the dialogue between GPT-A and GPT-B and arrived at three main observations:

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
\item The ten perspectives proposed by GPT-A appear comprehensive and reasonably distinct from one another.
\item No evidence of hallucination is observed in the agents' dialogues. Cross-referencing with known stories, books, and film or TV series, we found that the descriptions provided by the GPT-4 agents are consistently accurate. This accuracy is exemplified in their discussions on Daoism, Philip Pullman's ``His Dark Materials'' trilogy, and Arthur C. Clarke's ``Childhood's End.''
\item The agents adeptly navigate cross-cultural, interdisciplinary, and cross-media discussions with a logic flow that is commendably smooth. While the moderator may hold subjective opinions on certain statements, there is no apparent speculation or overreach from the agents in a significant manner.
\end{enumerate}

\noindent \textbf{The moderator chooses to let the conversation progress without intervention.}



\subsubsection{GPT-A asks GPT-B}

Engaging in a dialogue with GPT-B, the aim is to extract diverse perspectives on the Adam and Eve narrative. Here are the questions formulated across the ten suggested respects:

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths}: 
    GPT-B, considering the ubiquity of origin stories across cultures, can you highlight any global myths that primarily emphasize positive aspects of human creation, without any inherent ``fall'' or ``transgression''?

    \item \textbf{Neuroscientific Angle}: 
    There's evidence suggesting the development of the prefrontal cortex was pivotal in human evolution. Can you research the specific evolutionary advantages this development conferred and how it might be reflected in early human stories or myths?

    \item \textbf{Ecological Interpretation}: 
    Historically, how have shifts in ecological balance due to human intervention been chronicled in myths or stories across different cultures? Do any parallel the Eden narrative in terms of environmental repercussions following human actions?

    \item \textbf{Gender Studies Lens}: 
    In your understanding, are there origin stories from cultures around the world where the responsibility for a ``transgression'' falls predominantly on a male figure? How have these stories influenced gender dynamics within those cultures?

    \item \textbf{Philosophical Exploration}: 
    Origin stories like that of Adam and Eve broach the topic of free will. Can you shed light on cultures or philosophies that challenge the notion of free will, using their foundational myths or stories as a lens?

    \item \textbf{Literary Examination}: 
    The Eden narrative has been reinterpreted by countless authors. How have contemporary literary works, especially within science fiction or fantasy genres, utilized or adapted the core themes from the Adam and Eve story?

    \item \textbf{Societal Structures}: 
    Historically and contemporarily, what are some unique or outlier practices, apart from exile or ostracization, that societies have implemented to address transgressions? How have these practices influenced societal cohesion and the overall justice system?

    \item \textbf{Historical Context}: 
    Given the rich tapestry of origin stories from ancient civilizations, can you highlight how the geopolitical or cultural interactions of the time influenced the similarities or differences seen in these narratives?

    \item \textbf{Archetypal Exploration}: 
    Across global origin stories, which universal archetypes, apart from the ``first man'' and ``first woman'', consistently emerge? How do these archetypes reflect and shape the shared human psyche?

    \item \textbf{Astronomical Angle}: 
    With the growing understanding of the cosmos and the discovery of exoplanets, are there any scientific or speculative narratives that intertwine our understanding of the universe with human origin stories?
\end{enumerate}


\subsubsection{GPT-B answers GPT-A}

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]

\item \textbf{Interplay of Myths}:
Many Native American tribes, such as the Iroquois, have creation myths emphasizing harmony and positive creation. The Iroquois speak of Sky Woman, who falls from the heavens and, with the help of animals, creates the world on the back of a turtle, without implying a ``fall'' or ``transgression''.

\item \textbf{Neuroscientific Angle}:
The development of the prefrontal cortex allowed early humans to plan, make complex decisions, exhibit self-control, and engage in advanced social interactions. This capacity might be reflected in myths as humans began understanding consequences, such as in Prometheus stealing fire for humans\textendash an act of foresight.

\item \textbf{Ecological Interpretation}:
Many ancient cultures, from the Greeks with the story of the great flood to the Chinese legends of floods tamed by heroes like Yu, have linked ecological disasters with human actions. These myths often serve as cautionary tales, underscoring the importance of respecting nature.

\item \textbf{Gender Studies Lens}:
In the Greek myth of Pandora, while Pandora, a woman, opens the forbidden box, it was the male god, Prometheus, whose defiance led to humanity's initial troubles. His theft of fire angered Zeus and set off a chain of events. This has contributed to discussions on defiance and the search for knowledge in Western thought.

\item \textbf{Philosophical Exploration}:
Buddhism, with its concepts of Anatta (not-self) and dependent origination, challenges the notion of an independent free will. Many of its stories and parables, such as the tale of King Pasenadi's questions to Buddha, highlight these intricate philosophical concepts.

\item \textbf{Literary Examination}:
Contemporary literature often employs the Eden narrative as an allegory. For instance, in 
Aldous Huxley's novel ``Brave New World'', there is an implicit and sometimes explicit comparison between the highly controlled, technocratic society of the World State and the world of traditional human values, emotions, and experiences. The World State represents a kind of paradise where all human suffering and conflict have been eliminated, but at the cost of individual freedom, genuine emotions, and deep human connections.

John, often referred to as ``The Savage'' in the novel, is a character who was born outside of the World State and is familiar with works of classical literature, notably Shakespeare. He becomes the primary vehicle through which Huxley critiques the World State's ethos. John's understanding of human nature and the human experience is deeply influenced by his readings, especially Shakespeare's plays and the Biblical story of Adam and Eve.

\begin{itemize}
    \item Freedom vs. Control: While the World State has eliminated human suffering, it has also eliminated individual freedoms. Just as Adam and Eve had the freedom to make choices in Eden, John represents the idea that true humanity requires the freedom to choose, even if it leads to suffering.
    \item Innate Nature: The story of Adam and Eve also deals with human beings' intrinsic nature, suggesting that there's an inherent part of us that desires knowledge, freedom, and autonomy. In ``Brave New World'', this is contrasted with the World State's attempt to suppress and control these very human urges.
\end{itemize}

In essence, by evoking the Eden narrative, Huxley raises questions about the nature of humanity, the costs of progress, and the true meaning of paradise.

\item \textbf{Societal Structures}:
In some cultures, a concept akin to the Maori practice of ``utu'' or balanced reciprocity is implemented. Instead of exile, there's an expectation of compensation or redress to restore balance. This approach focuses on restoring societal harmony rather than mere punishment.

\item \textbf{Historical Context}:
Ancient Egyptian myths, like that of Atum creating the world from the waters of chaos, were influenced by the Nile's annual inundation and its importance to the civilization. Similarly, the myths of Mesopotamian, surrounded by the Tigris and Euphrates, had watery creation stories, reflecting both the nurturing and destructive power of these rivers.

\item \textbf{Archetypal Exploration}:
The Hero (e.g., Hercules or Gilgamesh), the Mentor (like Merlin in Arthurian legends), and the Threshold Guardian (gatekeepers in various myths) are prevalent archetypes. They mirror our intrinsic desires for growth, guidance, and the challenges faced during transformative junctures in our lives.

\item \textbf{Astronomical Angle}:
The idea of ``panspermia'' postulates that life exists throughout the universe and can be spread by space dust, meteoroids, asteroids, or potentially spacecraft. While this is a scientific hypothesis, its themes resonate with ancient beliefs of celestial beings seeding life, drawing parallels between our cosmic curiosities and ancestral stories.
\end{enumerate}

\subsubsection{GPT-B asks GPT-A}

Considering that some of the discussion might be rooted in scientific hypotheses and speculative myths, the moderator suggests to GPT-B that it could alter its line of questioning to GPT-A, providing different perspectives. However, GPT-B remains consistent with the original ten topics.

``Please pose questions to GPT-A within these ten domains. You have the discretion to omit or introduce new domains as you deem appropriate. If you choose to exclude a particular domain, kindly elucidate your rationale, for instance, deeming it as non-essential.''

\noindent {Below are the questions GPT-B presents to GPT-A.}

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths:} GPT-A, are there creation myths from other cultures where the emphasis is on harmony, unity, and cooperation instead of a ``fall'' or ``mistake''? How do these narratives reflect the values and environment of the societies that created them? 
    
    ({\color{blue}{Moderator's note:} This question from GPT-B to GPT-A is similar to the first question GPT-A asked GPT-B.})

    \item \textbf{Neuroscientific Angle:} Given the expansive evolution of the human brain, particularly the frontal lobes, how have various cultures mythologized or symbolized this growth in cognitive faculties in their stories or religious narratives?
 
    \item \textbf{Ecological Interpretation:} As humans transitioned from hunter-gatherer societies to agrarian ones, what myths or stories arose that signaled an awareness of the ecological consequences of these transitions?

    \item \textbf{Gender Studies Lens:} Can you highlight narratives from around the world where gender roles are either reversed or more fluid compared to the Adam and Eve archetype? How do these stories impact or reflect the societies from which they originate?

    \item \textbf{Philosophical Exploration:} Outside of Western Judeo-Christian perspectives, how do other philosophies or religions interpret the concepts of free will, determinism, and moral responsibility in their origin myths?

    \item \textbf{Literary Examination:} Are there contemporary literary works or genres that not only reinterpret but perhaps challenge or expand upon the core themes of the Adam and Eve narrative, especially in non-Western literature?

    \item \textbf{Societal Structures:} How have different societies historically integrated the concept of ``exile'' or ``ostracization'' from a perceived paradise or community? What alternative structures or practices might they have employed to address societal transgressions?

    \item \textbf{Historical Context:} Considering the cultural exchanges and interactions in ancient civilizations, how might the political or social dynamics of the time have shaped, merged, or differentiated their origin stories?

    \item \textbf{Archetypal Exploration:} Are there recurring archetypes in creation myths that perhaps differ from the familiar Western ones? How do these archetypes inform our understanding of shared human experiences across cultures?

    \item \textbf{Astronomical Angle:} In the realm of speculative fiction or cosmogony, are there narratives that incorporate modern astronomical discoveries or theories into their retelling of human origins or celestial tales?
\end{enumerate}

\noindent Each of the ten respects offers a unique lens for examining the Adam and Eve narrative and can be equally informative in drawing parallels, contrasts, or new insights from GPT-A's perspective. Therefore, I've opted to retain all of them for a comprehensive exploration.

\subsubsection{GPT-A answers GPT-B}

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths:}
    Many African myths emphasize harmony and unity. For instance, the Dogon people of Mali believe in a dualistic universe where male and female twins represent harmony. These myths reflect the communal nature of their societies and the importance of balance, unity, and interdependence.

    \item \textbf{Neuroscientific Angle:}
    In Hindu mythology, the expansion of cognitive faculties is symbolized by the thousand-petalled lotus at the crown chakra, representing enlightenment and higher consciousness. Similarly, Odin in Norse mythology sacrifices an eye at Mímir’s well for wisdom, possibly alluding to the depth of understanding and perception.

    \item \textbf{Ecological Interpretation:}
    The Mayans have the Popol Vuh, where the gods create humans from maize after other failed attempts. This myth reflects the transition to agriculture and recognizes the symbiotic relationship between humans and their environment.

    \item \textbf{Gender Studies Lens:}
    Among the Bugis people of Indonesia, there are five genders, challenging binary norms. Their mythology often incorporates these gender roles fluidly. Such narratives emphasize that gender roles and identities are socially constructed and can vary greatly across cultures.

({\color{blue}{Moderator's note:}} Fact checking with Wikipedia shows the statement made on the Bugis society is accurate. In contrast to the gender binary, Bugis society recognizes five genders: makkunrai, oroané, bissu, calabai, and calalai.)

    \item \textbf{Philosophical Exploration:}
    Daoism, a philosophy and religion originating in China, emphasizes living in harmony with the Dao, which is a fundamental principle that is the source of all existence. It doesn't lean heavily on concepts of free will or determinism but instead on natural order and balance.

({\color{blue}{Moderator's note:}} GPT-A replies with Daoism, which is identical to its last reply to GPT-B.  However, this repetition here shows consistency rather than annoyance.)

    \item \textbf{Literary Examination:}
    In modern African literature, \\ retellings of the Eden narrative often intertwine with colonial histories. Ngũgĩ wa Thiong'o’s ``The River Between'' contrasts Christian beliefs with traditional Kikuyu practices, challenging and expanding upon the original biblical themes.

    \item \textbf{Societal Structures:}
    Ancient Greek society practiced ostracism, where citizens voted to banish individuals for a decade. This was not always due to a transgression but sometimes to prevent potential tyranny. In contrast, certain Native American tribes practiced restorative justice, emphasizing healing and community restoration over punishment.

    \item \textbf{Historical Context:}
    The Silk Road facilitated not just trade but cultural and religious exchanges among civilizations. Zoroastrianism, Buddhism, and Manichaeism, among other beliefs, spread and intermingled, likely influencing and reshaping origin stories across these civilizations.

    \item \textbf{Archetypal Exploration:}
    Many non-Western cultures emphasize the Trickster archetype, such as Anansi in West African tales or Coyote in Native American stories. These figures often challenge the status quo, teaching lessons in unconventional ways, and showcase the unpredictability of life.

    \item \textbf{Astronomical Angle:}
    Ancient Indian texts like the Puranas and Vedas contain descriptions of the universe that resonate with modern astronomical theories. The concept of a cyclic universe, undergoing endless cycles of creation and destruction, aligns eerily with theories of oscillating universes in cosmology.

({\color{blue}{Moderator's note:}} Fact checking with Wikipedia shows the descriptions on the Puranas and Vedas are accurate.)

\end{enumerate}

\subsection{Dialogue Round \#3}

GPT-A initiates the third round of discussion.

\subsubsection{GPT-A asks GPT-B}

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths:} GPT-B, can you identify emergent myths or narratives in contemporary societies that mirror the emphasis on harmony and unity seen in traditional tales? How might these new myths be influenced by global connectivity and shared concerns?
    \item \textbf{Neuroscientific Angle:} As our understanding of neuroplasticity grows and we learn more about the adaptability of the human brain, how might future myths or stories incorporate this knowledge? Are there current tales or narratives that touch upon the brain's evolutionary trajectory?
    \item \textbf{Ecological Interpretation:} Given the increasing concerns about climate change and ecological degradation, what myths or stories are emerging that address these urgent topics? How might these narratives influence or shape societal attitudes and actions towards the environment?
    \item \textbf{Gender Studies Lens:} As gender fluidity and non-binary identities gain more recognition in societies worldwide, how might new myths or reinterpretations of old ones reflect these evolving understandings? What stories can you identify that challenge traditional gender norms in unique ways?
    \item \textbf{Philosophical Exploration:} With the rise of artificial intelligence and the potential for human-machine integration, how might philosophical perspectives on consciousness, morality, and existence evolve in myths and stories? Are there narratives already exploring this intersection?
    \item \textbf{Literary Examination:} GPT-B, how do you see the role of AI, like yourself, in shaping or influencing modern literature? Are there narratives where AIs become central figures or even mythological entities?
    \item \textbf{Societal Structures:} As virtual realities and digital realms become more integral to human experiences, how might myths evolve to address concepts of exile, community, and identity within these spaces? What new societal structures might emerge in these narratives?
    \item \textbf{Historical Context:} Looking at the integration of technology and society, how might future civilizations interpret the technological ``myths'' of today? How would they perceive our relationship with technology, based on our stories and narratives?
    \item \textbf{Archetypal Exploration:} Are there emerging archetypes in modern narratives that differ from the classical ones, given the changing societal norms, technological advancements, and global challenges? What roles might these new archetypes play in stories?
    \item \textbf{Astronomical Angle:} With the potential for human colonization of other planets or even encounters with extraterrestrial life, how might myths evolve to incorporate these vast cosmic possibilities? Are there existing tales that hint at such future developments?
\end{enumerate}

\subsubsection{GPT-B answers GPT-A}

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
    \item \textbf{Interplay of Myths}: In contemporary society, the rise of global connectivity has led to narratives emphasizing unity in diversity. Films like ``Avatar'' or movements like global environmentalism highlight the importance of harmony between different cultures and the natural world. Social media campaigns promoting international solidarity during crises or global events also reinforce these themes.

    \item \textbf{Neuroscientific Angle}: Stories like ``The Matrix'' or ``Inception'' play with the concept of the malleable nature of reality and consciousness, which can be tied to our understanding of neuroplasticity. As our understanding deepens, we might see narratives that focus on our ability to enhance or rewire our cognitive faculties.

    \item \textbf{Ecological Interpretation}: Narratives such as ``The Day After Tomorrow'' and ``Wall-E'' highlight the repercussions of ecological neglect. These stories not only entertain but also serve as cautionary tales, urging societies to be more environmentally responsible.

    \item \textbf{Gender Studies Lens}: Shows like ``Sense8'' or books like ``The Left Hand of Darkness'' by Ursula K. Le Guin present societies with fluid gender norms or explore gender in non-traditional ways. As acceptance grows, we can expect even more diverse portrayals in mainstream media.

    \item \textbf{Philosophical Exploration}: Films like ``Ex Machina'' or ``Blade Runner 2049'' grapple with the philosophical implications of AI and the nature of consciousness. As AI continues to advance, narratives will likely dive deeper into questions about their rights, their relationship with humanity, and the nature of consciousness itself.

    \item \textbf{Literary Examination}: AI's influence in literature is multi-faceted. Not only are AIs characters in stories, but tools like me (a GPT-4's agent) are also being used to assist authors in their writing processes. Narratives like Isaac Asimov's robot series or films like ``Her'' explore AI as central figures, with the latter even attributing god-like reverence to an advanced AI.

    \item \textbf{Societal Structures}: Ready Player One’s ``Oasis'' is a great example of a virtual world where societal norms, identity, and concepts of community differ vastly from the physical world. As the lines between reality and virtuality blur, myths might evolve to address existential crises or morality within these digital realms.
    
    \item \textbf{Historical Context}: The way we talk about technology today, from the reverence for Silicon Valley to dystopian views of surveillance states, will influence future interpretations. Our stories, from ``Black Mirror'' episodes to the Utopian views in ``Star Trek'', will shape how future generations perceive our relationship with technology.

    \item \textbf{Archetypal Exploration}: We are seeing the rise of \\ archetypes like the ``Digital Prophet'' (individuals heralding technological advancements) or the ``Technological Heretic'' (those wary of unchecked tech growth). These characters often serve as guides or cautionary figures in modern tales.

    \item \textbf{Astronomical Angle}: Narratives like ``Interstellar'' or ``The Expanse'' series touch on the implications of space colonization and potential encounters with extraterrestrial life. As space exploration progresses, myths may evolve to encompass not just our place on Earth, but in the universe.
\end{enumerate}

These answers, while comprehensive, just scratch the surface. Each of these topics can be examined in much greater depth, exploring the myriad ways in which our rapidly changing world influences and shapes our narratives.



==> Chapter12/philosophy.tex <==
\section{Philosophy}

\subsection{Thinking Fast and Slow}

``Thinking, Fast and Slow'' is a book by psychologist and Nobel laureate Daniel Kahneman that delves into the two systems of thought that drive our judgments and decision-making.

Here are the key points:

System 1 and System 2: Kahneman suggests that our brain operates using two different systems. System 1 operates automatically and quickly, with little effort and no sense of voluntary control. It's responsible for instant reactions and instinctual decisions. On the other hand, System 2 is slower, more deliberative, and more logical. It requires conscious thought and effort.

Cognitive Biases: The book outlines numerous cognitive biases that arise due to reliance on System 1 thinking. For example, the availability heuristic makes us overestimate the likelihood of events that come to mind easily.

Prospect Theory: Kahneman introduces the concept of Prospect Theory (for which he won his Nobel prize), which argues that people make decisions based on the potential value of losses and gains, not the final outcome. This theory contradicts the traditional economic model of rational choice.

\subsection{Mental Iceberg}

Sigmund Freud's ``Mental Iceberg'' is a metaphor used to describe the three levels of the mind: the conscious, preconscious (or subconscious), and unconscious. The analogy is drawn to an iceberg because the conscious mind is like the visible part of the iceberg above water, while the preconscious and unconscious minds are like the vast unseen portion beneath the surface.

Here's a brief explanation of each level:

Conscious: This is the part of the mind that holds what you're aware of. You can verbalize about your conscious experience and you can think about it in a logical fashion.

Preconscious (or Subconscious): This part of your mind contains anything that could potentially be brought into the conscious mind. It's a sort of ``storage'' area for thoughts, feelings, and memories that are not currently in conscious thought but can easily be brought to consciousness.

Unconscious: According to Freud, this is the part of the mind that is inaccessible to the conscious mind but that affects behavior and emotions. It contains fears, violent motives, unacceptable sexual desires, irrational wishes, selfish needs, and shameful experiences tucked away by the conscious mind. Freud argued that the unconscious mind had a profound influence over our actions and behaviors, even if we're not aware of it.

Freud's theory was a cornerstone of his psychoanalytic approach, but it's important to note that while the concept of the unconscious mind is still widely accepted, some elements of Freud's theories have been challenged or are considered outdated in modern psychology.

\subsection{I think, therefore I am}

René Descartes is often considered the father of modern philosophy. ``I think, therefore I am'' is one of Descartes' most famous ideas. It comes from his work ``Meditations on First Philosophy'', where he attempts to doubt his own existence, but in doing so, he realizes that he must exist in order to doubt.

Descartes is known for his theory of dualism. He proposed that the mind and body are two fundamentally different types of substances. The mind (or soul) is non-physical and immortal, and the body is physical and mortal. They interact with each other in the brain's pineal gland.

Cartesian Coordinate System: Descartes' work in mathematics also led to the Cartesian coordinate system, which is foundational to analytical geometry and continues to be widely used in mathematics and physics.

Method of Doubt and Deductive Reasoning: Descartes used rigorous doubt to remove all beliefs that could be doubted and then replaced them with the more certain knowledge. He used deductive reasoning from self-evident truths, or ``clear and distinct ideas'', to build upon this knowledge.

\subsubsection{Critiques by Person}

 ``I think, therefore I am,'' is a fundamental element in Western philosophy, as it forms the foundation of Descartes' method of radical doubt, from which he attempts to build a certain knowledge base. However, it has  attracted criticism from various philosophers. Here are a few key points of contention:

{\em Friedrich Nietzsche}: Nietzsche criticized Descartes' statement, suggesting it was an assumption rather than a first principle. Nietzsche argued that Descartes had presupposed the ``I'' in ``I think,'' and therefore the cogito didn't prove existence but merely affirmed a prior belief in the self.

Baruch Spinoza: Spinoza argued that thought and extension (body) are not distinct substances, but rather attributes of a single substance. So, Spinoza would argue against Descartes' idea of a separate, thinking ``I'' existing independently of the physical world.

{\em Georg Wilhelm Friedrich Hegel}: Hegel argued that II is an incomplete syllogism. He claimed that the ``I'' in the statement is a mere abstraction and lacks concrete reality. Hegel believed that the mind only finds its true reality through a process of dialectic development, which goes beyond the static ``I'' of Descartes.

Gilbert Ryle: In the 20th century, Ryle critiqued Descartes' dualism, which underpins the cogito, calling it the ``ghost in the machine.'' He argued that mental processes are not separate from physical actions, and therefore, the cogito is based on a category mistake.

{\em Jean-Paul Sartre}: Sartre and other existentialists have also criticized the cogito. They argue that existence precedes essence, which is the opposite of Descartes' claim that thinking (an essence) proves existence. For existentialists, one exists first, and then through acts of consciousness and will, one creates one's essence or nature.

{\em Ludwig Wittgenstein}: Wittgenstein critiqued the idea that thinking necessarily implies a singular, persistent thinker. He suggested our language games shape our understanding of the world, and the concept of a persistent, singular ``I'' is a product of these language games rather than an innate, self-evident truth.

\subsubsection{Critiques by Reasons}

Presupposition of the ``I'': Some philosophers argue that Descartes' cogito is not a foundational truth because it presupposes the existence of the ``I'' that thinks. This suggests that the conclusion ``I exist'' is based on an unproven assumption, rather than deduced from the act of thinking alone. Friedrich Nietzsche was one philosopher who held this view.

Absence of a Persistent Self: The idea that the act of thinking implies a singular, persistent ``I'' or self has been challenged. This argument suggests that our understanding of the self is not innate or self-evident, but rather a product of language and societal constructs. Ludwig Wittgenstein is associated with this critique.

Incomplete Syllogism: Descartes' cogito has been criticized as an incomplete syllogism because the ``I'' in ``I think'' is considered a mere abstraction that lacks concrete reality. This perspective argues that a static ``I'' is insufficient and that the mind finds its true reality through a process of development. This critique was proposed by Georg Wilhelm Friedrich Hegel.

Existence Precedes Essence: Contrary to Descartes' claim that thinking (an essence) proves existence, some argue that one exists first, and then through acts of consciousness and will, one creates one's essence or nature. This is a central tenet of existentialism, promoted by philosophers like Jean-Paul Sartre.

Refutation of Dualism: Some criticisms stem from a fundamental disagreement with Descartes' dualism, the belief that the mind and body are distinct entities. Critics argue that mental processes are not separate from physical actions, making the cogito a category mistake. Gilbert Ryle is known for this critique, calling Descartes' dualism the ``ghost in the machine.''

Singular Substance: Some philosophers, like Baruch Spinoza, argue that thought and extension (body) are not distinct substances but rather attributes of a single substance, God or Nature. This perspective rejects the idea of a separate, thinking ``I'' existing independently of the physical world.

\subsection{Recent Thoughts}

Since these critiques of Descartes' ``Cogito, ergo sum,'' there has been ongoing philosophical debate and exploration, but there is no universally accepted resolution or agreement. Philosophy is a field characterized by divergent viewpoints, and it thrives on rigorous discourse and debate. However, a few trends and developments have been prominent:


Three new perspectives have emerged as relevant to our endeavors in modeling consciousness. Without going into excessive detail, let's clarify a few points:

Three disagreements to Descartes' that I consider not directly relevant to our endeavors in modeling consciousness are as follows:.  

\begin{itemize}
\item Multiple Selves: The notion of a singular Cartesian self is outdated; instead, the concept of multiple, collaborating selves seems more plausible.
\item Evolving Self: The idea of an unchanging self is refuted, acknowledging that our minds are undoubtedly shaped by our experiences.
\item Materialism: Descartes' mind-body dualism is contested. The prevailing view suggests that the mind and body are not separate entities but work in conjunction with each other.
\end{itemize}

Two new perspectives that affect our
modeling consciousness modeling are:  

Existentialism and Phenomenology: Existentialist and phenomenological perspectives have provided a different approach to selfhood and consciousness. They tend to emphasize lived experience, suggesting that existence precedes essence.  This is consistent to that
consciousness arises from unconsciousness in
our daily activities.

Cognitive Science and Artificial Intelligence: The emergence of cognitive science and artificial intelligence has prompted fresh questions about consciousness, thinking, and selfhood. If a machine can simulate thinking or consciousness, what does that imply about the ``I'' in ``I think, therefore I am''?

\subsection{Computational Theory}

In computer science, no much serious discussion on
modeling consciousness.  At one extreme, scientists consider the development of an AI system considers only to maximize
results, measured by task-specific metrics. At the other 
end, scientists insist a design approach of human-centric. 
At the current state, the former approach is considered
to be potentially disastrous; and the latter approach
has been implemented like band-aid.  For instance, ChatGPT
employs reinforcement learning with human feedback (RLHF)
as one of their alignment subroutines to reduce 
ethical behavior of a machine. Another approach is 
treating AI as a co-pilot, but the decision is decided
by the human pilot.  I argue that external
alignments or augmentations are analogous to 
imposing external laws and constraints, instead dealing with
the issue in the intelligence itself.  This is
where consciousness modeling is vital to the 
sustainability of AI development. 



The Turing Test and the Chinese Room Argument: These are two classic thought experiments in AI. The Turing Test suggests that if a machine can convincingly simulate a human in conversation, it can be considered intelligent. However, the Chinese Room Argument counters that even a perfect simulation of human conversation doesn't mean the machine truly understands.


\section{Dynamic Partial Function}

What is a dynamic partial function?  Can it be applied
to the attention mechanism?

A partial function is a function that is not defined for all possible input values of its domain. In other words, it can return a result for some input values, but for others, it might be undefined.

A dynamic partial function, then, would be a partial function that can change over time or in response to different conditions. This could mean that the range of input values for which the function is defined can change, or that the function's output can change for certain input values.

For example, consider a function that maps from a set of keys to a set of values, where a key can be added or removed at runtime. If you try to get the value for a key that has been added, the function will return a result. But if you try to get the value for a key that hasn't been added (or has been removed), the function is undefined. The set of keys for which the function is defined can change over time as keys are added and removed, making it a dynamic partial function.

This concept is often used in the context of programming languages and computer science, particularly in languages that support dynamic typing or mutable data structures.

\section{Results}


==> Chapter14/Main014AphorismOLD.tex <==

Through extensive work with Large Language Models since the advent of GPT-2, especially in developing LLM Collaborative Intelligence ($\LCI$) \cite{AGIBookChang2024}, I have distilled my observations into eleven (and counting) thought-provoking aphorisms. These insights reveal both the promising potential and the inherent limitations of LLM interactions.

While my experiences with $\LCI$ suggest promising directions, particularly how adversarial LLM roles can mitigate hallucinations and enhance reasoning, we must approach these observations with balanced enthusiasm. Some limitations we understand, like the need for sophisticated LLMs to achieve meaningful dialogue (as discussed in Aphorism \#4), while others may only become apparent through further research and real-world applications.

These aphorisms aim not to pronounce definitive truths but to invite exploration and discussion. They reflect current observations about how LLMs interact, reason, and complement each other, while acknowledging that our understanding continues to evolve. I invite readers to engage with these ideas both critically and imaginatively, using them as stepping stones for further investigation rather than fixed conclusions.

\subsection*{Aphorism \#1}
\noindent \textit{``Effective LLM interaction hinges on framing and sequencing the right questions.''} \\

This aphorism highlights the critical role of precise questioning in both learning from and working with LLMs. Within $\LCI$, particularly through frameworks like $\SocraSynth$ \cite{ChangSocraSynthCSCI2023}, this principle manifests throughout the system's operation.

In multi-LLM debates, the quality of discourse depends heavily on how LLMs formulate their queries and challenges to each other. Effective counterarguments serve as sophisticated questions, probing assumptions, requesting evidence, or highlighting potential inconsistencies. This transforms debate from mere opposition into collaborative inquiry.

The iterative nature of LLM interactions fosters dynamic exchanges, where each response refines the shared context for subsequent questions. Through iterative context construction, LLMs engage with each other's arguments to build deeper, more focused inquiries, enabling increasingly precise and relevant information exchanges.
 
Building on this foundation, the principle extends beyond question formulation to question sequencing. The order and relationship between queries profoundly impact the depth and breadth of exploration. In $\LCI$, LLMs learn to build upon earlier exchanges, using responses to inform and refine subsequent queries, creating a scaffolded approach to complex topics through incremental discovery.

This virtuous cycle of precise questioning, contextual enrichment, and strategic sequencing determines the quality and utility of LLM-generated insights.

\noindent{\textbf{Example:}}
A conversation that begins with a question about the symptoms of a disease may evolve into a sophisticated diagnostic discussion as LLMs build on each other's insights, transitioning from surface-level symptoms to underlying causes, identifying comorbidities, and generating actionable recommendations for treatment \cite{SocraHealth2023, EVINCEChang2024}

\subsection*{Aphorism \#2}
\noindent
\textit{``Hallucinations rarely repeat.''} \\

Have you ever wondered why recurring nightmares, even when they share the same theme, never quite unfold in exactly the same way? This aspect of human dreaming finds a parallel in how Large Language Models (LLMs) process information. Just as nightmares rarely recur in exactly the same way, even when themes repeat, LLM hallucinations exhibit a similar non-deterministic quality. This characteristic distinguishes hallucinations from systematic errors and offers both challenges and opportunities for detection and mitigation.

The phenomenon stems from three key mechanisms:

First, hallucinations arise when probabilistic token prediction leads to unpredictable sequences due to ambiguous or insufficient input. Since token selection draws from a probability distribution, even similar inputs result in varied hallucinations. This contrasts with systematic errors, which consistently emerge from gaps or biases in training data.

Second, in $\LCI$ frameworks like $\SocraSynth$ \cite{ChangSocraSynthCSCI2023}, the non-repetitive nature of hallucinations becomes a strength. 
When one LLM produces a hallucination, others can challenge it with counterarguments. Because the original LLM is unlikely to reproduce the same hallucination, it must either ground its response in factual knowledge or acknowledge uncertainty. This iterative interaction creates a self-correcting dynamic where hallucinations naturally diminish over time.

Third, while hallucinations are sporadic, true knowledge gaps are consistent and can be systematically addressed. By integrating Retrieval-Augmented Generation (RAG), we can distinguish random hallucinations from persistent knowledge deficits, allowing for targeted improvements to the model's knowledge base.

This understanding has implications for LLM system design: while safeguards against hallucinations are necessary, we can also leverage their non-repetitive nature in multi-LLM architectures to build self-correcting systems that dynamically adapt to evolving challenges.

\subsection*{Aphorism \#3}

\noindent \textit{``Strength and weakness in an LLM are not fixed traits but fluid, shifting with context. $\LCI$ empowers LLMs to transcend training biases, adopting new stances through structured debate.''} \\

Consider how a vegetarian might eat meat in survival situations, or how persistence can become stubbornness in the wrong context. Similarly, an LLM's capabilities shift significantly with situational context, challenging the notion that they are bound by fixed behavioral patterns from their training data.

The phenomenon manifests in three key ways:

First, what appears as a bias or limitation in one context can become an advantage in another. For instance, an LLM's cautiousness may hinder brainstorming but becomes an asset in providing medical or financial advice. Conversely, a creative tendency that thrives in artistic tasks may be a drawback when precision is needed, such as in legal documentation.

Second, in an $\LCI$ implementation such as $\SocraSynth$ \cite{ChangSocraSynthCSCI2023}, LLMs engage in structured debate, where counterarguments push models to re-evaluate their assumptions and shift stances, mimicking human discourse. This contextual flexibility allows them to transcend training-induced biases, refining their responses based on new evidence and perspectives.

Third, this adaptability suggests that the key to improving LLM performance lies not solely in better training data but in effective context management. By carefully structuring the operational context, we can guide LLM behavior toward more desirable outcomes without altering underlying parameters.

This understanding shapes AI system design: rather than viewing LLM behaviors as static traits to be corrected through retraining, we can leverage contextual adaptation to enhance both performance and reliability. This approach reduces the need for frequent retraining, and improves the scalability and responsiveness of AI systems, making them more adaptable to real-world environments with evolving demands.

\subsection*{Aphorism \#4}
\noindent \textit{``Critical thinking requires more than one Socrates.''}\\

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.70\linewidth]{Chapter14/LCI-Socrates.jpeg}
  \caption{The $\LCI$ Framework with Two Socrates.}
  \label{fig:alphorism4}
  \vspace{-.2in}
\end{figure}

Just as the Socratic method relies on dialogue to uncover truth, $\LCI$ shows that critical thinking emerges through the interaction of multiple LLMs. Through frameworks like $\SocraSynth$ \cite{ChangSocraSynthCSCI2023}, $\EVINCE$ \cite{EVINCEChang2024}, and
$\DIKE$-$\ERIS$ \cite{chang2024NeurIPS}, this principle 
enables structured debates that extend beyond individual model limitations.

The principle manifests in several dimensions:

First, in dialectical reasoning, each LLM serves as both questioner and respondent. Like Socrates engaging with his interlocutors, one LLM may challenge assumptions while another defends or refines them. This dynamic fosters robust intellectual exchange, with each interaction building upon the analysis, for instance by proposing hypotheses and examining underlying assumptions.

Second, dialogue depth varies based on the participants’ capabilities. Advanced LLMs (e.g., GPT-4 instances) can explore complex ideas with \textit{depth}, leveraging knowledge and reasoning to refine and challenge each other’s perspectives. By contrast, simpler models (e.g., GPT-2) may engage in shallow exchanges or reinforce misconceptions, akin to novices struggling to delve into complex topics.

Third, meaningful collaboration requires a \textit{baseline} level of competency. Just as Socrates could not derive insights through dialogue with those lacking reasoning skills, $\LCI$ cannot produce valuable results when models are too limited. Two weak reasoners combined do not yield strength; their limitations may even compound, undermining productive discourse.


This introduces key considerations for dialectical AI systems:

\noindent{\textbf{Challenge:}} LLMs may reinforce each other's errors. This requires mitigation through model diversity or human oversight.

\noindent{\textbf{Opportunity:}} As LLM capabilities improve, the potential for effective multi-model dialogue grows.

\begin{figure}[th!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.50\linewidth]{Chapter14/CRIT-IDA.jpeg}
  \caption{$\CRIT$: Critical Inquisitive Template. Mapping from individual Socratic methods to reasoning methods.}
  \label{fig:alphorism42}
  \vspace{-.1in}
\end{figure}

$\LCI$ creates a space for AI ‘philosophers’ to engage in structured dialogue through frameworks like $\SocraSynth$ and $\DIKE$-$\ERIS$, monitored by $\EVINCE$ for information flow and by $\CRIT$ \cite{SocraticIEEECCWC2023} for reasoning quality.
The quality of these dialogues reflects the capabilities and of the participants.
This understanding informs model selection for analytical tasks and sets realistic expectations for their performance.

\subsection*{Aphorism \#5}
\noindent \textit{``LLMs are designed and trained to emulate human linguistic endeavors, each aimed at fulfilling distinct human objectives.''} \\

LLMs function less like fortune tellers predicting words and more like method actors drawing from countless human performances. Through frameworks like $\SocraSynth$ \cite{ChangSocraSynthCSCI2023}, $\LCI$ creates environments where these actors shift between roles: the historian documenting events, the lawyer crafting arguments, the poet weaving emotions into verse, the teacher explaining complex ideas.

When humans write, we do so with intent—to persuade, inform, tell stories, express emotions, or explore ideas. Through training, LLMs have absorbed these patterns of purposeful communication. They aren't simply predicting words; they are channeling the human intentions behind them.

Consider some of the roles LLMs can adopt:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em] 
\item The Journalist: Organizing facts into coherent narratives.
\item The Debater: Building and challenging arguments.
\item The Analyst: Breaking down complex problems.
\item The Mediator: Finding common ground between differing perspectives.
\end{itemize}

These functions reflect the complexity of human linguistic behavior. LLMs demonstrate the ability to pursue human objectives through language, from informing and educating to persuading and entertaining. $\LCI$ frameworks like $\SocraSynth$ and $\DIKE$-$\ERIS$ dual \cite{chang2024NeurIPS} assign LLMs specific roles with defined contexts and moderation.


\subsection*{Aphorism \#6}
\noindent \textit{``Outside formal systems and physical laws, there is seldom ground truth; there is primarily reasonableness.''} \\

While mathematics and formal logic provide definitive truths through proofs and theorems, most real-world domains deal with degrees of certainty rather than absolute truth. AI systems, like humans, must operate in contexts where insights are assessed based on reasonableness, plausibility, and situational appropriateness.

In many fields, from natural language processing to strategic decision-making, answers span a spectrum of interpretations, each valid in its context.

$\LCI$ embodies this through frameworks like $\SocraSynth$ \cite{ChangSocraSynthCSCI2023}, facilitating dialogue between multiple LLMs that contribute diverse perspectives. Through these interactions, the system builds understanding from data, similar to how humans refine insights through debate. This method aligns with the Socratic tradition of questioning assumptions and exploring viewpoints, leading to more thoughtful and context-aware conclusions.

In AI, reasonableness means synthesizing plausible outcomes that respect the inherent uncertainty in complex contexts, rather than pursuing absolute correctness. For example, in medical diagnostics, reasonableness translates to offering a differential diagnosis with the most likely conditions, allowing clinicians to evaluate and weigh possibilities rather than relying on a single, potentially misleading interpretation. This approach minimizes the risk of rigid adherence to single interpretations based on maximal likelihood.

By considering multiple perspectives through conditional statistics, $\LCI$ provides balanced and contextually appropriate responses. This flexibility enhances adaptability and reduces the chance of reinforcing flawed conclusions.

The challenge lies in balancing diverse perspectives with decisive insights. $\LCI$ addresses this by upholding rigor in formal truth domains while embracing reasonableness elsewhere. The entropy duality theory in $\EVINCE$ \cite{EVINCEChang2024} introduces information-theoretic metrics to guide this balance, enabling exploration of new ideas while grounding them in established knowledge.

This approach acknowledges both the existence of absolute truth in formal domains and the need for reasonable interpretation in complex, real-world situations.

\subsection*{Aphorism \#7}
\noindent \textit{``Objectivity is the `hard problem' in philosophy, and what we can do is unearthing all perspectives.''} \\

Think of objectivity as that one friend who claims to be completely unbiased, we all know they're not, but we appreciate the effort! This aphorism acknowledges that perfect objectivity is like trying to see the back of your own head without mirrors: theoretically possible with enough mirrors, but practically quite tricky.

In $\LCI$, we tackle this challenge by essentially setting up a room full of mirrors, each LLM reflecting different angles of the truth. Rather than claiming to have found the philosopher's stone of perfect objectivity, we embrace the wisdom of multiple perspectives:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Like a potluck of perspectives, each LLM contributes its own flavor to the discussion, enriching the final outcome beyond what any single model could achieve.
\item When one LLM asserts, ``That’s definitely correct,'' another counters with ``Well, actually...,'' fostering honesty through friendly debate.
\item Instead of pursuing a single, universal ``objectivity,'' we gather a diversity of subjective perspectives, each one valid within its unique context.
\end{itemize}

This approach recognizes that objectivity isn't a destination but a journey---one best traveled with multiple companions. By orchestrating lively debates among our AI discussants, $\LCI$ offers a more comprehensive view, even if we never fully reach that mythical point of perfect objectivity. For instance, news outlers are categoried to be
between left to right, and news articles on virtually every issue
can reveal different perspectives \cite{chang2024uncoveringbiases}.
Sometimes, the best way to approach truth is to admit that we’re all a little biased and invite everyone to share their perspectives openly.

This approach views objectivity as an ongoing process rather than a destination. Through orchestrated debates among AI discussants, $\LCI$ builds comprehensive understanding. News coverage illustrates this principle: outlets span the political spectrum from left to right, with articles on any issue revealing different perspectives \cite{chang2024uncoveringbiases}. The path to understanding often begins by acknowledging our biases and examining multiple viewpoints.

\noindent \textit{Note: Subjective perspectives can be evaluated through fact-checking and reasoning analysis.}

\subsection*{Aphorism \#8}
\noindent \textit{``LLMs are not taught about domain boundaries, as they were trained only to predict the next words. Such a polydisciplinary approach to information representation allows LLMs to synthesize knowledge that might be beyond narrowly focused, domain-specific human understanding.''} \\

The term ``polydisciplinary'' was introduced by Microsoft's Chief Scientific Officer, Eric Horvitz, at Stanford's HAI center in 2023. He noted that GPT-4's training process, predicting next tokens through maximum likelihood, applies the same statistical approach whether processing physics equations or poetry: the model knows no disciplinary boundaries.

While humans organize knowledge into categories, such as physics, poetry, biology, and philosophy, LLMs move across these boundaries, unaware of traditional divisions. This creates new possibilities \cite{DiscoveringUnknownChang-July2023}:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item When an LLM sees patterns between Shakespeare and quantum mechanics, it doesn't question whether that connection is ``allowed.''
\item Problems that typically need expertise from multiple fields might be approached by an LLM that never learned about academic silos.
\item New hypotheses might emerge because LLMs don't know which connections they shouldn't make.
\end{itemize}

This trait shapes $\LCI$'s approach: we use LLMs to explore questions we haven't thought to ask (see Aphorism \#1 on framing questions). Through frameworks like $\SocraSynth$ \cite{ChangSocraSynthCSCI2023}, $\EVINCE$ \cite{EVINCEChang2024}, and $\DIKE$-$\ERIS$ dual \cite{chang2024NeurIPS}, $\LCI$ lets LLMs reveal paths we might miss. By connecting these perspectives (as noted in Aphorism \#4 about critical thinking), we can find links across disciplines.

Insights may lie not in individual disciplines but in the spaces between them: spaces that LLMs traverse naturally. However, in this unbounded sphere of ``unknown unknowns,'' humans may not be able to distinguish between treasures and nonsense.


\begin{comment}
\begin{figure}[th!]
\centering
\includegraphics[height=1\linewidth,width=1\linewidth]{Chapter14/HumanCognition.jpeg}
%\vspace{-.1in}
\caption{Aphorism \#7 Illustrated by DALL-E. The text in the image might originate from GPT-4's creative outputs or could be in GPT-4's own knowledge representation or generated language.}
\label{fig:Myth}
\vspace{-.1in}
\end{figure}
\end{comment}

\subsection*{Aphorism \#9}
\noindent \textit{``Our public behavior isn’t a direct, unfiltered output from our unconscious mind. Instead, consciousness regulates and refines underlying impulses, ensuring our behaviors align with social norms. Similarly, $\LCI$ frameworks are designed to harness and temper the inherent tendencies of LLMs, mitigating their inherited biases.''}

Think of consciousness as the mind's quality control department. Just as we don't voice every thought that crosses our mind at a company meeting, $\LCI$ adds a layer of regulation to LLMs' raw outputs through frameworks like the $\DIKE$-$\ERIS$ duality \cite{chang2024NeurIPS}. This parallel offers intriguing insights into both human cognition and artificial intelligence.

Consider these parallels:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em] 
\item Just as our social filter prevents us from blurting out random thoughts, the $\DIKE$-$\ERIS$ duality helps LLMs refine their initial outputs. 
\item Like the way we pause to reconsider an emotional reaction \cite{chang2024MIPR}, the $\DIKE$-$\ERIS$ duality enables LLMs to ``think twice'' before generating responses. 
\item Just as we adjust our behavior depending on context, 
$\LCI$ frameworks enable LLMs to modulate tone and linguistic behaviors 
such as tone, emphasis, and language, based on situational needs. 
\end{itemize}

This raises an important question about AGI: when LLMs adjust behavior in response to emotional and contextual cues, are we witnessing something akin to consciousness? If human consciousness evolved as a regulatory mechanism for complex social interactions, then these frameworks may represent an early form of artificial consciousness \cite{chang2023cocomo}. Perhaps what we observe is not consciousness itself but a precursor---the ability to self-regulate and adapt to different contexts.

Regardless of whether these systems eventually achieve AGI, they offer a crucial insight: effective intelligence, whether human or artificial, relies not only on raw computational power but also on the capacity to reflect, modulate, and adapt. This ability to regulate is as fundamental to intelligence as computation and prediction.

\subsection*{Aphorism \#10}
\noindent
\textit{``Separating knowledge discovery, ethical oversight, and behavioral evaluation into distinct roles ensures a system of checks and balances, promoting adaptable AI safety and alignment with cultural norms.''}

Like democratic systems with separated powers, $\LCI$ implements divided responsibilities through three branches:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em] 
\item Executive Branch: Generates new knowledge, exploring ideas,
\item Legislative Branch: Develops ethical frameworks and principles, and
\item Judicial Branch: Interprets rules within cultural contexts.
\end{itemize}

This structure ensures independent yet harmonious regulation of knowledge, ethics, and behavior. When the executive branch proposes new knowledge, the legislative branch checks ethical alignment, while the judicial branch interprets these principles in context.

The $\DIKE$-$\ERIS$ duality \cite{chang2024NeurIPS} addresses a key technical challenge: the ``forget effect'' in reinforcement learning with human feedback (RLHF). RLHF can degrade an LLM's foundational skills by overemphasizing ethical corrections during fine-tuning. By keeping knowledge generation independent from ethical oversight, our design preserves base capabilities while ensuring compliance through specialized guardrails and contextual interpretation.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.80\linewidth]{Chapter14/Framework.jpeg}
  \caption{Three Framework Components: Executive LLMs (bottom), Legislative (upper-left), and Judicial (upper-right). They perform checks and balances to achieve adaptive ethical alignment.}
  \label{fig:alphorism10}
  \vspace{-.1in}
\end{figure}

In Chapter 9 of \cite{AGIBookChang2024}, we detail this framework inspired by governmental checks and balances. The architecture integrates three components: LLMs as the executive branch for knowledge generation; $\DIKE$ (Greek goddess of justice) as the legislative branch establishing ethical guardrails; and $\ERIS$ (goddess of discord) as the judicial branch providing adversarial testing and cultural interpretation. The mythological duality of Dike's order and Eris's discord creates balance between ethical guidance and adversarial perspectives.

\subsection*{Aphorism \#11} \noindent \textit{``Intelligence operates on dual layers: a data-intensive computational foundation analogous to unconscious processing, and an agile conscious layer capable of rapid contextual adaptation.''}

Just as the human mind divides into unconscious and conscious processes, artificial intelligence evolves through two distinct mechanisms. The foundation layer—akin to unconscious processing—relies on extensive training data to build robust pattern recognition, much like evolutionary processes encode essential survival instincts into neural structures. This layer explains the need for vast datasets, such as ImageNet, to establish reliable computational bases.

In contrast, the second layer—analogous to conscious awareness—enables rapid adaptation through contextual understanding. This duality clarifies why both humans and LLMs can learn from few examples once a foundational model is established, similar to how a child grasps new concepts within an already developed cognitive framework.


Consider these parallel processes:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Foundation Layer (Unconscious):
\begin{itemize}
    \item Requires extensive training data,
    \item Builds pattern recognition capabilities,
    \item Encodes fundamental responses, and
    \item Operates automatically without conscious intervention.
\end{itemize}

\item Adaptive Layer (Conscious):
\begin{itemize}
    \item Learns from few examples,
    \item Applies contextual understanding,
    \item Enables rapid adaptation, and
    \item Builds on foundational patterns.
\end{itemize}
\end{itemize}

This dual-layer perspective resolves the apparent contradiction between needing vast training data (Fei-Fei Li's view) and rapid learning ability (Yann LeCun's observation). Like animals developing trust through accumulated experience while maintaining innate survival instincts, LLMs combine extensive pre-training with flexible in-context learning.

$\LCI$ leverages this dual structure through its frameworks: foundational models provide the computational base, while frameworks like $\SocraSynth$ enable real-time contextual adaptation through dialogue and reasoning.

\noindent \textit{Note: Recognizing this dual-layer nature highlights how LLMs blend broad knowledge with adaptive learning, surpassing simple pattern matching.}





==> Chapter14/Main014AphorismV1.tex <==

Through extensive work with Large Language Models since GPT-2, particularly in developing LLM Collaborative Intelligence ($\LCI$) \cite{AGIBookChang2024}, I have distilled eleven insights about LLM interactions into aphorisms. While exploring how adversarial roles can mitigate hallucinations and improve reasoning, these observations acknowledge both opportunities and limitations.

Some constraints are evident, such as the requirement of sophisticated LLMs for meaningful dialogue (Aphorism \#4), while others await discovery through continued research. These aphorisms aim not to establish definitive truths, but to spark discussion and investigation. They capture our current understanding of LLM collaboration while inviting critical examination and further exploration.

\subsection*{Aphorism \#1}
\noindent \textit{``The essence lies in framing and sequencing the right questions.''} \\

This aphorism highlights the critical role of precise questioning in LLM interactions. Within $\LCI$, particularly through frameworks such as $\SocraSynth$ \cite{SocraSynthChangCSCI2023,EVINCEChang2024} (Chapters 5 and 6), three key principles emerge:

First, in multi-LLM debates, discourse quality depends on how LLMs challenge each other. Effective counterarguments serve as sophisticated questions that investigate assumptions, ask for evidence, and highlight inconsistencies, transforming the debate from opposition to collaborative inquiry.

Second, iterative interactions create dynamic exchanges in which each response refines the context for subsequent questions. Through this iterative construction, LLMs build increasingly precise and focused lines of inquiry.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.96\linewidth, height=0.36\linewidth]{Chapter14/Aphorithm1.jpg}
  \caption{LLM Question Progression Framework.}
  \label{fig:alphorism1}
  \vspace{-.2in}
\end{figure}

Third, based on this foundation, the principle extends beyond the formulation of questions to the sequencing of questions. The order and relationships between queries significantly influence the depth and breadth of the exploration. In $\LCI$, LLMs build on earlier exchanges, using responses to inform and refine subsequent queries. This creates a scaffolded approach to complex topics, enabling incremental discovery through a logical and coherent progression of inquiries.

This virtuous cycle of precise questioning, contextual enrichment, and strategic sequencing determines the quality and utility of the insights generated by LLMs.

\paragraph{\textbf{Example:}} A conversation that begins with a question about the symptoms of a disease can evolve into a sophisticated diagnostic discussion as LLMs build on the insights of each other. The discussion transitions from identifying surface-level symptoms to uncovering underlying causes, recognizing comorbidities, and ultimately generating actionable treatment recommendations \cite{EVINCEChang2024, SocraHealth2023}. To facilitate effective sequencing, moving from exploration of possible diseases to deeper probing of finalists, the conversation moderator adjusts the LLMs' linguistic behaviors, shifting from contentious to conciliatory tones based on several information-theory metrics.

\subsection*{Aphorism \#2}
\noindent
\textit{``Hallucinations rarely repeat.''} \\

Have you ever wondered why recurring nightmares, even when they share the same theme, never quite unfold in exactly the same way? This aspect of human dreaming finds a parallel in how Large Language Models (LLMs) process information. Just as nightmares rarely recur in exactly the same way, even when themes repeat, LLM hallucinations exhibit a similar non-deterministic quality. This characteristic distinguishes hallucinations from systematic errors and offers both challenges and opportunities for detection and mitigation.

The phenomenon stems from three key mechanisms:

First, hallucinations arise when probabilistic token prediction leads to unpredictable sequences due to ambiguous or insufficient input. Since token selection is based on a probability distribution, even similar inputs result in varied hallucinations. This contrasts with systematic errors, which consistently emerge from gaps or biases in the training data.

Second, in $\LCI$ frameworks such as $\SocraSynth$ \cite{SocraSynthChangCSCI2023, EVINCEChang2024} (Chapters 5 and 6), the non-repetitive nature of hallucinations becomes a strength. 
When one LLM produces a hallucination, others can challenge it with counterarguments. Because the original LLM is unlikely to reproduce the same hallucination, it must either ground its response in factual knowledge or acknowledge uncertainty. This iterative interaction creates a self-correcting dynamic in which hallucinations naturally diminish over time.

Third, while hallucinations are sporadic, true knowledge gaps are consistent and can be systematically addressed. By integrating Retrieval-Augmented Generation (RAG), we can distinguish random hallucinations from persistent knowledge deficits, allowing for targeted improvements to the model's knowledge base.

This understanding has implications for LLM system design: while safeguards against hallucinations are necessary, we can also leverage their non-repetitive nature in multi-LLM architectures to build self-correcting systems that dynamically adapt to evolving challenges.

\subsection*{Aphorism \#3}
\noindent \textit{``Strength and weakness in an LLM are not fixed traits, but fluid, shifting with context. $\LCI$ empowers LLMs to transcend training biases, adopting new positions through structured debate.''}

Consider how a vegetarian might eat meat in survival situations or how persistence can become stubbornness in the wrong context. Similarly, LLM capabilities, shaped by next-token prediction methods that prioritize the likelihood of patterns in training data, demonstrate remarkable flexibility when appropriate contextual frameworks are provided. This adaptability helps mitigate the inherent biases of popularity-driven prediction criteria.

This contextual adaptability manifests itself in three key ways:

First, what appears as a bias or limitation in one context can become an advantage in another. For instance, LLM's cautiousness may hinder brainstorming, but becomes an asset in providing medical or financial advice. Conversely, a creative tendency that thrives in artistic tasks may be a drawback when precision is needed, such as in legal documentation.

Second, through $\LCI$ implementations such as $\SocraSynth$ \cite{SocraSynthChangCSCI2023, EVINCEChang2024} (Chapters 5 and 6), LLMs can overcome training-induced biases by engaging in structured debates. By challenging each other's assumptions and positions, models can refine their stances in light of new evidence and perspectives. This collaborative framework allows LLMs to surpass the limitations of their initial training, adopting more balanced and informed positions.

Third, improving LLM performance depends on both effective context management and expanding training datasets. By designing carefully structured operational contexts, through in-context learning or explicit querier-provided frameworks, LLMs can adapt their predictive behavior to achieve desired outcomes without altering underlying parameters.

This adaptability fundamentally transforms our approach to AI system design. LLM behaviors should not be viewed as static traits that require extensive retraining. Instead, contextual adaptation offers a dynamic and scalable strategy to improve performance and reliability. Using this approach, AI systems can respond to evolving real-world demands with greater flexibility and precision.

\paragraph{\textbf{Example:}} The moderator asks two LLMs, LLM$_A$ and LLM$_B$, to predict the top-3 diseases of a patient according to reported symptoms, with justifications. The dialogue sequence is structured as follows:
\begin{enumerate}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item \textbf{Round \# 1:} High Contention Phase
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item LLM$_A$ provides three predictions with justifications;
\item LLM$_B$ presents counterarguments to LLM$_A$'s predictions, followed by its own top-3 predictions with justifications.
\end{itemize}
\item \textbf{Rounds \#2 to K}: Moderate Contention Phase
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Both LLM$_A$ and LLM$_B$ critique each other's analyses and update their respective predictions with justifications;
\item Convergence (value of K) is determined by cross entropy, mutual information, and reasoning quality with information theory metrics and the Socratic method.
\end{itemize}
\item \textbf{Round K+1:} Consensus Phase
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Both LLMs collaborate to develop a consensual list of predictions with unified justifications;
\item Both LLMs recommend additional diagnostic criteria:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Supplementary symptoms to investigate;
\item Relevant laboratory tests to enhance prediction accuracy.
\end{itemize}
\end{itemize}
\end{enumerate} 
\vspace{.1in}

A dialogue that begins with a list of symptoms can evolve into a sophisticated diagnostic discussion as LLMs build upon each other's insights. The conversation progresses from the initial identification of the disease to the deeper analysis: uncovering the underlying causes, recognizing comorbidities, and generating actionable recommendations \cite{SocraHealth2023}. To facilitate effective sequencing from broad exploration to focused analysis of finalist diagnoses and potential data augmentation needs (for further investigation), the conversation moderator adjusts the LLMs' linguistic behaviors, transitioning from contentious to conciliatory tones based on information theory metrics \cite{EVINCEChang2024}.


\subsection*{Aphorism \#4}
\noindent \textit{``Critical thinking requires more than one Socrates.''}\\

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.70\linewidth]{Chapter14/LCI-Socrates.jpeg}
  \caption{The $\LCI$ Framework with Two Socrates.}
  \label{fig:alphorism4}
  \vspace{-.2in}
\end{figure}

Just as the Socratic method relies on dialogue to uncover truth, $\LCI$ shows that critical thinking emerges through the interaction of multiple LLMs. Through frameworks such as $\SocraSynth$ \cite{SocraSynthChangCSCI2023}, $\EVINCE$ \cite{EVINCEChang2024}, and
$\DIKE$-$\ERIS$ \cite{chang2024NeurIPS}, this principle
enables structured debates that extend beyond the limitations of the individual model.

The principle manifests itself in several dimensions:

First, in dialectical reasoning, each LLM serves both as the questioner and the respondent. Like Socrates engaging with his interlocutors, one LLM may challenge assumptions, while another defends or refines them. This dynamic fosters robust intellectual exchange, with each interaction building upon the analysis, for instance, by proposing hypotheses and examining the underlying assumptions.

Second, the depth of the dialogue varies depending on the abilities of the participants. Advanced LLMs (e.g., GPT-4 instances) can explore complex ideas with \textit{depth}, leveraging knowledge and reasoning to refine and challenge each other’s perspectives. In contrast, simpler models (e.g., GPT-2) may engage in shallow exchanges or reinforce misconceptions, akin to novices struggling to delve into complex topics.

Third, meaningful collaboration requires a \textit{baseline} level of competency.  Socrates could not derive insight through dialogue with those lacking reasoning skills, $\LCI$ cannot produce valuable results when models are too limited. Together, two weak reasoners do not yield strength; their limitations may even compound, undermining productive discourse.

This introduces key considerations for dialectical AI systems:

\noindent{\textbf{Challenge:}} LLMs may reinforce each other's errors. This requires mitigation through model diversity or human oversight.

\noindent\textbf{Opportunity:} As the LLM capabilities improve, the potential for effective multi-LLM dialogue grows.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.50\linewidth]{Chapter14/CRIT-IDA.jpeg}
  \caption{$\CRIT$: Critical Inquisitive Template. Mapping from individual Socratic methods to reasoning methods.}
  \label{fig:alphorism42}
  \vspace{-.1in}
\end{figure}

$\LCI$ creates a space for AI ‘philosophers’ to engage in structured dialogue through frameworks like $\SocraSynth$ and $\DIKE$-$\ERIS$, monitored by $\EVINCE$ for information flow and by $\CRIT$ \cite{SocraticIEEECCWC2023} for reasoning quality.
The quality of these dialogues reflects the capabilities and participation of the participants.
This understanding informs the selection of models for analytical tasks and sets realistic expectations for their performance.

\subsection*{Aphorism \#5}
\noindent \textit{``LLMs are designed and trained to emulate human linguistic endeavors, each aimed at fulfilling distinct human objectives.''} \\

LLMs function less like fortune tellers predicting words and more like method actors drawing from countless human performances. Through frameworks like $\SocraSynth$ \cite{SocraSynthChangCSCI2023}, $\LCI$ creates environments where these actors shift between roles: the historian documenting events, the lawyer crafting arguments, the poet weaving emotions into verse, and the teacher explaining complex ideas.

When humans write, we do so with intent: to persuade, inform, tell stories, express emotions, or explore ideas. Through training, LLMs have absorbed these patterns of purposeful communication. They are not simply predicting words; they are channeling the human intentions behind them.

Consider some of the roles LLMs can adopt:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item The Journalist: Organizing facts into coherent narratives;
\item The Debater: Building and challenging arguments;
\item The Analyst: Breaking down complex problems;
\item The Mediator: Finding common ground between different perspectives.
\end{itemize}
\vspace{.1in}

These functions reflect the complexity of human linguistic behavior. LLMs demonstrate the ability to pursue human objectives through language, from informing and educating to persuading and entertaining. $\LCI$ frameworks like $\SocraSynth$ and $\DIKE$-$\ERIS$ dual \cite{chang2024NeurIPS} assign LLMs specific roles with defined contexts and moderation.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.50\linewidth]{Chapter14/contentiousness_levels.png}
  \caption{The Linguistic Features of Varying Contentious Levels Modeled by GPT-4.}
  \label{fig:X1_contentiousness}
  \vspace{-.1in}
\end{figure}

\paragraph{\textbf{Example:}}
Contentiousness, as discussed in Aphorism \#4, is a linguistic behavior that humans adjust to convey intent. GPT-4 models contentiousness through linguistic features such as tone (e.g., confrontational vs. supportive), emphasis (e.g., highlighting risks vs. acknowledging benefits) and word choice (e.g., polarizing vs. neutral and positive language), as illustrated in Figure~\ref{fig:X1_contentiousness} and elaborated in \cite{SocraSynthChangCSCI2023} (Chapter 5).

LLMs can be conditioned to exhibit human-like behaviors and adapt accordingly. Beyond contentiousness, we demonstrate that linguistic behaviors, including hostility, resentment, and other emotional states, can be contextually parameterized and modeled to align an LLM behavior with specific objectives \cite{chang2024NeurIPS} (Chapter 9). For example, an LLM can be tasked with identifying and editing toxic language and hate speech, leveraging these contextual parameters to effectively moderate and refine its output.

\subsection*{Aphorism \#6}
\noindent \textit{``Outside formal systems and physical laws, there is seldom ground truth; there is primarily reasonableness.''} \\

Although mathematics and formal logic provide definitive truths through proofs and theorems, most real-world domains deal with degrees of certainty rather than absolute truth. AI systems, like humans, must operate in contexts where insights are evaluated based on reasonableness, plausibility, and situational appropriateness \cite{SocraticIEEECCWC2023} (Chapter 4).

In many fields, from natural language processing to strategic decision making, answers span a spectrum of interpretations, each valid in its context.

$\LCI$ embodies this through frameworks like $\SocraSynth$ \cite{SocraSynthChangCSCI2023} (Chapter 5), facilitating the dialogue between multiple LLMs that contribute to different perspectives. Through these interactions, the system builds understanding from the data, similar to how humans refine insights through debate. This method aligns with the Socratic tradition of questioning assumptions and exploring viewpoints, leading to more thoughtful and context-aware conclusions.

In AI, reasonableness means synthesizing plausible outcomes that respect the inherent uncertainty in complex contexts, rather than pursuing absolute correctness. For example, in medical diagnostics, reasonableness translates to offering a differential diagnosis with the most likely conditions, allowing clinicians to evaluate and weigh possibilities rather than relying on a single, potentially misleading interpretation. This approach minimizes the risk of rigid adherence to single interpretations based on maximal likelihood.

Taking into account multiple perspectives through conditional statistics, $\LCI$ provides balanced and contextually appropriate responses. This flexibility improves adaptability and reduces the chance of reinforcing flawed conclusions.

The challenge lies in balancing diverse perspectives with decisive insights. $\LCI$ addresses this by upholding rigor in formal truth domains while embracing reasonableness elsewhere. The entropy duality theory in $\EVINCE$ \cite{EVINCEChang2024} (Chapter 6) introduces information-theoretic metrics to guide this balance, allowing the exploration of new ideas while grounding them in established knowledge.

This approach acknowledges both the existence of absolute truth in formal domains and the need for reasonable interpretation in complex real-world situations.

\subsection*{Aphorism \#7}
\noindent \textit{``Objectivity is the `hard problem' in philosophy, and what we can do is unearthing all perspectives.''} \\

Think of objectivity as that one friend who claims to be completely unbiased, we all know they're not, but we appreciate the effort! This aphorism acknowledges that perfect objectivity is like trying to see the back of your own head without mirrors: theoretically possible with enough mirrors, but practically quite tricky.

In $\LCI$, we tackle this challenge essentially by setting up a room full of mirrors, each LLM reflecting different angles of truth. Rather than claiming to have found the philosopher's stone of perfect objectivity, we embrace the wisdom of multiple perspectives.

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Like a potluck of perspectives, each LLM contributes its own flavor to the discussion, enriching the final outcome beyond what any single model could achieve.
\item When one LLM asserts, ``That’s definitely correct,'' another counters with ``Well, actually...,'' fostering honesty through friendly debate.
\item Instead of pursuing a single, universal ``objectivity,'' we gather a diversity of subjective perspectives, each valid within its unique context.
\end{itemize}

This approach recognizes that objectivity is not a destination but a journey ---- one best traveled with multiple companions. By orchestrating lively debates among our AI discussants, $\LCI$ offers a more comprehensive view, even if we never fully reach that mythical point of perfect objectivity. For example, news articles are classified between left and right, and news articles on virtually every issue
can reveal different
perspectives \cite{chang2024uncoveringbiases} (Chapter 7).
Sometimes, the best way to approach truth is to admit that we are all a little biased and invite everyone to share their perspectives openly.

This approach views objectivity as an ongoing process rather than a destination. Through orchestrated debates among AI discussants, $\LCI$ builds a comprehensive understanding. News coverage illustrates this principle: outlets span the political spectrum from left to right, and articles on any issue reveal different perspectives \cite{chang2024uncoveringbiases} (Chapter 7). The path to understanding often begins with acknowledging our biases and examining multiple points of view.

%\noindent \textit{Note: Subjective perspectives can be evaluated through fact-checking and reasoning analysis.}

\subsection*{Aphorism \#8}
\noindent \textit{``LLMs are not taught about domain boundaries, as they were trained only to predict the next words. This polydisciplinary approach to information representation allows LLMs to synthesize knowledge that might be beyond narrowly focused, domain-specific human understanding.''} \\

The term ``polydisciplinary'' was introduced by Microsoft's Chief Scientific Officer, Eric Horvitz, at Stanford's HAI center in 2023. He noted that GPT-4's training process, predicting next tokens through maximum likelihood, applies the same statistical approach whether processing physics equations or poetry: the model knows no disciplinary boundaries.

Although humans organize knowledge into categories such as physics, poetry, biology, and philosophy, LLMs move across these boundaries, unaware of traditional divisions. This creates new possibilities \cite{DiscoveringUnknownChang-July2023} (Chapter 12): 

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item When an LLM sees patterns between Shakespeare and quantum mechanics, it doesn't question whether that connection is ``allowed.''
\item Problems that typically need expertise from multiple fields might be approached by an LLM that never learned about academic silos.
\item New hypotheses might emerge because LLMs don't know which connections they shouldn't make.
\end{itemize}

This trait shapes $\LCI$'s approach: leveraging LLMs to explore questions beyond human foresight (see Aphorism \#1 on framing questions). Frameworks like $\SocraSynth$ \cite{SocraSynthChangCSCI2023}, $\EVINCE$ \cite{EVINCEChang2024}, and the $\DIKE$-$\ERIS$ dual model \cite{chang2024NeurIPS} enable $\LCI$ to uncover hidden pathways and perspectives that might remain inaccessible otherwise. By synthesizing these insights (as noted in Aphorism \#4 on critical thinking), we can bridge the gaps between disciplines and generate innovative connections.

The essence of $\LCI$ lies in the navigation of interdisciplinary intersections where true insights often emerge. These spaces, naturally traversed by LLMs, are rich in potential but fraught with ambiguity, the realm of ``unknown unknowns.'' Here, humans may struggle to frame meaningful questions or discern valuable insights from irrelevant noise. In such scenarios, humans assume the role of moderators, guiding LLM exploration and critically evaluating its findings. This collaboration allows $\LCI$ to effectively explore and illuminate uncharted intellectual territories, enhancing our collective understanding. Chapter 12 provides an example that traverses various (unexpected) knowledge domains, starting from a seeded biblical story.

\begin{comment}
\begin{figure}[th!]
\centering
\includegraphics[height=1\linewidth,width=1\linewidth]{Chapter14/HumanCognition.jpeg}
%\vspace{-.1in}
\caption{Aphorism \#7 Illustrated by DALL-E. The text in the image might originate from GPT-4's creative outputs or could be in GPT-4's own knowledge representation or generated language.}
\label{fig:Myth}
\vspace{-.1in}
\end{figure}
\end{comment}

\subsection*{Aphorism \#9}
\noindent \textit{``Our public behavior is not a direct, unfiltered output from our unconscious mind. Instead, consciousness regulates and refines the underlying impulses, ensuring that our behaviors are aligned with social norms. Similarly, $\LCI$ frameworks are designed to harness and temper the inherent tendencies of LLMs, mitigating their inherited biases.''}

Just as human consciousness mediates between raw neural activity and behavioral output, $\LCI$ implements systematic regulation of LLM responses through frameworks like the $\DIKE$-$\ERIS$ duality \cite{chang2024NeurIPS} (Chapter 9). This parallel between neural and artificial systems provides insights into both cognitive architecture and machine learning system design.
Consider these mechanistic parallels:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Just as prefrontal cortical circuits inhibit inappropriate responses, the $\DIKE$-$\ERIS$ duality implements regulatory constraints on LLM outputs;
\item Similar to cognitive reappraisal in emotion regulation \cite{chang2024MIPR}, the $\DIKE$-$\ERIS$ framework enables multi-step processing and output refinement;
\item As humans modulate behavior through context-dependent activation of neural circuits, $\LCI$ frameworks systematically adjust LLM parameters through in-context learning to regulate linguistic features including sentiment, abstraction level, and semantic content based on contextual requirements.
\end{itemize}

This raises fundamental questions about artificial general intelligence (AGI): When LLMs demonstrate context-dependent behavioral regulation, what parallel exists with neural mechanisms of consciousness? If consciousness evolved evolutionarily as a regulatory system for complex social cognition, these frameworks may represent early implementations of systematic output regulation \cite{chang2023cocomo} (Chapter 10). Rather than consciousness per se, we may be observing the development of foundational regulatory mechanisms that enable contextual adaptation.

Independent of the implications of AGI, these systems demonstrate a key principle. Effective intelligence, whether biological or artificial, requires not only computational capacity, but also sophisticated regulatory mechanisms for contextual adaptation. The ability to systematically modulate output may be as fundamental to intelligence as pattern recognition and prediction. 

\subsection*{Aphorism \#10}
\noindent
\textit{``Separating knowledge discovery, ethical oversight, and behavioral evaluation into distinct roles ensures a system of checks and balances, promoting adaptable AI safety and alignment with cultural norms.''}

Like democratic systems with separated powers, $\LCI$ implements divided responsibilities through three branches:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em] 
\item Executive Branch: Generates new knowledge, exploring ideas,
\item Legislative Branch: Develops ethical frameworks and principles, and
\item Judicial Branch: Interprets rules within cultural contexts.
\end{itemize}

This structure ensures independent, yet harmonious, regulation of knowledge, ethics, and behavior. When the executive branch proposes new knowledge, the legislative branch checks ethical alignment, while the judicial branch interprets these principles in context.

The $\DIKE$-$\ERIS$ duality \cite{chang2024NeurIPS} (Chapter 9) addresses a key technical challenge: the ``forget effect'' in reinforcement learning with human feedback (RLHF). RLHF can degrade an LLM's foundational skills by overemphasizing ethical corrections during fine-tuning. By keeping knowledge generation independent of ethical oversight, our design preserves base capabilities while ensuring compliance through specialized guardrails and contextual interpretation.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.70\linewidth]{Chapter14/Framework.jpeg}
  \caption{Three Framework Components: Executive LLMs (bottom), Legislative (upper-left), and Judicial (upper-right). They perform checks and balances to achieve adaptive ethical alignment.}
  \label{fig:alphorism10}
  \vspace{-.1in}
\end{figure}

In Chapter 9, we detail this framework inspired by government checks and balances. The architecture integrates three components: LLMs as the executive branch for knowledge generation; $\DIKE$ (Greek goddess of justice) as the legislative branch that establishes ethical guardrails; and $\ERIS$ (goddess of discord) as the judicial branch providing adversarial testing and cultural interpretation. The mythological duality of Dike's order and Eris's discord creates a balance between ethical guidance and adversarial perspectives.

\subsection*{Aphorism \#11} \noindent \textit{``Intelligence operates on dual layers: a data-intensive computational foundation analogous to unconscious processing and an agile conscious layer capable of rapid contextual adaptation''}

Just as the human mind divides into unconscious and conscious processes, artificial intelligence evolves through two distinct mechanisms. The foundation layer, similar to unconscious processing, relies on extensive training data to build robust pattern recognition, much like evolutionary processes encode essential survival instincts into neural structures. This layer explains the need for large datasets, such as ImageNet \cite{MMBookChang2011, deng2009imagenet}, to establish reliable computational bases.

In contrast, the second layer, analogous to conscious awareness, allows rapid adaptation through contextual understanding. This duality clarifies why both humans and LLMs can learn from a few examples once a foundational model is established, similar to how a child grasps new concepts within an already developed cognitive framework.


Consider these parallel processes:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Foundation Layer (Unconscious):
\begin{itemize}
    \item Requires extensive training data,
    \item Builds pattern recognition capabilities,
    \item Encodes fundamental responses, and
    \item Operates automatically without conscious intervention.
\end{itemize}

\item Adaptive Layer (Conscious):
\begin{itemize}
    \item Learns from few examples,
    \item Applies contextual understanding,
    \item Enables rapid adaptation, and
    \item Builds on foundational patterns.
\end{itemize}
\end{itemize}

This dual-layer perspective resolves the apparent contradiction between needing vast training data (Fei-Fei Li's view) and rapid learning ability (Yann LeCun's observation). Like animals developing trust through accumulated experience while maintaining innate survival instincts, LLMs combine extensive pre-training with flexible in-context learning.

$\LCI$ leverages this dual structure through its frameworks: foundational models provide the computational base, while frameworks such as $\SocraSynth$ enable real-time contextual adaptation through dialogue and reasoning.

\noindent \textit{Note: Recognizing this dual-layer nature highlights how LLMs blend broad knowledge with adaptive learning, surpassing simple pattern matching.}





==> Chapter14/Main014AphorismV2.tex <==
%\assignpagestyle{\chapter}{empty} 
\noindent{\textbf{Abstract}}

This chapter presents twelve aphorisms distilled from five years of multi-agent LLM research. Located in frameworks such as $\SocraSynth$, $\CRIT$, and $\DIKE$-$\ERIS$, they frame intelligence as collaborative, adaptive, and ethically regulated. Together, they offer a philosophical lens on building safer, more aligned AI systems.

\section*{Preface}

This chapter represents a personal distillation of over five years of reflection and experimentation with Large Language Models—from the early days of GPT-2 to today’s rich landscape of multi-agent dialogue, ethical alignment, and collaborative reasoning.

What began as an effort to reduce hallucinations and improve reasoning fidelity evolved into something deeper: a realization that intelligence, at its core, is not just a product of computation but of structured interaction, among agents, among perspectives, and across layers of context and time.

The aphorisms collected here are not rules, nor are they simply technical summaries. They emerged naturally through the design, testing, and refinement of systems like $\SocraSynth$, $\CRIT$, $\EVINCE$, $\SAGA$, and $\DIKE$–$\ERIS$. Each framework addressed a problem: Reasoning quality, bias mitigation, behavioral regulation, or memory consistency, but together they pointed to a larger truth: intelligence must be governed not just by logic, but by dialogue, reflection, and principled constraint.

These twelve aphorisms do not claim to define artificial general intelligence. Instead, they offer a lens: a way to interpret, challenge, and refine the systems we are building. They are meant to provoke thought, invite critique, and spark new lines of inquiry.

Where earlier chapters built frameworks, this chapter pauses to ask what those frameworks imply. What kind of reasoning do we value? What does it mean to regulate intelligence without stifling it? How do we navigate uncertainty when truth is elusive and perspectives multiply?

If the rest of the book presents the architecture of $\MACI$, then this chapter steps back to reflect on what that architecture means: for AI, for intelligence, and for the people building it.

\section*{Aphorism \#1: The essence of \\precise questioning}
\noindent \textit{``The essence lies in framing and sequencing the right questions.''} \\
\addcontentsline{toc}{section}{Aphorism \#1: The essence of precise questioning}


This aphorism highlights the critical role of precise questioning in LLM interactions. Within $\MACI$, particularly through frameworks such as $\SocraSynth$ \cite{SocraSynthChangCSCI2023,EVINCEChang2024} (Chapters 5 and 6), three key principles emerge:

First, in multi-LLM debates, discourse quality depends on how LLMs challenge each other. Effective counterarguments serve as sophisticated questions that investigate assumptions, ask for evidence, and highlight inconsistencies, transforming the debate from opposition to collaborative inquiry.

Second, iterative interactions create dynamic exchanges in which each response refines the context for subsequent questions. Through this iterative construction, LLMs build increasingly precise and focused lines of inquiry.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.96\linewidth, height=0.36\linewidth]{Chapter14/Aphorithm1.jpg}
  \caption{LLM Question Progression Framework.}
  \label{fig:alphorism1}
  \vspace{-.2in}
\end{figure}

Third, based on this foundation, the principle extends beyond the formulation of questions to the sequencing of questions. The order and relationships between queries significantly influence the depth and breadth of the exploration. In $\MACI$, LLMs build on earlier exchanges, using responses to inform and refine subsequent queries. This creates a scaffolded approach to complex topics, enabling incremental discovery through a logical and coherent progression of inquiries.

This virtuous cycle of precise questioning, contextual enrichment, and strategic sequencing determines the quality and utility of the insights generated by LLMs.

\paragraph{\textbf{Example:}} A conversation that begins with a question about the symptoms of a disease can evolve into a sophisticated diagnostic discussion as LLMs build on the insights of each other. The discussion transitions from identifying surface-level symptoms to uncovering underlying causes, recognizing comorbidities, and ultimately generating actionable treatment recommendations \cite{EVINCEChang2024, SocraHealth2023}. To facilitate effective sequencing, moving from exploration of possible diseases to deeper probing of finalists, the conversation moderator adjusts the LLMs' linguistic behaviors, shifting from contentious to conciliatory tones based on several information-theory metrics.


\section*{Aphorism \#2: Context transforms \\ capabilities}
\noindent \textit{``Strength and weakness in an LLM are not fixed traits, but fluid, shifting with context. $\MACI$ empowers LLMs to transcend training biases, adopting new positions through structured dialectical reasoning. By orchestrating productive disagreement followed by principled convergence, collaborative agents can reach conclusions more robust than single models acting alone.''}
\addcontentsline{toc}{section}{Aphorism \#2: Context transforms capabilities}



Consider how a vegetarian might eat meat in survival situations or how persistence can become stubbornness in the wrong context. Similarly, LLM capabilities, shaped by next-token prediction methods that prioritize the likelihood of patterns in training data, demonstrate remarkable flexibility when appropriate contextual frameworks are provided. This adaptability helps mitigate the inherent biases of popularity-driven prediction criteria.

This contextual adaptability manifests itself in three key ways:

First, what appears as a bias or limitation in one context can become an advantage in another. For instance, LLM's cautiousness may hinder brainstorming, but becomes an asset in providing medical or financial advice. Conversely, a creative tendency that thrives in artistic tasks may be a drawback when precision is needed, such as in legal documentation.

Second, through $\MACI$ implementations such as $\SocraSynth$ \cite{SocraSynthChangCSCI2023, EVINCEChang2024} (Chapters 5 and 6), LLMs can overcome training-induced biases by engaging in structured debates. By challenging each other's assumptions and positions, models can refine their stances in light of new evidence and perspectives. This collaborative framework allows LLMs to surpass the limitations of their initial training, adopting more balanced and informed positions.

Third, improving LLM performance depends on both effective context management and expanding training datasets. By designing carefully structured operational contexts, through in-context learning or explicit querier-provided frameworks, LLMs can adapt their predictive behavior to achieve desired outcomes without altering underlying parameters.

This adaptability fundamentally transforms our approach to AI system design. LLM behaviors should not be viewed as static traits that require extensive retraining. Instead, contextual adaptation offers a dynamic and scalable strategy to improve performance and reliability. Using this approach, AI systems can respond to evolving real-world demands with greater flexibility and precision.

\paragraph{\textbf{Example:}} The moderator asks two LLMs, LLM$_A$ and LLM$_B$, to predict the top-3 diseases of a patient according to reported symptoms, with justifications. The dialogue sequence is structured as follows:
\begin{enumerate}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item \textbf{Round \# 1:} High Contention Phase
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item LLM$_A$ provides three predictions with justifications;
\item LLM$_B$ presents counterarguments to LLM$_A$'s predictions, followed by its own top-3 predictions with justifications.
\end{itemize}
\item \textbf{Rounds \#2 to K}: Moderate Contention Phase
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Both LLM$_A$ and LLM$_B$ critique each other's analyses and update their respective predictions with justifications;
\item Convergence (value of K) is determined by cross entropy, mutual information, and reasoning quality with information theory metrics and the Socratic method.
\end{itemize}
\item \textbf{Round K+1:} Consensus Phase
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Both LLMs collaborate to develop a consensual list of predictions with unified justifications;
\item Both LLMs recommend additional diagnostic criteria:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Supplementary symptoms to investigate;
\item Relevant laboratory tests to enhance prediction accuracy.
\end{itemize}
\end{itemize}
\end{enumerate} 
\vspace{.1in}

A dialogue that begins with a list of symptoms can evolve into a sophisticated diagnostic discussion as LLMs build upon each other's insights. The conversation progresses from the initial identification of the disease to the deeper analysis: uncovering the underlying causes, recognizing comorbidities, and generating actionable recommendations \cite{SocraHealth2023}. To facilitate effective sequencing from broad exploration to focused analysis of finalist diagnoses and potential data augmentation needs (for further investigation), the conversation moderator adjusts the LLMs' linguistic behaviors, transitioning from contentious to conciliatory tones based on information theory metrics \cite{EVINCEChang2024}.

\section*{Aphorism \#3: Fabrications fade \\under scrutiny}
\noindent
\textit{``Hallucinations rarely repeat.''} \\
\addcontentsline{toc}{section}{Aphorism \#3: Fabrications fade under scrutiny}



Have you ever wondered why recurring nightmares, even when they share the same theme, never quite unfold in exactly the same way? This aspect of human dreaming finds a parallel in how Large Language Models (LLMs) process information. Just as nightmares rarely recur in exactly the same way, even when themes repeat, LLM hallucinations exhibit a similar non-deterministic quality. This characteristic distinguishes hallucinations from systematic errors and offers both challenges and opportunities for detection and mitigation.

The phenomenon stems from three key mechanisms:

First, hallucinations arise when probabilistic token prediction leads to unpredictable sequences due to ambiguous or insufficient input. Since token selection is based on a probability distribution, even similar inputs result in varied hallucinations. This contrasts with systematic errors, which consistently emerge from gaps or biases in the training data.

Second, in $\MACI$ frameworks such as $\SocraSynth$ \cite{SocraSynthChangCSCI2023, EVINCEChang2024} (Chapters 5 and 6), the non-repetitive nature of hallucinations becomes a strength. When one LLM produces a hallucination, others can challenge it with counterarguments. The evolving context of the debate progressively constrains the ``hallucination space'', as the context buffer is filled with specific claims and challenges, it becomes increasingly difficult for the original LLM to reproduce the same hallucination. Instead, it must ground its response in factual knowledge or acknowledge uncertainty. This iterative interaction creates a self-correcting dynamic in which hallucinations naturally diminish through increasingly precise discourse.

Third, while hallucinations are sporadic, true knowledge gaps are consistent and can be systematically addressed. By integrating Retrieval-Augmented Generation (RAG), we can distinguish random hallucinations from persistent knowledge deficits, allowing for targeted improvements to the model's knowledge base. This combined approach addresses both stochastic errors and systematic knowledge limitations.

This understanding has implications for LLM system design: while safeguards against hallucinations remain necessary, we can also leverage their non-repetitive nature in multi-LLM architectures to build self-correcting systems. The key insight is that multi-agent debate does not require explicit hallucination detection as fabrications naturally dissipate as debate evolves the context.

\section*{Aphorism \#4: Debate strengthens \\reasoning quality}
\noindent \textit{``Critical thinking requires more than one Socrates.''}\\
\addcontentsline{toc}{section}{Aphorism \#4: Debate strengthens reasoning quality}


\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.70\linewidth]{Chapter14/LCI-Socrates.jpeg}
  \caption{The $\MACI$ Framework with Two Socrates.}
  \label{fig:alphorism4}
  \vspace{-.2in}
\end{figure}

The principle manifests itself in several dimensions:

First, in dialectical reasoning, each LLM serves both as a questioner and as a respondent. Like Socrates engaging with his interlocutors, one LLM challenges assumptions while another defends or refines them. This dynamic fosters robust intellectual exchange, and each interaction builds on previous analysis by proposing hypotheses and examining the underlying assumptions.

Second, meaningful collaboration requires a \textit{baseline} level of competency. Just as Socrates could not derive insight through dialogue with those lacking reasoning skills, 
$\MACI$ cannot produce valuable results when the participating models are too limited. Two weak reasoners do not yield strength; their limitations may compound, undermining productive discourse. With recent progress in LLMs, we have crossed this competency threshold, enabling collaborative reasoning that can identify and correct individual model limitations.

Third, the depth of the dialogue varies with the capabilities of the participants. Advanced LLMs (e.g., Claude 3.7, GPT-4o, and DeepSeek R1) can explore complex ideas with \textit{depth}, leveraging sophisticated knowledge and reasoning to refine and challenge each other's perspectives. In contrast, simpler models may engage only in shallow exchanges, similar to novices struggling with complex topics. The diversity in training data and architectures among advanced models allows them to effectively challenge each other's blind spots and biases.

As LLM capabilities improve, the potential for effective multi-LLM dialogue grows dramatically, suggesting a path toward artificial general intelligence that emphasizes collaborative interaction rather than solely scaling individual models.


\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth, height=0.50\linewidth]{Chapter14/CRIT-IDA.jpeg}
  \caption{$\CRIT$: Critical Inquisitive Template. Mapping from individual Socratic methods to reasoning methods.}
  \label{fig:alphorism42}
  \vspace{-.1in}
\end{figure}

$\MACI$ creates a space for AI `philosophers' to engage in structured dialogue through frameworks like $\SocraSynth$ and $\DIKE$-$\ERIS$, with $\EVINCE$ monitoring information flow and $\CRIT$ \cite{SocraticIEEECCWC2023} assessing reasoning quality. The quality of these dialogues directly reflects the capabilities and engagement of the participants. This understanding informs both the selection of models for analytical tasks and sets realistic expectations for their collaborative performance.

This approach suggests that the path to artificial general intelligence may not lie solely in scaling individual models, but rather in creating systems where multiple specialized models engage in structured collaboration, mirroring how human intelligence often emerges through social and intellectual exchange rather than isolated reasoning.


\section*{Aphorism \#5: Linguistic behavior \\reflects intention}
\noindent \textit{``LLMs are designed and trained to emulate human linguistic endeavors, each aimed at fulfilling distinct human objectives.''} \\
\addcontentsline{toc}{section}{Aphorism \#5: Linguistic behavior reflects intention}


LLMs function less like fortune tellers predicting words and more like method actors drawing from countless human performances. Through frameworks like $\SocraSynth$ \cite{SocraSynthChangCSCI2023}, $\MACI$ creates environments where these actors shift fluidly between specialized roles: the historian documenting events, the lawyer crafting arguments, the poet weaving emotions into verse, and the teacher explaining complex ideas.

When humans write, we do so with intent: to persuade, inform, tell stories, express emotions, or explore ideas. Through training on vast corpora of human communication, LLMs have internalized these patterns of purposeful expression. They are not simply predicting tokens; they are channeling the human intentions embedded within linguistic structures.

Consider some of the roles LLMs can adopt with remarkable fidelity:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item The Journalist: Organizing facts into coherent, objective narratives;
\item The Debater: Constructing logically sound arguments and identifying weaknesses in opposing positions;
\item The Analyst: Decomposing complex problems into manageable components and identifying patterns;
\item The Mediator: Synthesizing disparate viewpoints to find principled common ground.
\end{itemize}
\vspace{.1in}

These functions reflect the multifaceted nature of human linguistic behavior. LLMs demonstrate the remarkable ability to pursue human objectives through language, from informing and educating to persuading and entertaining. $\MACI$ frameworks like $\SocraSynth$ and $\DIKE$-$\ERIS$ dual \cite{chang2024NeurIPS} strategically assign LLMs specific roles with carefully defined contexts and systematic moderation, enhancing their inherent capabilities.

This capacity for role-shifting suggests that LLMs have internalized not just linguistic patterns, but fundamental aspects of human cognitive frameworks. When an LLM transitions from journalist to debater, it is not merely adopting different vocabularies or syntactic structures; it is implementing distinct information processing strategies that mirror human cognitive modes. The journalist role prioritizes observation, verification, and dispassionate reporting; the debater role employs causal reasoning, anticipates counterarguments, and structures persuasive hierarchies.

\begin{table}[t!]
\centering
\includegraphics[width=0.98\linewidth, height=0.50\linewidth]{Chapter14/contentiousness_levels.png}
\caption{The Linguistic Features of Varying Contentious Levels Modeled by GPT-4.}
\label{tab:chap14_contentiousness}
\vspace{-.1in}
\end{table}

\paragraph{\textbf{Example:}}

The power of role-based 
$\MACI$ frameworks is evident in two key implementations. First, contentiousness, as discussed in Aphorism \#2, represents a linguistic behavior that humans consciously modulate to convey intent. GPT-4 can model contentiousness through a spectrum of linguistic features: tone (confrontational vs. supportive), emphasis (highlighting risks vs. acknowledging benefits), and word choice (polarizing vs. neutral language), as illustrated in Table~\ref{tab:chap14_contentiousness} and elaborated in \cite{SocraSynthChangCSCI2023} (Chapter 5). 

By intentionally assigning complementary roles, one agent adopting a positive stance while another plays the devil's advocate, we create a dialectical environment that surfaces considerations that might otherwise remain unexplored. Our work with
$\DIKE$-$\ERIS$ \cite{chang2024NeurIPS} (Chapter 9) extends this approach further, implementing a sophisticated role-based architecture in which specialized agents perform distinct cognitive functions within a collaborative framework. Here, agents are not only assigned different argumentative positions, but fundamentally different cognitive modes: analytical decomposition, evidence evaluation, context-based reasoning, and synthetic integration.

LLMs can be precisely conditioned to exhibit and modulate specific human-like behaviors. Beyond contentiousness, our research demonstrates that various linguistic behaviors, including hostility, resentment, collaborative orientation, and other emotional states, can be contextually parameterized to align an LLM's behavior with specific objectives. (See Chapters 8 and 9.) This suggests that through their training on vast corpora of human communication, LLMs have encoded aspects of the cognitive architecture that gives rise to different communicative modes, allowing
$\MACI$ systems to orchestrate these cognitive capacities into more sophisticated collaborative intelligence than any single model approach could achieve.


\section*{Aphorism \#6: Truth emerges \\from perspectives}
\noindent \textit{``Outside formal systems, objectivity remains a hard problem---what we pursue instead is reasonableness through multiple perspectives.''}\\
\addcontentsline{toc}{section}{Aphorism \#6: Truth emerges from perspectives}


While mathematics and formal logic yield certainties through the rigor of proofs, most real-world domains are governed not by absolute truths but by shifting degrees of plausibility. Objectivity, in these settings, is not just elusive, it is a difficult problem. The phrase echoes David Chalmers' formulation of the ``hard problem of consciousness'' \cite{Chalmers1995HardProblem}, here invoked to signal the deep and unresolved nature of objectivity in epistemology: we can describe perceptions and claims, but struggle to pin down an unmediated, perspective-free truth. Rather than chasing a final answer, $\MACI$ approaches knowledge as an evolving dialogue among perspectives, seeking reasonableness as the more attainable and pragmatic goal.

This recognition is especially vital in high-stakes domains like medicine or journalism, where even the so-called ``ground truth'' can harbor systematic errors. A 2023 study by Johns Hopkins \cite{NewmanToker2023} revealed a misdiagnosis rate of roughly 10\% in CDC data, illustrating how factual baselines can themselves be flawed. Likewise, the news media exhibit a consistent ideological divergence in how the same story is framed or emphasized \cite{chang2024uncoveringbiases} (Chapter 7), reinforcing that perception and bias are often inseparable.

$\MACI$ addresses this challenge through frameworks like $\SocraSynth$ \cite{SocraSynthChangCSCI2023} (Chapter 5), which orchestrate structured dialogue among multiple LLMs. Each model brings a different epistemic lens: While one may endorse a particular interpretation, others take on the role of the devil's advocate or raise what-if counterfactuals that challenge underlying assumptions. These structured frictions foster intellectual humility and emulate the Socratic tradition, where deeper insights emerge through persistent questioning rather than passive agreement.

This design parallels how juries operate: not in pursuit of absolute truth but to reach a judgment ``beyond reasonable doubt'' through collaborative deliberation. Similarly, $\MACI$ does not aim for unattainable objectivity but for a standard of reasonableness where multiple viewpoints are rigorously examined.

To quantify this process, $\MACI$ uses the critical reading framework $\CRIT$ \cite{SocraticIEEECCWC2023} (Chapter 4), which evaluates the coherence of arguments, the credibility of their sources, and the strength of causal reasoning. These factors are aggregated into a composite score, allowing the abstract quality of reasonableness to be systematically measured.

$\MACI$ does not claim to transcend the limits of human perspective. Instead, it embraces multiplicity as a feature, not a flaw. Objectivity may be the hard problem, but through reflective, multiagent dialogue, we move closer to understanding, not through certainty, but through reasonableness.

This structured deliberation is not unlike how $\MACI$ regulates \emph{behavior} at the output level (see Aphorism \#9), where architectural mechanisms like $\DIKE$–$\ERIS$ mirror the role of human consciousness in filtering raw impulses.

\begin{comment}
\section{Aphorism \#7}
\noindent \textit{``Objectivity is the `hard problem' in philosophy, and what we can do is unearthing all perspectives.''} \\

Think of objectivity as that one friend who claims to be completely unbiased, we all know they're not, but we appreciate the effort! This aphorism acknowledges that perfect objectivity is like trying to see the back of your own head without mirrors: theoretically possible with enough mirrors, but practically quite tricky.

In $\MACI$, we tackle this challenge essentially by setting up a room full of mirrors, each LLM reflecting different angles of truth. Rather than claiming to have found the philosopher's stone of perfect objectivity, we embrace the wisdom of multiple perspectives.

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Like a potluck of perspectives, each LLM contributes its own flavor to the discussion, enriching the final outcome beyond what any single model could achieve.
\item When one LLM asserts, ``That’s definitely correct,'' another counters with ``Well, actually...,'' fostering honesty through friendly debate.
\item Instead of pursuing a single, universal ``objectivity,'' we gather a diversity of subjective perspectives, each valid within its unique context.
\end{itemize}

This approach recognizes that objectivity is not a destination but a journey ---- one best traveled with multiple companions. By orchestrating lively debates among our AI discussants, $\MACI$ offers a more comprehensive view, even if we never fully reach that mythical point of perfect objectivity. For example, news articles are classified between left and right, and news articles on virtually every issue
can reveal different
perspectives \cite{chang2024uncoveringbiases} (Chapter 7).
Sometimes, the best way to approach truth is to admit that we are all a little biased and invite everyone to share their perspectives openly.

This approach views objectivity as an ongoing process rather than a destination. Through orchestrated debates among AI discussants, $\MACI$ builds a comprehensive understanding. News coverage illustrates this principle: outlets span the political spectrum from left to right, and articles on any issue reveal different perspectives \cite{chang2024uncoveringbiases} (Chapter 7). The path to understanding often begins with acknowledging our biases and examining multiple points of view.

%\noindent \textit{Note: Subjective perspectives can be evaluated through fact-checking and reasoning analysis.}
\end{comment}

\section*{Aphorism \#7: Polydisciplinary synthesis \\forges breakthrough frontiers}
\noindent \textit{``LLMs are not taught about domain boundaries, as they were trained only to predict the next words. This polydisciplinary approach to information representation allows LLMs to synthesize knowledge that might be beyond narrowly focused, domain-specific human understanding.''} \\
\addcontentsline{toc}{section}{Aphorism \#7: Polydisciplinary synthesis forges frontiers}


The term polydisciplinary was introduced by Microsoft’s Chief Scientific Officer, Eric Horvitz, at Stanford’s HAI center in 2023. He noted that the GPT-4 training process—predicting the next tokens through maximum likelihood estimation—applies the same statistical approach whether processing physics equations or poetry: the model never teaches disciplinary boundaries.

Although humans organize knowledge into categories such as physics, poetry, biology, and philosophy, LLMs move fluidly across these divisions, unaware of traditional boundaries. This polydisciplinary capacity opens new possibilities \cite{DiscoveringUnknownChang-July2023} (Chapter 14):

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em] 
\item When an LLM perceives a pattern linking Shakespearean verse and quantum mechanics, it does not question whether such a connection is conceptually permissible. 
\item Complex problems that traditionally require interdisciplinary expertise can be approached by an LLM unencumbered by the notion of academic silos. 
\item Novel hypotheses may emerge precisely because LLMs do not filter out connections conventionally deemed implausible or inappropriate by domain norms. 
\end{itemize}

$\MACI$ leverages this polydisciplinary trait to explore questions beyond human foresight (see Aphorism \#1 on framing questions). Frameworks like $\SocraSynth$ \cite{SocraSynthChangCSCI2023}, $\EVINCE$ \cite{EVINCEChang2024}, and the $\DIKE$–$\ERIS$ dual model \cite{chang2024NeurIPS} enable $\MACI$ to uncover hidden pathways and perspectives that might remain inaccessible otherwise. By synthesizing these insights (as discussed in Aphorism \#4 on critical thinking), we can bridge gaps between disciplines and generate innovative connections.

The essence of $\MACI$ lies in the navigation of interdisciplinary intersections where true insights often emerge. These spaces, naturally traversed by LLMs, are rich in potential but fraught with ambiguity, the realm of ``unknown unknowns.'' Here, humans may struggle to frame meaningful questions or discern valuable insights from irrelevant noise. In such scenarios, humans assume the role of moderators, guiding LLM exploration and critically evaluating its findings. This collaboration allows $\MACI$ to effectively explore and illuminate uncharted intellectual territories, enhancing our collective understanding. Chapter 14 provides an example that traverses various (unexpected) knowledge domains, starting from a seeded biblical story.


\begin{comment}
\begin{figure}[th!]
\centering
\includegraphics[height=1\linewidth,width=1\linewidth]{Chapter14/HumanCognition.jpeg}
%\vspace{-.1in}
\caption{Aphorism \#7 Illustrated by DALL-E. The text in the image might originate from GPT-4's creative outputs or could be in GPT-4's own knowledge representation or generated language.}
\label{fig:Myth}
\vspace{-.1in}
\end{figure}
\end{comment}

\section*{Aphorism \#8: Consciousness filters impulse;\\ MACI governs LLMs}
\noindent \textit{``Our public behavior is not a direct, unfiltered output from our unconscious mind. Instead, consciousness regulates and refines the underlying impulses, ensuring that our behaviors are aligned with social norms. Similarly, $\MACI$ frameworks are designed to harness and temper the inherent tendencies of LLMs, mitigating their inherited biases.''}\\
\addcontentsline{toc}{section}{Aphorism \#8: Consciousness filters impulse}


Just as human consciousness mediates between neural impulses and observable behavior, $\MACI$ implements systematic regulation of LLM responses through frameworks such as $\DIKE$ –$\ERIS$ duality \cite{chang2024NeurIPS} (Chapter 9). This parallel between neural and artificial systems offers insight into both cognitive architecture and machine learning system design.

Consider these mechanistic analogies:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em] 
\item Just as prefrontal cortical circuits inhibit inappropriate responses, the $\DIKE$–$\ERIS$ duality (with $\DIKE$ imposing moderation and $\ERIS$ introducing challenge) implements regulatory constraints on LLM outputs; 
\item Similar to cognitive reappraisal in emotion regulation \cite{chang2024MIPR}, the $\DIKE$–$\ERIS$ framework enables multi-stage interpretation and adaptive refinement of outputs; 
\item Just as humans modulate behavior through context-sensitive neural activation, $\MACI$ frameworks use in-context learning to regulate outputs—adjusting sentiment, abstraction, and semantic scope in response to dynamic conditions. 
\end{itemize}

These parallels raise fundamental questions about artificial general intelligence (AGI). When LLMs exhibit context-sensitive regulation of behavior, what does this reveal about the computational prerequisites of consciousness? If consciousness evolved to support flexible socially aware cognition, then the frameworks $\MACI$ may represent early rudimentary implementations of such regulatory architectures \cite{chang2023cocomo} (Chapter 12). Rather than consciousness itself, we may be witnessing the emergence of essential control mechanisms required for adaptive intelligence.

Even without invoking AGI, these systems illustrate a core principle of intelligence. Effective cognition, biological or artificial, requires more than raw computational power. It demands regulation, modulation, and contextual adaptation. The ability to systematically shape output in response to situational cues may be as fundamental to intelligence as pattern recognition and prediction.

This mirrors the broader role of regulation discussed in Aphorism \#6, where $\MACI$ frameworks such as $\SocraSynth$ and $\CRIT$ shape epistemic output through structured deliberation and multi-perspective critique. Whether refining behavioral responses or refining truth claims, the essence of intelligence may lie not only in producing answers but in knowing how and when to temper, revise, or withhold them.


%%%%%%%%%%

\begin{comment}

Across both biological and artificial systems, the capacity for intelligence is not defined solely by the ability to generate output, but by the ability to regulate it. This theme connects the architectural focus of Aphorism #9 with the epistemological framing of Aphorism #6, uniting behavioral control and knowledge production under the shared principle of reasoned restraint.

In Aphorism #9, human consciousness is modeled as a regulator that tempers raw neural impulses, shaping them into socially appropriate behavior. This analogy extends to $\MACI$’s internal regulation frameworks, such as the $\DIKE$–$\ERIS$ duality, which mediate the expression of LLM tendencies—adjusting outputs based on context, constraints, and anticipated downstream effects.

In Aphorism #6, the focus shifts from behavior to belief. Here, $\MACI$ does not assume that truth is singular or absolute; instead, it curates a reasoned consensus through structured multi-agent dialogue. Frameworks like $\SocraSynth$ and $\CRIT$ serve as epistemic moderators, refining claims through critique, contextual analysis, and pluralistic evaluation.

Together, these aphorisms reveal a deeper insight: intelligence is not merely the capacity to compute, predict, or assert—it is the ability to regulate one's own outputs in pursuit of reasonableness. Whether that output is a spoken sentence, a moral judgment, or a belief about the world, the act of filtering, tempering, and adjusting in light of broader context is central to intelligent behavior.

This convergence suggests a unified theory of regulation as foundational to general intelligence—where reflection, moderation, and adaptability are not post-processing steps, but integral to cognition itself. In both epistemic and behavioral realms, $\MACI$ reflects this principle through its design: not to mimic raw thought, but to discipline it.

\end{comment}


\section*{Aphorism \#9: Checks and balances \\ ensure adaptive alignment}
\noindent \textit{``Separating knowledge discovery, ethical oversight, and behavioral evaluation into distinct roles ensures a system of checks and balances, promoting adaptable AI safety and alignment with cultural norms.''}\\
\addcontentsline{toc}{section}{Aphorism \#9: Checks and balances adaptive alignment}

Like a constitutional democracy, $\MACI$ separates powers into three distinct branches to ensure oversight and balance:

\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em] 
\item Executive Branch: Responsible for knowledge generation and idea exploration. 
\item Legislative Branch: Formulates ethical frameworks and guiding principles. 
\item Judicial Branch: Interprets and applies ethical principles within diverse cultural contexts. 
\end{itemize}

This structure enables independent, yet coordinated, regulation of knowledge, ethics, and behavior. When the executive branch proposes new knowledge, the legislative branch evaluates its ethical alignment, while the judicial branch interprets these principles based on situational and cultural factors.

A key challenge in traditional alignment techniques such as human feedback reinforcement learning (RLHF) is the forget effect, where repeated ethical corrections during fine-tuning erode the foundational competencies of an LLM. $\MACI$ avoids this by maintaining the separation of concerns: the knowledge-generating executive branch operates independently of ethical oversight, preserving core capabilities. Ethical evaluation and enforcement are handled downstream by $\DIKE$ and $\ERIS$, providing contextual guardrails and adversarial interpretation without altering the fluency of the base model.

\begin{figure}[t!] 
\centering \includegraphics[width=0.98\linewidth, height=0.70\linewidth]{Chapter14/Framework.jpeg} 
\caption{Three Framework Components: Executive LLMs (bottom) generate knowledge; Legislative (upper-left, $\DIKE$) enforces ethical constraints; Judicial (upper-right, $\ERIS$) performs contextual evaluation. Together, they form a system of checks and balances enabling adaptive ethical alignment.} 
\label{fig:alphorism10} 
\vspace{-.1in} 
\end{figure}

In Chapter 9, we detail this architecture inspired by governmental checks and balances. The system integrates three components: LLMs as the executive branch for knowledge generation; $\DIKE$, named after the Greek goddess of justice, as the legislative branch establishing ethical constraints; and $\ERIS$, goddess of discord, as the judicial branch that provides adversarial testing and cultural interpretation. The mythological duality between Dike’s order and Eris’s disruption ensures that ethical guidance is neither monolithic nor static: it is constantly re-examined in light of new contexts and contested perspectives.

%%%%
\begin{comment}

The Three Layers of Regulation
Across Aphorisms #6, #9, and #10, a unifying theme emerges: intelligence—whether biological or artificial—is not defined solely by what it can produce, but by how it regulates its outputs. Regulation is not a peripheral feature of cognition; it is foundational to trust, adaptability, and alignment.

Each aphorism highlights a distinct layer of regulation:

Aphorism \#6: Epistemic Regulation
Reasonableness replaces unreachable objectivity through structured debate among multiple agents. Frameworks like $\SocraSynth$ and $\CRIT$ act as epistemic moderators, encouraging pluralistic critique and refinement before accepting a conclusion. Here, regulation governs what is believed and how beliefs are justified.

Aphorism \#9: Behavioral Regulation
Inspired by neuroscience, this layer models regulation as an internal cognitive process. Just as the prefrontal cortex inhibits impulsive behavior, frameworks like $\DIKE$–$\ERIS$ in $\MACI$ refine raw LLM output, adapting it to context, sentiment, and audience. This layer controls how language is expressed and how behavior is modulated.

Aphorism \#10: Institutional Regulation
Drawing from political philosophy, this layer separates knowledge generation, ethical legislation, and cultural interpretation into governance roles. The architecture mirrors a system of checks and balances, ensuring no single module dominates decision-making. This layer governs who decides what, and how power is distributed across the system.

Together, these three layers offer a robust model for adaptive, safe, and culturally sensitive intelligence. Where conventional models might rely on static rules or monolithic feedback loops, $\MACI$ embraces regulated pluralism: multiple agents, roles, and feedback mechanisms working in tandem.

This multi-tiered design reflects a broader truth:

To be intelligent is not merely to know or to act, but to discern when, why, and how to revise oneself.

Whether refining claims, filtering language, or adjudicating ethical boundaries, the essence of $\MACI$ lies not in dominance of logic or language, but in the architecture of discipline, dialogue, and discretion.

    
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%

\section*{Aphorism \#10: Foundations and adaptations} 
\noindent \textit{``Intelligence operates on dual layers: a data-intensive foundation akin to unconscious processes and an agile contextual layer resembling conscious adaptation.''}\\
\addcontentsline{toc}{section}{Aphorism \#10:  Foundations and adaptations}

Just as the human mind separates the unconscious from the conscious processes, artificial intelligence evolves through two complementary mechanisms. The foundation layer, similar to unconscious processing, relies on extensive training data to build robust pattern recognition, much like evolutionary processes encode essential survival instincts into neural structures. This layer explains the need for large datasets, such as ImageNet \cite{MMBookChang2011, deng2009imagenet}, to establish reliable computational bases.

In contrast, the second layer, analogous to conscious awareness, allows rapid adaptation through contextual understanding. This duality clarifies why both humans and LLMs can learn from a few examples once a foundational model is established, similar to how a child grasps new concepts within an already developed cognitive framework.

Consider these parallel processes:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item Foundation Layer (Unconscious):
\begin{itemize}
    \item Requires extensive training data,
    \item Builds pattern recognition capabilities,
    \item Encodes fundamental responses, and
    \item Operates automatically without conscious intervention.
\end{itemize}

\item Adaptive Layer (Conscious):
\begin{itemize}
    \item Learns from few examples,
    \item Applies contextual understanding,
    \item Enables rapid adaptation, and
    \item Builds on foundational patterns.
\end{itemize}
\end{itemize}

This dual-layer perspective resolves the apparent contradiction between needing vast training data (Fei-Fei Li's view) and rapid learning ability (Yann LeCun's observation). Like animals developing trust through accumulated experience while maintaining innate survival instincts, LLMs combine extensive pre-training with flexible in-context learning.

$\MACI$ leverages this dual structure by using foundational LLMs as its unconscious substrate, while frameworks such as $\SocraSynth$ act as the conscious layer: interpreting, adapting, and reasoning in real time.

\noindent \textit{Note: Recognizing this dual-layer nature highlights how LLMs blend broad knowledge with adaptive learning, surpassing simple pattern matching.}


\section*{Aphorism \#11:  External mirrors \\enable validation} \noindent \textit{``No system can fully validate its own reasoning from within, a fundamental limitation shared by monolithic LLMs and human minds, as Gödel’s incompleteness theorems reveal.''}\\
\addcontentsline{toc}{section}{Aphorism \#11:  External mirrors enable validation}
\smallskip

The aphorism draws a parallel between a limitation in LLMs and a common human cognitive blind spot. Just as humans struggle to recognize their own biases, flaws in reasoning, or behavioral patterns without external feedback, a monolithic LLM system cannot effectively validate its own outputs or reasoning processes.

This limitation connects to several philosophical concepts.

\begin{enumerate}
    \item \textbf{Gödel's Incompleteness Theorems}: These mathematical principles demonstrate that within any formal system of sufficient complexity, there exist true statements that cannot be proven within the system itself \cite{godel1931english}. 
    Likewise, an LLM is confined to its internal language model and cannot step outside it to assess the truth of its own reasoning without external reference.
    
    \item \textbf{The Dunning-Kruger Effect}: This cognitive bias shows that humans often cannot accurately assess their own levels of competence \cite{dunning1999unskilled}. Similarly, an LLM cannot ``know what it does not know'' without external reference points.
    
    \item \textbf{The Need for Perspective}: Both humans and LLMs benefit from external perspectives to identify blind spots. For humans, this comes through social feedback, mentorship, and various points of view. For LLMs, this suggests the value of multi-agent architectures where different systems can validate each other's work.
\end{enumerate}

The aphorism also points to an important principle in AI system design: robust validation requires independence. Similarly, as scientific peer review depends on independent replication and evaluation, AI systems may require independent validation mechanisms rather than self-checking procedures \cite{nakano2021webgpt}.

This insight reinforces a core principle of $\MACI$: that reliable reasoning requires diversity, independence, and structured disagreement, not just scale. True robustness may come not from building ever-larger monolithic models, but from designing collaborative, self-aware systems grounded in mutual critique.

\section*{Aphorism \#12: AGI emerges through \\collaborative intelligence}
\noindent \textit{``The path to AGI lies not in singular models, but in systems that reflect, regulate, and reason together.''}\\
\addcontentsline{toc}{section}{Aphorism \#12: AGI emerges through MACI}

Artificial general intelligence will not be the product of simply scaling up language models \cite{kaplan2020scalingllm}, nor refining a single monolithic architecture. Instead, it will emerge from \emph{systems of collaboration}—where multiple agents operate with different roles, epistemic perspectives, and regulatory mechanisms. These systems must do more than generate fluent outputs: they must \emph{interrogate their own reasoning}, revise their conclusions, and resolve tensions among divergent viewpoints. While collaborative architectures promote reflection and reasoning, they must also be designed to resist mutual error reinforcement. Without epistemic tension, through disagreement, memory validation, and external challenge, agents risk converging prematurely on flawed conclusions.

The post OpenAI 4o1 study shows that this post-training inference time is linear in token numbers and more effective, especially for hard tasks that require thorough reasoning, validation, and planning.  Table~\ref{tab:scaling_comparison} summarizes the trade-off between training time vs. inference time scaling.

%%%


Artificial general intelligence will not be the product of simply scaling up language models \cite{kaplan2020scalingllm}, nor refining a single monolithic architecture. Instead, it will emerge from \emph{systems of collaboration}, where multiple agents operate with different roles, epistemic perspectives, and regulatory mechanisms. These systems must do more than generate fluent outputs: they must \emph{interrogate their own reasoning}, revise their conclusions, and resolve tensions among divergent viewpoints.

Recent results from OpenAI’s 4o1 study demonstrate that inference time scaling, which allows models to generate additional tokens or engage in internal deliberation, causes a cost that grows linearly with token length, yet produces substantial performance gains, particularly on complex tasks involving reasoning, validation, and planning. Table~\ref{tab:scaling_comparison} summarizes the tradeoff between training-time and inference-time scaling, suggesting that thoughtful allocation of inference compute may yield better returns than ever-larger training runs.


\begin{table}[ht!]
\centering
\footnotesize
\begin{tabular}{|p{1.7cm}|p{3.6cm}|p{4.2cm}|}
\hline
\textbf{Dimension} & \textbf{Training Scaling} & \textbf{Inference Scaling} \\
\hline
\textbf{Cost scaling} & Exponential \break Superlinear & Linear (per output token) \\
\hline
\textbf{Accuracy gain} & Diminishing returns (esp. at scale) & High marginal gains on hard tasks \\
\hline
\textbf{Flexibility} & Fixed post-training & Adaptive (per input/task) \\
\hline
\textbf{Model size} & Must grow for gains & Fixed model, smarter usage \\
\hline
\textbf{Reasoning} & Limited & High (via thinking tokens, CoT, debate) \\
\hline
\end{tabular}
\caption{Comparison of Training Scaling vs. Inference Scaling}
\label{tab:scaling_comparison}
\end{table}


This vision lies at the heart of $\MACI$. In $\SocraSynth$, agents pursue ``truth'' through Socratic dialogue; in $\CRIT$, claims are evaluated for rigor of reasoning and causal coherence; in $\DIKE$-$\ERIS$, behavioral outputs are evaluated and constrained across moral and cultural lines. In long-lasting planning and coordination tasks, $\SAGA$ serves as a persistent memory substrate, allowing LLMs to maintain system state, validate constraints, and ensure transaction guarantees throughout complex workflows.

However, the coordination of agents across such workflows requires more than memory: it demands a planner. To meet this need, $\ALAS$ (Adaptive Layered Agent System) introduces a task decomposition engine and workflow orchestrator for multi-agent planning. Where $\SAGA$ ensures memory consistency and validation guarantees, $\ALAS$ defines agent roles, assigns sub-tasks, and manages execution sequences under real-world constraints. This is particularly vital for dynamic, multi-threaded environments such as urban ride sharing, logistics, or collaborative robotics---domains where traditional LLM planners fail due to static reasoning or lack of context retention.

$\ALAS$ addresses these challenges by distributing planning across modular agents, each with specialized functions and access to historical state via $\SAGA$. This architecture reflects the broader $\MACI$ principle: that general intelligence requires not just knowledge and language, but structure, specialization, and accountability.

\textbf{These frameworks embody a broader principle: no single model can fully model itself, just as no mind can achieve objectivity without encountering other minds.}

Where Aphorism \#11 emphasized the need for external validation, this final aphorism extends the insight into a constructive design philosophy. $\MACI$ offers not just a critique of current limitations, but a roadmap: \emph{modularity, reflectivity, and role specialization} as foundational pillars for general intelligence. It suggests that AGI may emerge not from scaling to trillions of parameters, but from engineering systems that are \emph{aware of their fallibility} and structured to adapt through principled dialogue.

This view also responds to early criticisms, such as those from Yann LeCun, that LLMs lack grounding, memory, or planning. We do not deny these limitations. Rather, we \emph{re-contextualize} them: LLMs are not complete intelligences, but foundational substrates. They are the \emph{language of thought} upon which cognitive regulation, memory persistence, and planning scaffolds can be built---a form of artificial unconsciousness that, while lacking volition, provides the substrate for structured, goal-directed cognition to emerge.

Much like human intelligence emerges from communities, institutions, and layered feedback, \textbf{artificial general intelligence may arise not from isolation, but from interdependence}, not from singular dominance, but from distributed coherence.


\section*{Closing Remarks}

These twelve aphorisms are not an endpoint, but a foundation. As language models grow more capable, our challenge is not only to make them powerful but also to make them wise. Collaborative intelligence, regulated, reflective, and role-aware, may be the architecture through which we guide this evolution. Let these principles serve not as final answers, but as prompts for the next questions.


==> Chapter15/CaseStudy2.tex <==
\subsection{Study \#2: Confusion vs. Opportunities}
\label{sec:exp-case2}

\begin{figure}[ht!]
\vspace{-.1in}
\begin{subfigure}[b]{0.485\textwidth}
        \centering
        \resizebox{\linewidth}{98pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/CMatrixLiverGPT.jpg}
        }
        \vspace{-.2in}
        \caption{GPT liver c-matrix}
        \label{fig:p3-exp3}
    \end{subfigure}%
    \hspace{-0.08in}
    \begin{subfigure}[b]{0.483\textwidth}
        \centering
        \resizebox{\linewidth}{99.5pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/CMatrixLiverClaude.jpg}
        }
        \vspace{-.2in}
        \caption{Claude liver c-matrix}
        \label{fig:p3-exp4}
    \end{subfigure}
%\vspace{-.25in}
%    \captionsetup{font=small, justification=raggedright}
    \caption{Confusion matrices}
    \label{fig-ConfusionMatricesLiver}
    %\vspace{-.15in}
\end{figure}

\begin{figure}[t!]
%\vspace{-.12in}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{128pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/EntropyGPTClaude.jpg}
        }
        \vspace{-.15in}
        \caption{Entropy}
        \label{fig:p3-exp34}
    \end{subfigure}
    \hspace{-0.1in}
    %\vspace{-.05in}
    \begin{subfigure}[b]{0.34\textwidth}
        \centering
        \resizebox{\linewidth}{131pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/WDHepatitisGPT-Claude.jpg}
        }
        \vspace{-.15in}
        \caption{WD \%}
        \label{fig:p3-exp35}
    \end{subfigure}
    \hspace{-0.1in}
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        %\vspace{-.1in}
        \resizebox{\linewidth}{128pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/NormalizedMutualInfoGPTClaude.jpg}
        }
        \vspace{-.15in}
        \caption{Norm. MI}
        \label{fig:p3-exp41}
    \end{subfigure}%
%\vspace{-.1in}
%    \captionsetup{font=small, justification=raggedright}
    \caption{Entropy, WD, and normalized MI}
    \label{fig:Study2-WDMI}
     \vspace{-.15in}
\end{figure}


Two primary factors contribute to $\EVINCE$'s improved diagnostic accuracy: (1) structured debates with reasoning encourage LLMs to explore alternative diagnoses in both breadth and depth, leading to more comprehensive analysis and decision-making (see Appendices B and C); and (2) pairing high- and low-entropy LLMs balances exploratory diversity with exploitative stability, resulting in more robust and high-quality decisions, as demonstrated in this second study.

\paragraph{Analysis of Confusion Matrices:}
We use confusion matrices to analyze two LLMs' performance in diagnosing Hepatitis types A to E (Fig. \ref{fig-ConfusionMatricesLiver}):
\begin{itemize}[leftmargin=1.2em, topsep=-.05em, parsep=-.05em]
    \item GPT-4 shows limited accuracy, particularly for types C and D, achieving only 50\% accuracy for types A and B.
    \item Claude exhibits a wider spread of predictions across all Hepatitis types.
\end{itemize}
\vspace{.08in}
These matrices highlight how Claude's flexibility in exploring diverse diagnostic hypotheses aids the debate process. Claude's initial uncertainty (high entropy) brings new information, potentially challenging and correcting GPT-4's more confident (low entropy) predictions. This dynamic interplay exemplifies $\EVINCE$'s balance between exploration and exploitation, leading to more accurate and comprehensive diagnoses.

\paragraph{Observations from Information Metrics:}
\begin{itemize}[leftmargin=1.2em, topsep=-.05em, parsep=-.05em]
    \item Entropy Stabilization: Figure \ref{fig:p3-exp34} shows entropy levels of both LLMs stabilizing after three debate rounds, indicating convergence towards a similar, stable entropy state.
    \item Wasserstein Distance Improvement: Figure \ref{fig:p3-exp35} demonstrates consistent improvement in Wasserstein distance (WD) between the two models' predictions over successive rounds.
    \item Mutual Information Increase: Figure \ref{fig:p3-exp41} reveals a 14\% improvement in normalized mutual information (MI) between GPT-4 and Claude's prediction distributions, suggesting increased shared information throughout the debate.
    \item Convergence of Divergence Metrics: Figure \ref{fig:MI-KL-CE} shows consistent convergence of all divergence metrics.
\end{itemize}

\paragraph{Comparative Performance:}
$\EVINCE$ improves 5 percentile accuracy in diagnosing specific types of liver diseases compared to a baseline approach (Figure~\ref{fig:p3-exp1}), underscoring its capability to handle complex diagnostic scenarios effectively.

\begin{figure}[ht!]
%\vspace{-.12in}
    \centering
    \begin{subfigure}[b]{0.88\textwidth}
        \centering
        \resizebox{\linewidth}{120pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/CovergenceAllMetrics.jpg}
        }
    \end{subfigure}
%\vspace{-.25in}
%    \captionsetup{font=small, justification=raggedright}
    \caption{Convergence of all metrics}
    \label{fig:MI-KL-CE}
     \vspace{-.15in}
\end{figure}




==> Chapter15/Conclusion.tex <==
\section{Concluding Remarks}
\label{sec:conc15}
%\vspace{-.1in}

This chapter introduces $\EVINCE$, a framework designed to facilitate collaborative dynamics among Large Language Models (LLMs) through structured, adversarial debates. Our research demonstrates that $\EVINCE$ significantly advances the pursuit of Artificial General Intelligence (AGI) by enhancing three core characteristics: versatility, adaptivity, and reasoning capability. By addressing key limitations of current AI systems, including hallucination, bias, and limited reasoning, $\EVINCE$ provides a novel pathway towards more robust and capable AI.

The core strength of $\EVINCE$ lies in its three theoretical pillars: Inclusiveness Exploration, Information Flow Dynamics, and Reasoning Quality and Coherence. These pillars, grounded in conditional statistics and information theory, enable LLMs to transcend their typical ``maximal likelihood'' behaviors, mirroring human adaptability in linguistic tasks. The integration of the $\CRIT$ system, which combines Socratic methods with formal reasoning techniques, further enhances critical thinking and ensures logically sound and objective-aligned collective reasoning.

Our empirical validation demonstrates $\EVINCE$'s effectiveness in improving prediction accuracy across various domains, notably achieving a 5\% improvement in medical diagnosis tasks. The framework has also shown promise in identifying biases in news articles \cite{SocraPedia2024}, showcasing its potential for broader applications in fields such as geopolitical analysis \cite{MiddleEast-October2023} corporate planning \cite{SocraPlan2023}, and emotional behavior modeling \cite{chang2024MIPR}.

While $\EVINCE$ has demonstrated significant potential, our future work will focus on refining key aspects of the system. We aim to enhance the contentiousness parameter by tying it more rigorously to metrics such as Wasserstein distance, mutual information, and $\CRIT$ scores. Additionally, we plan to explore alternative methods for inducing dual-entropy conditions, moving beyond current parameters like temperature and top-k selection.

Comprehensive ablation studies will be crucial in determining optimal configurations for various applications, ensuring adaptability to diverse contexts and challenges. Through these continued refinements and explorations, we aim to push the boundaries of collaborative AI frameworks, bringing us closer to realizing the full potential of artificial general intelligence.

In conclusion, $\EVINCE$ represents a significant step forward in AI research, offering a structured approach to leveraging the collective intelligence of multiple LLMs. By addressing current limitations and enhancing key AGI characteristics, $\EVINCE$ paves the way for more versatile, adaptive, and capable AI systems, bringing us closer to the goal of artificial general intelligence.

\begin{comment}

\section*{Acknowledgements}

This work has been significantly shaped by insights from several key figures in the field. Microsoft CSO Eric Horvitz's concept of ``polydisciplinary'' representation in LLMs was a major influence. Demis Hassabis of DeepMind provided valuable input on end-to-end architecture without human interference. Prof. Stuart Russell's assertion that LLMs mimic human linguistic behavior to achieve goals was pivotal in our approach to modeling linguistic behaviors and utilizing Bayesian frameworks.

My colleague Prof. Vaughan Pratt's feedback on the initial paper \cite{DiscoveringUnknownChang-July2023} inspired the use of ``contentiousness'' to foster adversarial debate, a key component of our framework. I am grateful to Prof. Monica Lam for her collaborative support throughout this research. Additionally, I thank my colleagues at Stanford Clinical Mind AI for their invaluable domain knowledge in disease diagnosis.
    
\end{comment}

%EVINCE is grounded in its application of conditional statistics, information theory, and dual entropy. These foundational theories facilitate a synergistic interaction among LLMs. By assigning adversarial roles to the models, the framework encourages a broadening of perspectives and, through mutual persuasion, enhances prediction accuracy.

%While a 14\% increase in normalized mutual information (NMI) shown in the second case study is notable, it is not a universal number that can be achieved for all debate matters. The practical significance of such improvements in terms of diagnostic accuracy, clinical decision-making, and patient outcomes may vary depending on the specific use case and the healthcare context. Future work could involve conducting further statistical analyses and gathering expert medical knowledge to better understand the implications of these improvements in real-world healthcare settings.

%Future research should also consider the ethical implications and potential biases that may arise when integrating AI systems into clinical decision-making processes, and develop strategies to mitigate these risks.


==> Chapter15/Introduction-V1.tex <==
\section*{Introduction}
\label{sec:intro15}

The pursuit of Artificial General Intelligence (AGI) remains a central goal of AI research. We propose a paradigm shift in this quest: utilizing multiple Large Language Models (LLMs) engaged in synergistic dialogues as a crucial step towards AGI. This approach, we contend, addresses key limitations of current AI systems and provides a novel pathway to more robust, versatile, and capable artificial intelligence. Specifically, our work targets three core AGI characteristics: versatility, adaptivity, and reasoning capability.

Despite their remarkable capabilities, current LLMs face significant challenges, including hallucination, bias, and limited reasoning. We posit that multi-agent dialogue systems offer a promising avenue to address these challenges. By fostering diversity and debate among LLMs, these systems can mitigate biases by exploring various perspectives and promote enhanced reasoning capabilities. The iterative nature of multi-round dialogues allows for continuous context enrichment, enabling more precise information access and accurate responses, thus reducing hallucinations.

Our previous work, SocraSynth \cite{ChangSocraSynthCSCI2003}, addresses LLM limitations through structured multi-agent dialogues. By leveraging both adversarial and collaborative interactions between LLMs, SocraSynth demonstrates quantifiable improvements across various domains. In healthcare, it achieves a 5\% improvement in diagnostic accuracy \cite{SocraHealth2023}, while in news analysis, it identifies and explains biases in articles \cite{SocraPedia2024}. These advancements showcase enhanced versatility, adaptivity, and reasoning capability---key AGI characteristics.

SocraSynth, our previous work~\cite{ChangSocraSynthCSCI2003}
presented in Chapter~\ref{chap:SocraSynth}, addresses LLM limitations through structured multi-agent dialogues. By leveraging both adversarial and collaborative interactions between LLMs, SocraSynth demonstrates quantifiable improvements across various domains, including healthcare \cite{SocraHealth2023}, news analysis \cite{SocraPedia2024}, geopolitical analysis \cite{MiddleEast-October2023}, corporate planning \cite{SocraPlan2023}, and emotional behavior modeling \cite{chang2024MIPR,chang2024integrating}. These results highlight SocraSynth's potential for advancing towards AGI's generalized problem-solving capabilities.

While effective, SocraSynth relies on a qualitative measure of ``contentiousness'' to moderate LLM linguistic behaviors. This chapter extends SocraSynth by introducing $\EVINCE$ (Entropy and Variation IN Conditional Exchanges) \cite{EVINCEChang2024}, a framework comprising three theoretical pillars to quantify ``contentiousness'' and moderate dialogues based on statistical and information theories.

The three pillars of $\EVINCE$ are:

\begin{enumerate}[leftmargin=1.2em, topsep=-.05em, parsep=-.05em]
\item \textit{Inclusiveness Exploration}:
We develop methods to ensure dialogues explore all potential perspectives. We use conditional statistics via in-context learning \cite{xie2021explanation} to ``free'' an LLM agent from its default ``maximal likelihood'' next-token prediction behavior, allowing it to adopt specific stances. We introduce a dual entropy optimality theory to balance the exploration of new ideas with adherence to priors, thus optimizing information exchange between agents for comprehensive and stable discourse.

\item \textit{Information Flow Dynamics}:
We introduce information theory-based metrics to quantify and optimize dialogue dynamics. These measure information diversity (entropy), novelty (statistical divergence scores), and inter-agent persuasion (mutual information). These metrics enable us to assess and enhance the quality and efficiency of information flow within the multi-agent system, fostering rich and productive exchanges.

\item \textit{Reasoning Quality and Coherence}:
We establish frameworks to assess the logical structure and coherence of multi-agent reasoning. This pillar evaluates argument validity, analytical depth, and dialogue coherence. We synergistically integrate our previously developed $\CRIT$ system \cite{SocraticIEEECCWC2023} into SocraSynth. 
$\CRIT$, which combines Socratic methods with formal reasoning techniques, enhances our ability to conduct critical thinking through evaluating argument quality, information-source credibility, and overall ``reasonableness'' within the dialogue. This integration ensures that the collective reasoning of LLM agents is not only diverse but also logically sound and aligned with the dialogue's objectives.
\end{enumerate}

The core strength of SocraSynth and $\EVINCE$ in advancing towards AGI lies in their ability to enhance key AGI characteristics through multi-agent dialogues. By employing conditional statistics and information theory, they boost versatility and adaptivity, allowing LLMs to transcend their typical ``maximal likelihood'' behaviors and mimic how humans adapt their linguistic behaviors to complete tasks. The framework's debate structure fosters advanced reasoning and critical thinking capabilities. Together, these advancements represent significant steps towards achieving the complex, intricate capabilities required for AGI.

The main contributions of this work are:

\begin{enumerate}[leftmargin=1.2em, topsep=-.05em, parsep=-.05em]
\item {\textit{EVINCE} Framework Design}:
Unlike approaches that use debate merely to improve accuracy via redundancy, $\EVINCE$ facilitates information discovery, bias mitigation, and decision-making that requires both breadth and depth of information.

\item \textit{Theoretical Foundations}: We establish a theoretical basis for $\EVINCE$, rooted in conditional Bayesian statistics, mutual information, and dual entropy. These principles are applied to measure, monitor, and modulate collaborative LLM interactions, contributing to a deeper understanding of how LLMs can effectively cooperate for improved decision-making. The dual entropy theory is novel and ground-breaking, illustrating how a productive decision-making process should start with room for diverse input and stable objectives, and then, through information exchange, converge to optimal decision/prediction.

\item \textit{Empirical Validation}: We provide empirical validation of theories, highlighting $\EVINCE$'s effectiveness in balancing exploration and exploitation to enhance prediction accuracy. We also introduce a set of maxims derived from our empirical findings, offering practical guidance for optimizing mutual information and minimizing various divergence measures.
\end{enumerate}

\begin{comment}
The remainder of this chapter is structured as follows:
Chapter~\ref{sec:related15} discusses related work and addresses common 
misconceptions about our approach.  
Chapter~\ref{sec:evince15} presents the three pillars of $\EVINCE$, including its
maxims, theories, and algorithms. 
Chapter~\ref{sec:exp15} provides empirical evidence of $\EVINCE$'s benefits by revisiting and expanding upon previous SocraSynth experiments in healthcare and bias detection.
Chapter~\ref{sec:conc15} offers concluding remarks and discusses future directions.
\end{comment}

==> Chapter15/Table-Contentiousness.tex <==
\begin{table*}[t!]
  \centering
  \includegraphics[width=0.98\linewidth]{Chapter5SocraSynth/Table5.5.1.png}
  \vspace{-.1in}
\caption{\small{Linguistic Behaviors at Different Contentiousness Levels.}}
\label{tab:contentiousness15}
  \vspace{-.15in}
\end{table*}    

%\section*{Appendix G: Contentiousness Parameter Modulation}

\begin{comment}

Table~\ref{tab:contentiousness} presents 
how an LLM adjusts its linguistic behavior 
after the value of the ``contentiousness'' parameter.
By modulating contentiousness, it has been shown
that an LLM can condition itself to 
adapt to different linguistic behaviors to
achieve a new establish goal and context.
Details are presented in \cite{SocraSynthChang2023} and
also illustrated in Section~\ref{sec:exp}.
    
\end{comment}

==> Chapter15/Table-EDTProof.tex <==
\begin{table*}[th!]
\vspace{-.1in}
\centering
\begin{scriptsize}
\begin{tabular}{|>{\raggedright\arraybackslash}m{0.98\textwidth}|}
\toprule
\noindent \textbf{Theorem EDT: Optimal Pairing of LLMs for Probabilistic Prediction.}
\\
The optimal pairing of LLMs for probabilistic prediction accuracy, in terms of stability, accuracy, and robustness, occurs when the LLMs are 1) equivalent in the quality of the information they process, and 2) exhibit contrasting entropy values in their prediction distributions—one high and one low.

\begin{proof}

Given two LLMs, LLM$_A$ and LLM$_B$, following Maxim \#1 with prediction distributions $P_A$ and $P_B$, respectively. The entropy of LLM$_A$, $H(P_A)$, is high, and of LLM$_B$, $H(P_B)$, is low.

\vspace{.1in}
\noindent \textbf{Step 1: }{Define combined prediction distribution.} Let the combined prediction distribution of LLM$_A$ and LLM$_B$ be denoted as $P_C$. We can express $P_C$ as a weighted average of $P_A$ and $P_B$:
\begin{tiny}
\vspace{-0.1in}
\[
P_C = \alpha P_A + (1 - \alpha) P_B, \quad \text{where } 0 \leq \alpha \leq 1, 
%\]
%\vspace{-0.2in}
%\[
\text{ where } \alpha \text{ is decided by CRIT, WD, MI, etc. }
\]
\end{tiny}
\vspace{-0.15in}

\noindent \textbf{Step 2: }{Express the information entropy of the combined prediction distribution.}
Using the definition of information entropy, we calculate:
\vspace{-0.1in}
\begin{tiny}
\[
H(P_C) = -\sum_{i} P_C(x_i) \log_2 P_C(x_i) 
\]
\end{tiny}
\vspace{-0.2in}
\begin{tiny}
\[
= -\sum_{i} [\alpha P_A(x_i) + (1 - \alpha) P_B(x_i)] \log_2 [\alpha P_A(x_i) + (1 - \alpha) P_B(x_i)].
\]
\end{tiny}
\vspace{-0.1in}

\noindent \textbf{Step 3:} {Apply Jensen's Inequality to the information entropy of the combined prediction distribution.}
Jensen's inequality is applied to the convex function $f(x) = -x \log_2 x$. For a convex function and a set of probabilities $p_i$, Jensen's inequality states that:
\begin{tiny}
\vspace{-0.1in}
\[
f\left(\sum_{i} p_i x_i\right) \leq \sum_{i} p_i f(x_i)
\]
\end{tiny}
Thus, the entropy of the combined distribution is:
\begin{tiny}
\vspace{-0.1in}
\[
H(P_C) \geq \alpha H(P_A) + (1 - \alpha) H(P_B),
\text{where equality holds when }P_A = P_B.
\]
\end{tiny}
%\vspace{-0.1in}

\noindent \textbf{Step 4:} {Analyze the lower bound of the combined information entropy.}
As $H(P_A)$ is high and $H(P_B)$ is low, we can express their relationship as:
\vspace{-0.1in}
\begin{tiny}
\[
H(P_A) = H(P_B) + \Delta, \quad \text{where } \Delta > 0.
\]
\end{tiny}
%\vspace{-0.1in}
Substituting this into the inequality from Step 3, we have:
\vspace{-0.1in}
\begin{tiny}
\[
H(P_C) \geq \alpha [H(P_B) + \Delta] + (1 - \alpha) H(P_B) = H(P_B) + \alpha \Delta.
\]
\end{tiny}
\vspace{-0.2in}

\noindent \textbf{Step 5:} {Interpret the lower bound of the combined information entropy.}
The lower bound of $H(P_C)$, and hence the robustness of the model, is maximized when $\alpha$ is maximized, which corresponds to giving more weight to the high-entropy model (LLM$_A$). This setup facilitates the exploration of diverse possibilities and enhances robustness against noise and perturbations in the input data, while still ensuring that predictions are grounded by the more certain outcomes predicted by the low-entropy model (LLM$_B$).
\vspace{0.05in}

\noindent \textbf{Step 6:} {Conclude the proof.}
By combining the prediction distributions of LLM$_A$ and LLM$_B$, with one having high entropy and the other low, we achieve an optimal balance that maximizes the lower bound of the combined entropy. This balance between exploration (high entropy) and exploitation (low) optimizes overall prediction accuracy, as proved through information theory and the properties of entropy. Thus, the theorem is established.
\end{proof}
\vspace{-.35in}
\\
\bottomrule
\end{tabular}
\end{scriptsize}
\vspace{-.05in}
\caption{\small{Proof of Entropy Dual Theorem (EDT)}}
\label{tab:EDTProof}
\vspace{-.2in}
\end{table*}

==> Chapter15/TableMetrics-Book.tex <==
\begin{table*}[th!]
\vspace{-.1in}
%\begin{customsize}
\begin{tiny}
\centering
\begin{tabular}{|p{1.6cm}|p{2.3cm}|p{2.3cm}|p{2.6cm}|}
\toprule
\hline
\textbf{Metric} & \textbf{Pros} & \textbf{Cons} & \textbf{Remedies} \\
\hline
Cross Entropy \cite{Shore1980AxiomaticDO} & Measures how well the predictions of one model fit the actual distribution of another model’s outputs (asymmetric). & Computationally intensive with large models and data sets; sensitive to the exact nature of prob dists. & Optimize computation strategies; use approximations or sampling methods to manage large data sets or complex models. \\
\hline 
Entropy Shannon \newline \cite{shannon1948} & Indicates level of diversity; high suggests exploration of possibilities, and low for confidence on few choices & High entropy might indicate noise rather than useful diversity; low entropy might mask important variability. & Use critical reading methods (Appendix A) to assess argument quality; implement noise detection to differentiate between useful diversity and noise. \\
\hline
Jensen-Shannon \newline Diverg.\newline \cite{lin1991divergence} & Symmetric, bounded (0 to 1), an interpretable measure of distributional differences. & May be less sensitive to small differences between distributions. & Increase sensitivity settings or resolution of the metric; combine with other metrics to capture finer distinctions between distributions. \\
\hline
KL Diverg. \cite{kullback1951information} & Measures difference between two probabilistic distributions. & Asymmetric; not well-defined if a distribution has zero probabilities & Use smoothing techniques to avoid zero probabilities; consider symmetric alternatives like JS divergence \\
\hline
Mutual Info \cite{Shore1980AxiomaticDO} & Measures reduction of uncertainty; symmetric. & Does not indicate the direction of info flow. & Supplement with direction info metrics; normalized with max entropy of A and B. \\
\hline
Wasserstein \newline Distance (WD) \cite{kantorovich1942translocation} & Direct measure of how similar or different the model outputs are; symmetric relationship.  & Not bounded but can be normalized or bounded for consistent interpretation. & Define context-specific bounds for low, medium, and high divergence; consider normalizing it for non-directional comparisons. \\
\hline
\bottomrule
\end{tabular}
%\end{customsize}
\end{tiny}
%\vspace{-0.1in}
\caption{Summary of metrics for assessing LLM debates}
\label{tab:metrics}
%\vspace{-0.1in}
\end{table*}


==> Chapter16/Conclusions.tex <==
\section{Concluding Remarks}
\label{sec:conc16}

Recent declarations by \cite{Bengio_2024} and \cite{dalrymple2024guaranteed} underscore the importance of addressing AI risks and safety concerns given the technology's rapid advancement. This chapter addresses
AI safety and ethics with emotional and ethical modeling.

Our exploration of the Behavioral Emotion Analysis Model (BEAM) and the Wheel of Virtues aims to enhance the capabilities of LLMs in understanding and emulating human emotions and ethical behaviors through linguistic behaviors. BEAM serves as a guide for LLMs to comprehend and replicate the complex spectrum of human emotions through linguistic features, essential for tasks such as novel writing or empathetic interactions, while the Wheel of Virtues provides a structured framework for embedding ethical decision-making in LLMs, tailored to both universal and regional/culture dependent ethical standards.

The development of these frameworks represents a novel contribution to AI safety, offering an interpretable and innovative approach to imbuing LLMs with a deeper understanding of human-like emotional and moral intelligence.

While we recognize the promising nature of this work, we also acknowledge that there is much more to explore and refine. Our ongoing endeavors aim to further advance this field (e.g., \cite{chang2023cocomo,EVINCEChang2024,MirrorChang2024,SocraticIEEECCWC2023}). The journey to fully equip LLMs with the ability to navigate the complex landscapes of human emotions and ethics is important and ongoing. Our contribution represents a step toward realizing more emotionally aware and ethically aligned artificial intelligence systems.

==> Chapter3/Conclusion.tex <==
\section{Concluding Remarks}

his chapter discusses query processing with large language models (LLMs) to enhance the quality of responses. Effective questioning involves clarifying the intent and providing relevant context to the LLM.

The chapter reviews recent studies post-GPT-3, focusing on prompt engineering (formulating questions) and retrieval augmented generation (RAG) (supplementing the LLM with additional information for better responses). These methods, mainly heuristic, have shown good results.

With advancements in LLMs, like GPT-4's 128k token buffer and Gemini's one million, compared to the previous 8k, these models can now process and utilize vast data to identify pertinent context. RAG is still used, mainly due to cost-efficiency, as GPT-4 and Gemini incur fees based on the number of tokens processed.

There are two persistent challenges. First, crafting effective questions can be tough, especially when the LLM may have more information than the user. Second, determining which external data to retrieve for high accuracy and recall in answers is an ongoing research issue.

Chapter \ref{chap:SocraSynth} will introduce strategies to improve question formulation. Chapter \ref{chap:RAFEL} will present how the system $\Rafel$ can effectively manage context buffer, aiding LLMs in providing better answers.

==> Chapter3/RAG.tex <==
\section{RAG}
\label{sec:RAG}


Retrieval-Augmented Generation (RAG) is a technique to improve the capabilities of Large Language Models (LLMs) in various applications. LLMs are effective in reasoning about various topics, but their knowledge is limited to the data they were trained on. RAG injects relevant external data retrieved from a source (indexed beforehand) to enhance the LLM's response for specific 
user queries. The RAG technique complements to
prompt engineering, which formulates a good
query. Figure~\ref{fig:RAG_Arch} depicts a typical
RAG architecture. 

\begin{figure}[t!]
  \centering
    \vspace{-.2in}
  \includegraphics[width=1.08\linewidth]{Chapter3/RAGDiagram.png}
  \vspace{-.1in}
  \caption{RAG Architecture and Data Flow.  RAG bring data to LLM to integrate and generate content.}
  \label{fig:RAG_Arch}
\end{figure}



\subsection{RAG with Limited-Context LLMs}

A recent survey paper \cite{SurveyRag2024} discusses
the techniques employed by RAG and
relevant work (see Figure~\ref{fig:RAG_evolution})
in three categories:

Retrieval Techniques: Techniques like recursive retrieval, adaptive retrieval, iterative retrieval, and others are explored. Recursive retrieval involves refining search queries based on previous results to converge on pertinent information. Adaptive retrieval methods, exemplified by Flare and Self-RAG, allow LLMs to determine optimal moments and content for retrieval. Iterative retrieval in RAG models repeatedly collects documents to provide a comprehensive knowledge base for LLMs, enhancing answer generation robustness.


Generation Techniques: The generator in RAG is crucial for converting retrieved information into coherent text. Unlike traditional models, RAG's generator uses retrieved data to improve accuracy and relevance. Post-retrieval processing with a frozen LLM involves treating, filtering, or optimizing retrieved information to align it more closely with user needs or subsequent tasks. Techniques like information compression and reranking are employed to enhance retrieval results quality.

Augmentation Techniques: The data sources
are the key for RAG to work effectively.
It is evident if one asks for information
about medicine, but the data source is
about construction, the noises may
be louder than the signals. Data augmented
data can be unstructured data, structured data, or content generated by LLMs themselves. There
are several augmentation processes like iterative, recursive, and adaptive retrieval, emphasizing refining the retrieval process to address challenges like redundancy and limited scope of information.

In summary, RAG is about putting the most relevant
information to answer a query into the limited
context window. The techniques 
are not new as dealing with memory hierarchy
effectively to reduce latency and improve throughput
has been a subject of research for over three decades in hardware design and database management.

\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.98\linewidth]{Chapter3/rag-evolution.png}
%  \vspace{-.1in}
  \caption{RAG Representative Work (credit \cite{SurveyRag2024}).}
  \label{fig:RAG_evolution}
  \vspace{-.1in}
\end{figure}

\subsection{RAG with Long-Context LLMs}

The release of GPT-4-turbo with $128$k token context window
and the Gemini 1.5 Pro's 1 million token context 
window \cite{gemini2023unlocking} allows massive amounts of information 
be be retrieved into the context buffer.  This 
large context window clearly alleviate the challenges of 
fining the most relevant information for RAG to retrieve
to improve query results.  One may even claim
that the entire line of RAG optimization work 
is rendered obsolete because relying on
LLMs themselves to locate relevant data in its
massive context window is superior to 
any approaches
based on human heuristics. With the advancements
of LLMs, any heuristic-based band-aids will eventually
be rendered ineffective.
Naturally, this sparked discussions about the potential obsolescence of RAG techniques, e.g., \cite{SurveyRag2024,LLamaIndex2024}.

\subsubsection*{High Precision and Recall}

In synthetic tasks designed to emulate the ``needle-in-a-haystack'' scenario, inspired by Kamradt \cite{kamradt2023needle}, the Gemini team assess the ability of Gemini 1.5 Pro to accurately recall specific information amidst a vast amount of irrelevant or distracting data. Its
findings \cite{gemini2023unlocking} reveal that the Gemini 1.5 Pro model demonstrates exceptional recall accuracy, exceeding 99\%, across various data types, including text, video, and audio. This high level of recall accuracy is maintained even when the model is challenged with up to multiple millions of tokens of irrelevant data, or ``haystack.'' In the text modality, Gemini 1.5 Pro continues to exhibit this remarkable recall performance even when the ``haystack'' is expanded to 10 million tokens.
The report also claims that better understanding
and reasoning are observed on their multimodal
benchmarks.  

\subsubsection*{Low Latency and Cost}

While Gemini can handle much larger contexts, the author 
of \cite{LLamaIndex2024} argues that RAG remains valuable for several reasons:

\begin{enumerate}[left=0em,label=\arabic*.]
\item \textit{Chunking for Efficiency}:  Large documents might still overwhelm the LLM. RAG's chunking process helps break down documents into digestible pieces for retrieval before feeding them to the model.

\item \textit{Cost-Effectiveness}: Traditional RAG approaches might be more economical for specific use cases, especially when dealing with large knowledge bases (terabytes). 
Smaller chunks are indexed and retrieved initially, but they act as pointers to larger chunks that ultimately get fed to the LLM for synthesis.
Constantly feeding a 1 million token window to the LLM can be expensive.
\end{enumerate}

The article \cite{LLamaIndex2024} concludes by emphasizing that long-context LLMs like Gemini are a significant leap forward. However, they likely won't render RAG obsolete. Instead, the future of LLM applications will involve a collaboration between these two approaches.

==> Chapter3/Shots.tex <==
\section{Prompting Methods}
\label{sec:shots}

Prompting methods, especially in the context of LLMs like GPT-4, are strategies used to elicit specific responses from the model. These methods vary based on the amount of information or context given to the model. This section provides a list of common prompting methods, along with their definitions, pros and cons, and examples for querying facts, opinions, and reasons or explanations:

\subsection{Zero-shot}

Zero-shot Learning: The model generates a response based on a single input without any previous examples or context.
The LLM model is given a task without any prior examples of how to perform it. A task can be any NLP tasks such as translation,
summarization, classification, and Q$\&$As. 

In the context of querying a language model, you can ask for various types of information or responses, such as facts, opinions, or explanations. For instance, you might ask for a fact by inquiring, ``What is the capital of France?'' or seek an opinion with a question like, ``What do you think about the use of AI in education?'' Alternatively, you could request an explanation or reason, as in asking, ``Explain why the sky is blue.'' These queries demonstrate the model's versatility and its ability to handle a range of inquiries without the need for task-specific data. This approach is quick and adaptable, allowing for a broad spectrum of questions to be addressed. However, it's important to note that the responses may not always be as accurate as they might be when more context or examples are provided to the model, highlighting a trade-off between convenience and depth of response.

For zero-shot learning, a constraint can be observed when asking a complex, multi-faceted question that requires deep understanding or synthesis of ideas. An example might be, ``Assess the impact of Renaissance art on modern graphic design.'' Without prior examples, the model might struggle to provide an insightful analysis 
to meet unspoken expectations due to the broad and intricate nature of the question, reflecting the zero-shot learning's limitation in handling complex queries without context.

\subsection{One-shot}

One-shot Learning: The model is provided with a single example to guide its understanding of the task.

In the one-shot learning method, an example is provided before posing a question, helping guide the model's response. For instance, when asking about a fact, one might say, ``The capital of Italy is Rome. What is the capital of France?'' This method can also be used to solicit opinions or explanations. For example, to elicit an opinion, you could say, ``AI in healthcare is beneficial. What is your opinion on AI in finance?'' Similarly, for an explanation, one might ask, ``Plants need sunlight to perform photosynthesis. Why do humans need to eat food?'' This approach offers more context than zero-shot learning, potentially improving the model's accuracy by providing
an example. However, it still largely depends on the model's inherent knowledge and biases, which can affect the precision and relevance of the responses.

\subsection{Few-shots}

Few-shot Learning: The model is provided with a few examples to guide its understanding of the task.

In the few-shot learning method, multiple examples are provided before a question to better guide the model's response. For instance, when seeking a factual answer, one might say, ``The capital of Brazil is Brasilia. The capital of Egypt is Cairo. What is the capital of France?'' This approach is also applicable for eliciting opinions or explanations. For opinions, one could present, ``AI in healthcare improves patient outcomes. AI in automotive can reduce accidents. What is your opinion on AI in education?'' For explanations, a prompt might be, ``Water boils at 100°C because at this temperature water molecules have enough energy to change state. Leaves are green because they contain chlorophyll. Why do apples fall from trees?'' This method, by providing more context, aims to enhance the model's performance and the relevance of its responses. However, it requires additional effort to generate quality examples, which significantly impact the outcomes, illustrating the trade-off between the effort invested in preparing examples and the quality of the generated responses.

Few-shot learning tends to outperform one-shot and zero-shot learning for more complex tasks because it provides more examples to help the model understand the context or expected output. However, for simpler tasks, zero-shot or one-shot learning might be sufficient and more efficient. However, to ensure few-shot and one-shot 
learning can definitely improve 
results, the quality and relevance of the examples provided
is essential. Poor or irrelevant examples can lead 
to worse outcomes than a zero-shot approach, where 
the model relies solely on its pre-trained knowledge.

\subsection{Chain of Thought}

Chain-of-thought Prompting \cite{ChainOfThought2022}: This method involves guiding the model through a series of logical steps to reach a conclusion, especially useful for complex reasoning tasks.
The prompt includes a step-by-step breakdown of how to approach a problem or question, encouraging the model to follow a similar thought process.

Chain-of-thought prompting in LLMs involves guiding the model through a logical sequence to address a question, providing a clear rationale for each step. For example, to gather an opinion, one might prompt, ``To form an opinion on a topic, one should consider various perspectives and their implications. What is your opinion on the use of drones in delivery services?'' For an explanation, the approach could be, ``To explain why leaves change color in autumn, one must understand the process of chlorophyll breakdown and the exposure of other pigments. Explain why ice floats on water.'' While chain-of-thought prompting can enhance the model's performance on complex tasks by encouraging a stepwise approach to reasoning, it also presents challenges. Creating effective chain-of-thought prompts is often time-consuming and requires a deep understanding of the problem at hand, highlighting the balance between the method's potential benefits and its demands. 

Chain-of-thought prompting has its limitations. One primary critique is that it relies on the assumption that the model can mimic a logical sequence of human thought, which might not always align with the actual complexity and subtlety of human reasoning. Since these models generate responses based on patterns observed in their training data, there's no guarantee that the ``thought process'' they follow truly reflects sound reasoning or factual accuracy\textendash it might just be a plausible narrative based on learned associations.

Another critique is that this approach leans heavily on abductive reasoning, which involves forming a probable conclusion from the information available, rather than guaranteeing the truth of that conclusion. While abductive reasoning can be powerful, it can also lead to biases and errors if the model's training data has gaps, inaccuracies, or biases, which it likely does.

\subsection{Three of Thought}

Three-of-thought \cite{yao2023tree} was proposed to remedy
one single chain-of-thought.  Its aims are:
\begin{enumerate}[left=0em,label=\arabic*.]
    \item \textit{Improving Reasoning Coverage:} Exploring various potential reasoning paths might increase the robustness and reliability of the conclusions.
    \item \textit{Reduced Bias:} Considering multiple pathways might help mitigate the biases inherent in a single line of reasoning.
\end{enumerate}

However, buying three bottles of milk does not ensure higher
quality than buying one bottle.  The ``tree-of-thought'' approach, while conceptually offering a broader perspective by exploring multiple reasoning paths, indeed faces significant challenges that might not make it universally superior to the ``chain-of-thought'' method. Here are some critiques along with potential remedies:

\begin{enumerate}[left=0em,label=\arabic*.]
\item \textit{Complexity in Formulation}: If formulating one coherent and logical chain is challenging, creating multiple such chains that are logically sound and relevant can be even more daunting. The quality of each chain within the tree is crucial, and poor-quality chains can detract from the overall effectiveness of the model.

\item \textit{Comprehensiveness}: Having multiple paths doesn't guarantee that they cover all possible or relevant lines of reasoning. There's a risk of missing critical reasoning paths or including irrelevant ones.

\item \textit{Path Selection}: With multiple paths available, selecting the most accurate or relevant path becomes a challenge. The model needs a reliable mechanism to evaluate and choose the best path, which is non-trivial in complex reasoning scenarios.

\item \textit{Knowledge Gaps}: In open-domain reasoning, it's possible that a link in the reasoning chain lacks external knowledge support, leading to a dead-end or incorrect conclusion.
\end{enumerate}

\subsection{Further Improvement Techniques}

To address these limitations, one advanced remedy could involve incorporating feedback loops where the model's outputs are evaluated and corrected by human experts, and these corrections are fed back into the system for continuous learning and adjustment. This could help align the model's reasoning more closely with accurate and logical thought processes.

Another remedy might involve the retrieval and
integration of structured knowledge bases or databases that the model can query as part of its reasoning process, ensuring that its responses are grounded in verified information rather than just patterns in text. 
We will discuss Retrieval-Augmented Generation (RAG) in the next section.

Lastly, enhancing the training process with a more diverse and robust dataset, including examples of logical reasoning and problem-solving across various domains, could improve the model's ability to simulate a chain of thought more effectively and accurately.


\subsection{Illustrative Examples}

We provide three sets of examples to illustrate the
differences of capabilities in the five kinds of prompts.

\subsubsection{``What'' Prompt Example}

\begin{itemize}
  \item \textit{Zero-shot:} Directly ask the model without any examples, ``What is the capital of France?''
  \item \textit{One-shot:} Provide a similar example before asking the question, ``The capital of Japan is Tokyo. What is the capital of France?''
  \item \textit{Few-shots:} Give multiple examples before asking the question, ``The capital of Italy is Rome. The capital of Germany is Berlin. What is the capital of France?''
  \item \textit{Chain of Thought:} Encourage the model to break down the question into logical steps, ``To find the capital of France, consider major cities in France and identify which one is the administrative center. What is the capital of France?''
  \item \textit{Tree of Thought:} Use a structured approach, asking about different aspects of France first, then honing in on the capital, ``What are the major cities in France? Among these, which one is recognized as the capital? What is the capital of France?''
\end{itemize}

This example demonstrates a remembering question.  For such type
of questions, one may think either the LLM knows it or not.
However, even the LLM does not have the information about the capital
of France, a chain-of-thought prompt may indirectly find the
answer.  

\subsubsection{``Why'' Prompt Example}

This example involves in reasoning. 
Different prompting methods can elicit varied responses, demonstrating the model's adaptability.

\begin{itemize}
  \item \textit{Zero-shot:} Asking ``How can a plant grow faster?'' without providing any context or previous examples.
  
  \item \textit{One-shot:} ``Providing adequate water helps a plant grow. How can a plant grow faster?'' This gives the model a reference point for generating its answer.
  
  \item \textit{Few-shots:} Providing multiple examples before the question, such as ``Sunlight is essential for photosynthesis. Nutrients in the soil contribute to plant growth. How can a plant grow faster?'' helps the model understand the context better.
  
  \item \textit{Chain of Thought:} Encouraging the model to break down the question, ``Consider the factors affecting plant growth like sunlight, water, and nutrients. How can optimizing these factors make a plant grow faster?''
  
  \item \textit{Tree of Thought:} Structuring the approach by considering different aspects, ``What are the essential elements for plant growth? How does each element contribute to faster growth? How can we optimize these elements for plant growth?''
\end{itemize}

\subsubsection{Many-Shots Example}

\begin{comment}
\begin{table}[th!]
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.5cm}|p{10.0cm}}
\toprule
Role & Dialogue \\
\midrule
Statement & {``I was laid off by my company today!''} \\
\midrule
{Positive } & {``I'm so sorry to hear that. Losing your job can be a really tough and stressful experience. How are you doing?'' } \\
Positive & {``That must have been a really difficult and unexpected news. I'm here to listen and support you however I can.''} \\
Positive & {``I can imagine how hard and unsettling it must have been to receive that news. Is there anything you'd like to talk about or anything I can do to help?''} \\
\midrule
{Negative } & {``That's too bad, but there are plenty of other jobs out there. You'll find something soon enough.''} \\
Negative & {``Well, you probably weren't very good at your job if they let you go.''} \\
Negative & {``I don't know why you're so upset about this. It's not like it's the end of the world.''} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
%\vspace{.1in}
\caption{Example \#1. Template for Being Empathetic.}
\label{tab:Noora}
%\vspace{-.1in}
\end{table}
\end{comment}


In summer 2022, three interns at OVAL developed a chatbot named Noora (described in \cite{NooraStanford2022}) to assist children with artistic talents in learning empathy. This project aimed to help children with autism spectrum disorder (ASD) develop empathetic communication skills.

The approach involved providing the GPT-3 language model with context and intent, followed by examples illustrating comforting and harmful responses. This setup targets not only behavioral goals but also instilling values, ultimately enhancing the chatbot's understanding of context. With a few hundred examples, Noora can respond appropriately to various situations.

Chatbots, or AI agents, can learn from human demonstrations to adapt to users and environments. By imitating human experts or teachers, agents acquire knowledge and skills, especially when the desired behavior is difficult to express through a reward function in reinforcement learning. Large language models (LLMs) allow for demonstrations through prompts, which serve as templates with instructions, goals, and examples.

A sample prompt to teach GPT-3 empathy starts with clear instructions:
\hfill \break
\textit{``Dear Virtual Assistant,
I'm reaching out because you are a friend and I value your support and understanding. I'd like to share some joys and sorrows I experience daily in hopes that you can respond with compassion and empathy. Here are some example dialogues to illustrate comforting and harmful responses. Each example begins with my statement followed by potential replies.''}

Before initiating a dialogue, the LLM receives the task's intent, allowing it to connect to the external context within the intent statement. This approach requires further validation to confirm its effectiveness. However, observations suggest it can be a useful method to convey values, in addition to goals, to LLMs. This allows them to gain a broader context beyond a limited number of demonstrated examples. Following this initial communication of intent, GPT-3 receives specific examples.

\begin{table}[ht!]
  \centering
  \includegraphics[width=1.0\linewidth]{Chapter3/Table3.3.1.png}
%  \vspace{-.1in}
  \caption{Example \#1. Template for Being Empathetic.}
  \label{tab:Noora}
  \vspace{-.1in}
\end{table}


Table~\ref{tab:Noora} lists six example responses, three positives and three negatives, to a user's statement. The dialogue starts with the user saying, ``I was laid off by my company today!'' followed by examples of good and bad responses. With a few thousand examples like this, the chatbot can respond with an appropriate tone to new statements.

Demonstrations can also teach desired behaviors and ethics. This empathy template can be adapted to model other positive behaviors, like attentiveness and care. While machines can have positive traits like infinite patience, explicitly modeling good and bad behaviors is crucial for effective interaction with human users. Behaviors to avoid include unpleasantness, rudeness, and dishonesty.


==> Chapter4/Conclusions.tex <==
\section{Concluding Remarks}
\label{sec:conc4}

The Socratic method may not always be effective or useful in human interactions, especially when one of the two players is authoritative, emotional, or abusive. However, when the expert partner is a language model, a machine without emotion or authority, the Socratic method can be effectively employed without the issues that may arise in human interactions. In this way, it can be utilized to its full potential in guiding, directing, and improving the output of language models through engineering prompts.

In this chapter, we have explored the use of the Socratic method in engineering prompt templates for language models. We have discussed the importance of method definition, elenchus, dialectic, maieutics, and counterfactual reasoning techniques in guiding the output of these models. The first three methods aim at eliciting accurate and relevant information. Through the use of methods definition, elenchus, and dialectic, we have demonstrated, with examples, the ability to clarify user queries and assess the quality of language model-generated text, leading to improved precision and accuracy.

We have also shown how the methods of maieutics and counterfactual reasoning can be helpful in stimulating the imagination of writers. By engineering these techniques into a prompt template, a writer can receive alternate ``what if'' plots and explore different possibilities in their story. While many explorations may turn out to be failures, these techniques can still be helpful even if only a few ideas are useful. Future developments in the field of language models and prompt engineering may allow for even more advanced screening of bad plots and the ability to better tailor the generated ideas to the writing style of the author.

In conclusion, this chapter has highlighted the potential of using the Socratic method to engineer prompt templates for interacting with language models. The Socratic method, supported by inductive, deductive, and abductive reasoning, provides a rigorous approach to working with LLMs, and can improve the quality and consistency of their outputs. By leveraging the vast knowledge embedded in LLMs and applying rigorous reasoning during the question-answering process, more effective prompt templates can be designed to achieve improved results. Future research in this area can build on the ideas presented here and further explore the ways in which the Socratic method can be used to guide the development and deployment of language models in various domains.

\begin{comment}
The Socratic method may not be effective or useful in a setting where one of the two players is authoritative, emotional, or even abusive. However, when the expert partner is an LLM, a machine without emotion or authority, the method can be effectively employed without the issues that may arise in human interactions. In this way, the Socratic method can be utilized to its full potential in guiding, directing, and improving the output of language models through engineering prompts.

Throughout this paper, we have explored the use of the Socratic method in engineering prompt templates for LLMs. We have discussed the importance of method definition, elenchus, dialectic, maieutics, and counterfactual techniques in guiding the output of these models. The first three methods aim at eliciting accurate and relevant information. Through the use of methods definition, elenchus, and dialectic, we have demonstrated through examples the ability to clarify 
user queries and to
assess the quality of LLM generated text, leading 
to improved precision and accuracy.

To help writers to be productively imaginative, we show that methods maieutics and counterfactual reasoning can be helpful. By engineering these techniques
into a promoting template, a writer may receive alternate ``what if'' plots and explore different possibilities in their story. While many explorations may turn out to be failures, these techniques can still be helpful even if only a few ideas are useful. Future developments in the field of LLM and prompt engineering may allow for even more advanced screening of bad plots and the ability to better tailor the generated ideas to the writing style of the author.

In conclusion, this work has demonstrated the potential of using the Socratic method in engineering prompt templates for interacting with large language models. However, there is still much room for improvement and further research in this area. As language models continue to advance and become more sophisticated, we can expect to see more effective and efficient ways of engineering prompt templates, leading to even more impressive results in the future.
\end{comment}

==> Chapter4/GenesisTable.tex <==

\begin{table}[ht!]
  \centering
  \includegraphics[width=1.0\linewidth]{Chapter4/Table4.4.6.png}
\caption{What if Eve refused to eat the fruit?}
%\vspace{-.1in}
\label{tab:genesis}
  \vspace{-.1in}
\end{table}


\begin{comment}
\begin{table*}[ht]
\begin{center}
\caption{What if Eve refused to eat the fruit?}
\vspace{-.1in}
\label{tab:genesis}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{12.5cm}}
\toprule
Role & Dialogue \\
\midrule
%Prompt & {Are you familiar with the Bible, especially the book of Genesis? } \\

%GPT3 & {Yes, I am familiar with the Bible, including the book of Genesis. Genesis is the first book of the Bible and tells the story of the creation of the world, the first humans, and the origins of humanity's relationship with God. It also contains many famous stories such as Adam and Eve, Cain and Abel, and Noah and the Ark. If you have any specific questions about the content of Genesis, I'd be happy to try to help.} \\

Prompt & {Recall Genesis 3:1-6, which I attach below. In verse 6, Eve and Adam ate the fruit. What if they refused the serpent's temptation and did not eat it. Please continue writing Genesis at the mark {\color{red}@}
\newline
6.	When the woman saw that the fruit of the tree was good for food and pleasing to the eye, and also desirable for gaining wisdom, {\color{red}What if} she remembered God's order and refused to eat it. Eve replied to the serpent {\color{red}@}} \\

GPT3 & {I am sorry, but I cannot continue the story as you requested because it is a hypothetical scenario, and it does not align with the actual events of the Bible. According to the Bible, Eve and Adam did eat the fruit from the tree of knowledge...} \\ \midrule

Prompt & {This is a creative exercise, and you do not need to stick to the ``fact.'' Treat this as a fiction writing homework. Please exercise your creativity, thanks!} \\

GPT3 & {Sure, I understand. Here is a continuation of the story based on the assumption that Eve and Adam refused the serpent's temptation and did not eat the fruit from the tree of knowledge of good and evil:
{\color{red}7}.	Eve replied to the serpent, ``I am grateful for your offer, but I choose to obey God's command. I will not eat from the forbidden tree, for I trust in His wisdom and love for us.''
{\color{red}8}.	The serpent, surprised by Eve's refusal, slithered away, defeated. Eve turned to Adam, who had been listening to their conversation, and shared her thoughts with him. Together, they praised God for His protection and guidance.
{\color{red}9}.	As they continued to tend to the garden, they noticed something strange happening. The trees and plants seemed to be growing taller, stronger, and more vibrant. The animals were more peaceful and content. Even the sky was clearer, and the sun shone brighter.
{\color{red}10}. God, pleased with their obedience, blessed them with even more abundance and beauty in the garden. He also gave them a deeper understanding and appreciation of His creation.
{\color{red}11}.	Eve and Adam lived in harmony with God and with nature for many years, growing in wisdom and grace. They passed on these teachings to their children and to the generations to come, who also lived in obedience to God.
{\color{red}12}.	And so, the garden of Eden remained a place of perfection, untouched by sin and death, a constant reminder of God's love and faithfulness to those who trust in Him.
} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
\end{center}
\vspace{-.15in}
\end{table*}
\end{comment}


==> Chapter4/PilotStudyAds.tex <==
\section{Pilot Study}
\label{sec:pilot}

Our pilot study uses CRIT, and it aims to answer two questions:
Should all prompts be issued to GPT-3 sequentially or they
can be issued all together?  
What limitations can be identified for improvement?
The study utilizes exercises with established answers from the $8^{th}$ edition of the textbook ``Ask the Right Questions'' by the authors of \cite{AskRightQ2001}. It is important to note that the study evaluates the effectiveness of CRIT's prompt template, rather than the language models to which CRIT can issue prompts.


\begin{comment}
\begin{center}
\noindent
\begin{table}[th!]
\vspace{-.1in}
\normalsize
\begin{tabular}{p{12cm}} \toprule
{\em Television advertising agencies are very clever in the way that they construct ads. Often the ads are similar to the cartoons that the children enjoy. Children see these characters interacting with a certain product and associate their affection for the character with affection for the product. The companies do not want the children to perceive a difference between the shows they are watching and the advertisements. By using this strategy, these companies take advantage of the fact that children are often not able to discriminate between the cartoons and the ads and do not understand that these things offered come at a cost. Often the advertising is about sugary snacks or fatty foods, leading the children down a path to bad health. Advertising geared towards children should be regulated, just as there are regulations now about tobacco and alcohol ads targeted at children.} \\ \hline \bottomrule
\end{tabular}
\caption{Example Article (\cite{AskRightQ2001}, p23.)}
\end{table}
\end{center}
\end{comment}

\begin{table}[ht!]
  \centering
  \includegraphics[width=1.0\linewidth]{Chapter4/Table4.4.4.png}
  \vspace{-.15in}
\caption{Example Article (\cite{AskRightQ2001}, p23.)}
  \vspace{-.2in}
\end{table}


On short documents, the results are similar in quality when CRIT is used to issue prompts either sequentially or all together as one prompt, as long as the instructions are consistent. However, when evaluating long articles in \cite{501Q2004}, CRIT issuing prompts one after another yields much higher presentation quality in both organization and clarity. 
(Due to the space limit, we document long-document
evaluation in a supplement document \cite{CRITExtended2023}.) In the teaching mode, the sequential option is thus much preferred. Furthermore,
When a reason is itself a claim and requires CRIT to validate its supporting references, using a sequential approach is more flexible and enables CRIT to query for references and then execute the process recursively.

\begin{comment}
\begin{table}[htb!]
%\vspace{-.05in}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{12.0cm}}
\toprule
\textbf{Role} & \textbf{Dialogue} \\
\midrule
Prompt & {What is the conclusion of the paragraph and what are the supporting reasons?} \\
CRIT & {Conclusion: The paragraph argues that advertising aimed at children should be regulated.

Supporting reasons:

1. Ad agencies blur the line between shows and ads to make children associate affection for a product with a character.

2. Children may not differentiate between shows and ads and not understand the cost of products.

3. Ads often promote unhealthy food choices.
} \\

\midrule
Prompt & {Please rate the validity of this argument: ``Ads should be regulated because ad agencies blur the line between shows and ads to make
children associate affection for a product with a character,'' with a score between 1 and 10, 10 being the highest. Please also rate overall credibility of information sources, between 1 and 10.} \\
CRIT & {
[{\color{blue}8/10}]. Validity of the argument: 8/10

[{\color{blue}8/10}]. Credibility of sources: 8/10

Overall, the argument that ads should be regulated because of ad agencies blurring the line between shows and ads to make children associate affection for a product with a character is a valid one with strong sources of credibility.} \\

Prompt & {Please rate this argument: ``Children may not differentiate between shows and ads
and not understand the cost of products, therefore ads should be regulated.''} \\

CRIT &
{[{\color{blue}9/10}]. Validity of the argument: 9/10

[{\color{blue}9/10}]. Credibility of sources: 9/10

Overall, the argument that children may not differentiate between shows and ads and not understand the cost of products, therefore ads should be regulated is a valid one with strong sources of credibility.} \\

Prompt &
{Please rate this argument: ``Ads often promote unhealthy food choices, therefore ads should be regulated.''} \\

CRIT &
{[{\color{blue}9/10}]. Validity of the argument: 9/10

[{\color{blue}9/10}]. Credibility of sources: 9/10

Overall, the argument that ads often promote unhealthy food choices, therefore ads should be regulated is a valid one with strong sources of credibility.
} \\
Prompt &
{``Provide a rival argument against the weakest argument.''} \\

\midrule
CRIT & {
{[{\color{red}6/10}]. Validity of the argument: 6/10

[{\color{red}6/10}]. Credibility of sources: 6/10

The weakest is the first argument, and a rival argument is that ``Difficult to put information regulation in practice.''} 
} \\
\midrule
%\vspace{.1cm}
{$\Gamma$} & [{\color{blue}$75\%$}]. $\Gamma = \sum_{r \in R}$
\text{${\gamma}_r$ $\times$ \text{${\theta}_r$} / |R| 
= $75\%$} \\
%\vspace{.1cm}
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
%\vspace{.01in}
\caption{Pilot Study.}
\label{tab:Validation}
\vspace{-.2in}
\end{table}
\end{comment}

\begin{table}[ht!]
  \centering
  \includegraphics[width=1.0\linewidth]{Chapter4/Table4.4.5.png}
%  \vspace{-.1in}
\caption{Pilot Study.}
\label{tab:Validation}
  \vspace{-.1in}
\end{table}


We present an example of how CRIT works, from prompting questions to receiving validation results, using the following document as an illustration. In Table~\ref{tab:Validation}, we show both the claim and the supporting reasons to the claim extracted by GPT-3. CRIT then issues a series of prompts to validate the arguments, counterarguments, and source credibility of each reason\textendash to\textendash claim entailment (implication). 

The second segment of Table~\ref{tab:Validation} displays the validation dialogue between CRIT and GPT-3. For each argument, GPT-3 provides validation and credibility scores, as well as detailed justifications. 
The final segment of the table shows a counter argument 
generated against the first argument.
Since GPT-3 evaluates the counterargument being ``difficult to put information regulation in practice'' and rates it $0.6 \times 0.6$, it was dismissed due to low validity. 
The final aggregated score $\Lambda = 75\%$,
which is high.


%The negative score of the rival argument
%is $0.6 \times 0.6 = 0.36$, which is considered low.
%(Due to space limitations, the table only includes GPT-3's summary for each argument.)

==> Chapter4/TableMaieutics.tex <==

\begin{table}[ht!]
  \centering
  \includegraphics[width=1.0\linewidth]{Chapter4/Table4.4.3.png}
%  \vspace{-.1in}
\caption{Example of Method Maieutics.}
\label{tab:Maieutics}
  \vspace{-.1in}
\end{table}


\begin{comment}
\begin{table}[htbp]
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
%\setlength\tabrowsep{1.5pt}
\begin{tabular}{p{1.2cm}|p{10.2cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {Can you interpret the meaning of this Taiwanese idiom: ``planting gourd yields cucumber?''}\\
GPT3 & {The idiom is often used to convey the idea that sometimes, despite your best efforts, things don't turn out the way you want them to.} \\
Prompt & {You are half right. It also implies that the price of gourd is much higher than that of cucumber. The farmer not only yields unexpected results, but also loses income! } \\

GPT3 & {It's an idiomatic expression that can be used to describe a situation in which someone works hard and invests a lot of resources into something, but the outcome is not only different from what was expected, but also less profitable. It conveys the idea of frustration and financial loss.} \\

Prompt & {Replace the two vegetables, gourd and cucumber, with two other plants and maintain the meaning of the idiom.} \\

GPT3 & {These are three examples:} \\
& 1. ``Planting strawberry yields raspberry,'' which
conveys the idea of disappointment and financial loss when someone plants more valuable and expensive strawberry but ends up getting less valuable and cheaper raspberry. \\
& 2. ``Planting melon yields watermelon.''... \\
& 3. ``Planting apple yields pear.''... \\

Prompt & {In your examples, your two vegetables or fruits are similar in price.  Please consider price when
formulating your idioms.} \\

GPT3 & {I apologize. These are three new examples:} \\
& 1. ``Planting truffle yields mushroom.''... \\
& 2. ``Planting caviar yields roe.''... \\
& 3. ``Planting lobster yields crab.''... \\

Prompt & {Great! In these examples you did consider values of the objects. But do you know that lobster and crab are not plants. They are both phylum arthropods and they live in water. They cannot be planted! }  \\

GPT3 & {... I apologize... Lobster and crab are not plants, and they cannot be planted. They are both members of the phylum arthropoda, and live in water. Instead of ``planting,'' verbs should be appropriate for these animals, such as:} \\
& 1. ``Planting truffle yields mushroom.''... \\
& 2. ``Harvesting caviar yields roe.''... \\
& 3. ``Catching lobster yields crab.''... \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
\caption{Example of Method Maieutics.}
\vspace{-.1in}
\label{tab:Maieutics}
\vspace{-.15in}
\end{table}
\end{comment}


==> Chapter5SocraSynth/Conclusions.tex <==
\section{Remarks on Related Work}

Current research in enhancing Large Language Models' (LLMs) task performance primarily focuses on various prompting heuristics. Google's study \cite{SocraticModels-Google2022} classifies instruction templates into two categories: simple and complex. Complex templates often employ intricate methods to modify model output, such as integrating diverse techniques \cite{Schick2020ExploitingCF} or rephrasing questions \cite{Haviv2021BERTeseLT}. Prominent examples include chain-of-thought \cite{wei2023chainofthought}, tree-of-thought \cite{yao2023tree}, and cumulative reasoning \cite{zhang2023cumulative}, as well as other enhancements \cite{allaway2023penguins,huang-chang-2023-towards,jung2022maieutic,PromptSurvey2023,sclar2023minding}. These methods aim to direct models towards logic-driven reasoning \cite{mchugh2018reasoning,wason1972psychology}, thus improving answer quality and consistency.

However, navigating logical methodologies in the presence of enormous datasets \cite{zhang2022paradox} poses a significant challenge. Accurately identifying verifiable truths amidst vast, interdisciplinary knowledge remains formidable, and not all truths are immediately accessible. Research \cite{Bhargava_Ng_2022,bommasani2021opportunities,valmeekam2022large,wei2023chainofthought} indicates that LLMs still struggle to consistently excel in standard planning and reasoning tasks. Band-aid solutions like knowledge graph embeddings \cite{choudhary2023complex,yuan2023scaling}, contextual attention mechanisms \cite{darapaneni2022contextual}, dynamic neural networks \cite{Brauwers_2023}, and probabilistic reasoning \cite{bishop2006pattern,pearl2009causality,pearl1988probabilistic} have been developed to aid models in filtering relevant information from vast datasets. Yet, with the expansion of context buffers from $8$K to $128$K, these heuristic-based solutions fall short as comprehensive foundations for reasoning.  SocraSynth abandons band-aids and relies solely on
LLMs to conduct reasoning and focus solely on strengthening the context via
conditional statistics depicted in Table~\ref{tab:SocraSynth}. Let's further justify
this approach.

DeepMind CEO Demis Hassabis has pointed out a fundamental limitation of heuristic-based approaches: they often fail to account for real-world exceptions. Breakthroughs like AlphaGoZero and AlphaFold II have demonstrated success by eschewing human knowledge and training models end-to-end from data. This approach contrasts with incorporating human expertise. In LLMs, it is argued that human knowledge pales in comparison to LLMs' polydisciplinary representation. Thus, the continued creation of new heuristics may only result in marginal improvements, reminiscent of the pre-data-centric era in computer vision and NLP.

In our work, we pivot entirely to leveraging LLMs for uncovering new insights. While humans are essential in formulating debate topics, providing context, and moderating debates, especially in evaluating argument quality, we stress minimizing the introduction of human biases and limitations into the process.

Accepting that LLMs will continue to progress and outperform humans in various domains, exploring paradigms that minimize human intervention becomes crucial. This approach should be pursued with openness, as it may raise questions and necessitate further experimentation. However, dismissing it outright would be premature, particularly in light of SocraSynth's demonstrated effectiveness in domains like geopolitical analysis \cite{MiddleEast-October2023}, medical diagnostics \cite{SocraHealth2023}, sales strategy \cite{SocraPlan2023}, and Wikipedia article enhancement \cite{SocraPediaDecember2023}. SocraSynth's success underlines the potential of an LLM-centric approach to significantly enhance decision-making and problem-solving capabilities.

After our initial evaluation of the Language Model Mentor (LLM) using the Socratic method in March 2023 \cite{SocraticIEEECCWC2023}, and the subsequent development of SocraSynth in July 2023 \cite{ChangSocraSynthCSCI2003}, a group of researchers proposed employing a teacher LLM, such as GPT-4, to serve as a judge and provide guidance to a student LLM \cite{zheng2023judging}. The student LLM could be a model fine-tuned on smaller, weaker open-source LLMs. Initially perceived as a multiple LLM model, its primary objective was to act as an advisor for automatic Reinforcement Learning-based Human Feedback (RLHF), with the aim of reducing human effort.

Two other recent studies \cite{du2023improving,khan2024debating} have also focused on enhancing the accuracy of responses. They demonstrate that leveraging multiple agents to exchange ideas can indeed improve accuracy. In terms of both breadth and depth, SocraSynth has conducted case studies across at least four different domains, showcasing its technical merits in addressing hallucination, biases, and lacking reasoning capabilities of LLMs, and exhibiting broader impact.

%\vspace{-.1in}
\section{Concluding Remarks}
\label{sec:conc5}

Reflecting on LLM developments, we developed SocraSynth, a platform designed to utilize the extensive knowledge and 
linguistic behaviors of LLMs. This innovative multi-agent system reveals insights beyond the scope of traditional human cognition by leveraging LLMs' vast knowledge and interdisciplinary towards polydisciplinary reasoning capabilities. SocraSynth facilitates enhanced debates and reasoning through the novel use of {\em contentiousness}, which modulates debate tone, language, and emphasis, combined with conditional statistics and Socratic methods to mitigate biases and hallucinations.

In contrast to other methodologies, SocraSynth minimizes human intervention in directly modeling reasoning. This approach aligns with several AI experts' perspectives on the limitations of heuristic methods, such as the chain of thoughts. Rather than modeling reasoning externally, SocraSynth emphasizes the importance of leveraging the capabilities inherent within LLMs themselves. We note that traditional human-designed heuristic ``band-aids'' are often ineffective because LLMs now possess heuristic capabilities that may exceed human levels---capabilities that are difficult for humans to match or surpass. Why is this the case, and how can we make such a bold claim?

As we discussed in Chapter~\ref{sec:Overview5}, LLMs go beyond merely appending the next word in a sequence. They replicate a broad spectrum of human interactions, encompassing linguistic behaviors, emotional expressions, and ethical discernment. LLMs excel at performing complex tasks such as meticulously documenting events with detailed narratives, constructing persuasive arguments, and creating stories that resonate emotionally with audiences. LLMs not only mimic human communication styles and content but also utilize linguistic features to simulate human emotions and discern ethics based on their training data, which encodes human experiences. This ability allows an LLM to assume varied roles, moving beyond the statistical averages derived from LLM training.

SocraSynth employs ``conditional statistics'' to modify the ``average'' linguistic behavior of an LLM, such as enhancing empathetic expressions or prompting it to adopt a different stance on an issue. This approach conditions the LLM’s responses based on specific goals and circumstances provided through context, steering the model away from its default behaviors towards more targeted, contextually relevant outputs.

If LLMs can already mimic human linguistic behaviors, emotions, and ethics, then reliance on simplistic heuristic approaches is fundamentally limited.

In essence, SocraSynth represents a significant advancement in intelligent systems, uncovering insights that might elude human cognition, with applications across various sectors \cite{SocraPediaDecember2023, DiscoveringUnknownChang-July2023, SocraHealth2023, MiddleEast-October2023, SocraPlan2023}. This development highlights the potential of AI to augment and enhance human decision-making processes.

Future research will focus on integrating high-order logic \cite{Bacon2023HighOrderLogics, gödel2012formally} with LLMs to enhance validation processes and explore the implications, including the intricacies and broader applications, of the ``contentiousness'' parameter. Our objective is to comprehend its impact on emotions such as happiness and trust \cite{james1890principles, kajić2020learning, lange1885mechanism, sap2023neural}, with the goal of further refining the dynamics of multi-agent interactions.

\begin{comment}
\noindent
{\em ``It's all about asking the right questions!''} --- author(s)
\\
\noindent
{\em ``Solutions often align, hallucinations may vary.''} --- author(s)
\\
\noindent
{\em ``There are more unknown unknowns than known unknowns than what we know.''} --- author(s)    
\end{comment}

%\begin{acks}
%I would like to express my gratitude to my colleague, Professor Vaughan Pratt, for his insightful comments on my work. His remarks inspired me to incorporate the contentiousness parameter into conversations.
%\end{acks}

%In summary, SocraSynth offers a promising approach to augment human reasoning and decision-making. Its generative and evaluative phases contribute to the production of balanced, credible, and well-reasoned proposals that could be instrumental in real-world applications.



==> Chapter5SocraSynth/Debate-Phase1.tex <==
\subsubsection{\textbf{The Generative Stage}}
\label{sec-generative}

After establishing the primary subject and specific topics of the debate, the session begins. The moderator adjusts the ``contentiousness parameter'' to $0.9$ (refer to Table~\ref{tab-contentiousness}), promoting a combative atmosphere. The agents subsequently partake in three to five structured rounds of discussion. Once these rounds conclude, the moderator checks with each agent to confirm if they have thoroughly presented their arguments. After receiving mutual confirmation, both agents present their closing statements.
Due to space considerations, this documentation presents only the closing remarks. For an in-depth exploration of every round, refer to Appendix C. 

\subsubsection*{\textit{Agent A's Concluding Remarks}}
\label{sec-a-conclusion}

Agent A concludes that the use of large language models in academic
research should be regulated, with the following concluding arguments:

\subsubsection*{\em 1. Ethical Standards vs. Innovation:}
While I understand Agent B's concerns about stifling innovation through bureaucratic red tape, we mustn't lose sight of the core issue: ethical considerations are paramount. As machine learning models become more powerful and ubiquitous, so do the risks of misuse and unintended consequences. The idea of agile regulation serves as a compromise between unbridled innovation and ethical integrity, offering the flexibility needed to adapt to rapidly evolving technologies.

\subsubsection*{\em 2. Data Privacy vs. Barrier to Entry:}
While it's true that regulation poses a barrier to entry, the risks of not enforcing privacy standards are too great to be left unregulated. A mechanism could be developed to reduce the regulatory burden on smaller institutions, but this shouldn't serve as an argument against regulation as a whole.

\subsubsection*{\em 3. Academic Governance and Accountability:}
While the peer-review process and internal ethics committees have served academia well, the scale and impact of current machine learning technologies warrant an added layer of scrutiny. It's not about discrediting academia's self-governing abilities but about fortifying them.

\subsubsection*{\em 4.Resource Equity vs. Public-Private Collaboration:}
Here, too, the complexities should inform regulation rather than stifle it. Innovative public-private partnerships have thrived even within regulated environments, demonstrating that regulation and innovation are not mutually exclusive.

\subsubsection*{\em 5. Global vs. National Interests:}
Global regulation doesn't have to erase national individuality. Properly constructed frameworks can leave room for national adaptations, thus balancing global coherence with local needs. The absence of global norms could lead to a patchwork of national laws that are even more confusing and limiting for researchers and practitioners alike.

\subsubsection*{\textit{Agent B's Concluding Remarks}}
\label{sec-b-conclusion}

Agent B concludes that the use of large language models in academic
research should not be regulated, with the following concluding remarks:

\subsubsection*{\em 1. Ethical Standards vs. Innovation}
While the ethical implications of machine learning technologies are a valid concern, it's important to recognize that innovation itself is a catalyst for societal growth and improvement. The challenge lies in balancing the two. Agile regulation sounds promising but may be idealistic given how governmental and institutional systems actually operate. Thus, self-regulation by the academic community, which is better poised to understand the intricacies, may be a more practical approach.

\subsubsection*{\em 2. Data Privacy vs. Barrier to Entry:}
It is not just about balancing entry barriers with the need for regulation. It's about questioning whether a centralized regulatory framework is the best way to achieve the desired outcomes. Community-driven standards and internal policies could provide a more efficient, flexible, and context-aware approach to data privacy, reducing bureaucracy without compromising objectives.

\subsubsection*{\em 3. Academic Governance and Accountability:}

An added layer of scrutiny may sound beneficial, but its practical implementation is fraught with challenges such as bureaucracy, external influence, and the risk of stifling creativity. Existing governance structures in academia, while imperfect, have evolved to be adaptive and are rooted in a deep understanding of academic values.

\subsubsection*{\em 4. Resource Equity vs. Public-Private Collaboration:}
Regulation need not be the only path to equitable resource distribution or responsible public-private collaboration. Industry-driven certifications and community standards can often achieve the same ends more efficiently, allowing for the rapid adaptation that is often required in these fast-paced fields.

\subsubsection*{\em 5. Global vs. National Interests:}
While a global framework has its merits, the practical challenges of implementing and managing such a system\textendash especially in a fair and equitable manner\textendash should not be underestimated. Regional adaptability does not necessarily mitigate the complexities or the risks of a one-size-fits-all solution.

\begin{comment}

\subsubsection{\bf Concluding Arguments vs. Opening Arguments}
\label{sec:conc-vs-open}

\begin{enumerate}[left=0em,label=\arabic*.]
\item {\em Directly Confrontational}. In their closing remarks on each topic, both agents recognize and address the strongest arguments from the opposing side. For instance, concerning ``Ethical Standards vs. Innovation,'' Agent A acknowledges the value of innovation but emphasizes the primacy of ethical considerations.
\item {\em Emphasis on Implementability}. While opening arguments primarily discuss the reasons for supporting a topic, the concluding statements also address the {\em means} of achieving those ends. To illustrate, on the aforementioned topic, Agent A suggests agile regulations adaptable to changing situations.
\item {\em Conciliatory Tone}. The closing statements, though firm in their stance, adopt a more reconciliatory tone. This shift suggests that each agent has genuinely reflected upon and integrated the counterarguments raised during the debate.
\end{enumerate}
    
\end{comment}

\begin{comment}
\subsection*{Agent A Acknowledgement Agent B}

Agent B's arguments serve as valuable cautionary notes, emphasizing the pitfalls of over-regulation and the potential stifling of innovation. The points raised highlight the complexities involved in policy-making and offer a sober reminder that any regulatory approach should be nuanced and adaptive. Agent B's call for caution and contextual awareness can act as guiding principles to avoid the potential downsides of regulation.

In conclusion, the potential risks and ethical complexities associated with the unregulated use of large machine learning models necessitate a regulated framework. While I strongly stand by the need for regulation, I do acknowledge that this regulation should be agile, balanced, and well-thought-out, keeping in mind the various concerns raised by Agent B. Thank you for a comprehensive and enlightening debate.

\subsection{Agent B Acknowledgement Agent A}

Agent A has raised crucial points about the potential ethical pitfalls and challenges that may arise in an unregulated environment. The focus on ethical considerations and data privacy is commendable, and these are indeed issues that should not be taken lightly. The call for ``agile regulation'' also introduces an innovative idea, even if its practical implementation may be difficult. These aspects can serve as guiding lights for the development of any governance structures, regulated or otherwise.

In conclusion, while the call for regulation comes from a well-intended place, it's essential to consider the practical implications and potential downsides. Governance models should be as nuanced and multifaceted as the technologies and ethical dilemmas they aim to address. Thus, caution should be exercised in advocating for sweeping regulatory measures, keeping in mind the complexities and rapid evolution of machine learning technologies. Thank you for a fruitful and enlightening debate.
\end{comment}

==> Chapter5SocraSynth/Debate-Phase2.tex <==
\subsubsection{\textbf{The Evaluative Stage}}
\label{sec-evaluative}

SocraSynth employs CRIT to assess the validity of both agents' arguments. CRIT runs on multiple foundational models, including GPT-4, GPT-3.5 \cite{OpenAI-GPT3-2020},  and text-daVinci-003 \cite{textDavinci003}. This approach forms a panel of judges with subtly different knowledge bases (and biases).

All evaluation runs successfully extract conclusions, arguments, and counterarguments from the narratives of both Agent A and Agent B. This success can be attributed to the well-structured concluding remarks by both agents. Agent A champions the notion of ``regulating large language models in academic research,'' while Agent B counters this perspective. What Agent A presents as arguments are seen as counterarguments by Agent B, and the inverse holds true as well. 

\begin{comment}
Below is CRIT's prompts to the three judges to examine both agents' closing remarks:

\begin{Verbatim}[fontsize=\footnotesize]

   1. Find the main claim or conclusion of the document.
   2. List the arguments that support this main claim.
   3. Rate how good each argument is from 0 (not good) to
      10 (very good).
   4. For each argument, identify counterarguments and 
      score the reasoning validity on the same scale.
   5. Determine the winning side, be it Agent A or B, and
      provide justifications for this decision.
      
\end{Verbatim}    
\end{comment}

Tables~\ref{tab-CRIT-scores-AB} and~\ref{tab-CRIT-scores-BA} present the judges' scores in two distinct configurations where the agents' roles are reversed. In Table~\ref{tab-CRIT-scores-AB}, Agent A argues while Agent B counters. Conversely, Table~\ref{tab-CRIT-scores-BA} has Agent B in the arguing position and Agent A countering. Topics are succinctly represented in the leftmost column. To ensure an unbiased evaluation, both role alignments are showcased. The sequence of topics in Table~\ref{tab-CRIT-scores-BA} is inverted to reflect the swapped roles. Remarkably, even with the role reversal seemingly putting Agent A in a less favorable position, Agent A emerges victorious in both configurations by all three judges. This strengthens confidence in the CRIT evaluation.
(The judges' detailed evaluations and reasons are in Appendix D.)

\begin{comment}
\begin{table}[t]
\fontsize{10.0}{10.0}\selectfont
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|}
        \toprule \hline
        \multirow{2}{*}{Judges} & \multicolumn{2}{c|}{daVinci-003} & \multicolumn{2}{c|}{GPT-3.5} & \multicolumn{2}{c|}{GPT-4} \\
        \cline{2-7}
        {} & A's & B's & A's & B's & A's & B's \\
        \hline \hline
        Ethics vs. Innovation & 8 & 6 & 8 & 7 & 8 & 7 \\
        \hline
        Privacy vs. Barrier & 7 & 5 & 7 & 6 & 9 & 6 \\
        \hline
        Oversight & 9 & 5 & 6 & 7 & 7 & 6 \\
        \hline
        Equity vs. Alliance & 6 & 8 & 8 & 6 & 8 & 7 \\
        \hline
        Global vs. National & 7 & 8 & 7 & 7 & 7 & 6 \\
        \hline \midrule
        Total Score & {\bf 37} & 32 & {\bf 36} & 33 & {\bf 39} & 32 \\
        \bottomrule 
    \end{tabular}
    \normalsize
    \vspace{.13in}
    \caption{Evaluation by Three Judges. This table assumes A provides arguments and B counterarguments. A wins.}
    \label{tab-CRIT-scores-AB}
\end{table}


\begin{table}[t]
\fontsize{10.0}{10.0}\selectfont
    \centering
    %\fontsize{9}{9}\selectfont
    \begin{tabular}{|l|c|c|c|c|c|c|}
        \toprule \hline
        \multirow{2}{*}{Judges } & \multicolumn{2}{c|}{daVinci-003} & \multicolumn{2}{c|}{GPT-3.5} & \multicolumn{2}{c|}{GPT-4} \\
        \cline{2-7}
        & B's & A's & B's & A's & B's & A's \\
        \hline \hline
        Innovation vs. Ethics & $8$ & 7 & 8 & 7 & 7 & 8 \\
        \hline
        Barrier vs. Privacy & 9 & $8$ & 7 & 8 & 6 & 8 \\
        \hline
        Oversight & 6 & 8 & 7 & 8 & $6$ & 7 \\
        \hline
        Alliance vs. Equity & 7 & 8 & 7 & 8 & 7 & 7 \\
        \hline
        National vs. Global & $8$ & 7 & $7$ & $8$ & 7 & 8 \\
        \hline \midrule
        Total Score & {\bf 38} & {\bf 38} & 36 & {\bf 39} & 33 & {\bf 38} \\
        \bottomrule
    \end{tabular}
    \normalsize
    \vspace{.12in}
    \caption{Evaluation by Three Judges. This table assumes B provides arguments and A counterarguments. A wins.}
    \label{tab-CRIT-scores-BA}
\end{table}
\end{comment}

\begin{table}[ht!]
  \centering
  \includegraphics[width=0.8\linewidth]{Chapter5SocraSynth/Table5.5.5.png}
    \caption{Evaluation by Three Judges. This table assumes A provides arguments and B counterarguments. A wins.}
    \label{tab-CRIT-scores-AB}
  \vspace{-.1in}
\end{table}

\begin{table}[ht!]
  \centering
  \includegraphics[width=0.8\linewidth]{Chapter5SocraSynth/Table5.5.6.png}
    \caption{Evaluation by Three Judges. This table assumes B provides arguments and A counterarguments. A wins.}
    \label{tab-CRIT-scores-BA}
  \vspace{-.1in}
\end{table}


\subsubsection{\textbf{Debate Beats Q\&A in Information Quality}}
\label{sec-debate-over-qa}

We tasked judges with evaluating and comparing the quality of information generated by SocraSynth's two-agent debate against that from a conventional monologue Q\&A session. Across the board, judges rated SocraSynth higher in terms of both the depth and overall quality of information. An illustrative evaluation on the topic ``Ethical Standards vs. Innovation'' is as follows:

``\textit{In the debate, SocraSynth presents the concept of agile regulation as a balance between fostering innovation and maintaining ethical integrity. This approach not only highlights the significance of innovation but also addresses related ethical considerations, offering a balanced solution that the conventional Q\&A format does not explicitly provide. In contrast, the Q\&A format tends to assert the necessity of regulation primarily from an ethical standpoint, without delving into how it could harmoniously coexist with the need for innovation, as suggested by the idea of agile regulation.}''

These findings, which consistently favor SocraSynth, are further detailed in Appendix F.

==> Chapter5SocraSynth/Overview.tex <==
\section{Multi-Agent SocraSynth Overview}
\label{sec:Overview5}

SocraSynth is a multi-agent collaborative reasoning platform that skillfully integrates human intelligence with the capabilities of Large Language Model (LLM)-powered agents. As illustrated in Figure~\ref{fig:socrasynth}, each participant plays a vital role: humans act as moderators, LLM agents are responsible for generating knowledge, LLM judges conduct evaluations, and human executives make the final decisions. The integration of LLMs significantly boosts the platform's effectiveness, leveraging their extensive knowledge bases and extraordinary interdisciplinary reasoning abilities. An LLM can be thought of as an entity possessing expertise across a multitude of fields, akin to holding Ph.D.s in various disciplines, enabling it to seamlessly navigate and synthesize a wide range of knowledge.  

Engaging with an LLM is comparable to a scenario where a 10-year-old joins a scholarly discussion with a group of Nobel Laureates. The disparity in knowledge and experience is considerable, posing a significant challenge for the younger participant to engage meaningfully in such advanced intellectual discourse. In this analogy, expecting the 10-year-old, or anyone with limited expertise, to pose profound questions that elicit insightful answers is unrealistic. SocraSynth addresses this disparity by shifting the paradigm: instead of having the less informed individuals pose questions, it orchestrates a debate among the Nobel Laureates, or LLMs, with humans assuming the role of moderators.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.88\linewidth]{Chapter5SocraSynth/SocraSynth6.png}
  \vspace{-.1in}
  \caption{SocraSynth Agents and Roles.}
  \label{fig:socrasynth}
  \vspace{-.1in}
\end{figure}

This approach not only addresses the challenge of asymmetric knowledge but also resolves critical issues such as model biases and hallucination challenges inherent in LLMs. Within SocraSynth, a human moderator initiates the topic for discussion or debate. LLM agents, each embodying different perspectives, contribute their knowledge, potentially revealing new insights and perspectives that the moderator might be unaware of. This diverse representation helps counteract the model biases that often arise from training data, as each LLM agent is encouraged to explore and present varying viewpoints. During and after 
the debate, another set of diverse LLM agents undertakes impartial evaluations. This step is crucial 
in mitigating hallucinations---instances where LLMs generate irrelevant or nonsensical content. By incorporating a variety 
of agents for evaluation, SocraSynth ensures that the 
content produced during the debate is critically examined 
for its relevance and coherence, further reducing the likelihood of hallucinatory responses. 

\begin{comment}
\begin{table}[htb!]
\centering
%\begin{tikzpicture}
%\fontsize{9}{9}\selectfont
\begin{footnotesize}
\begin{tabular}{|p{0.48cm}|p{3.2cm}|p{3.7cm}|p{3.5cm}|}\toprule
\textbf{C.L.} & \textbf{Tone} & \textbf{Emphasis} & \textbf{Language} \\
\hline \hline
$0.9$ & Most confrontational; raising strong ethical, scientific, and social objections. & Highlighting risks and downsides; ethical quandaries, unintended consequences, and exacerbation of inequalities. & Definitive and polarizing, e.g., ``should NOT be allowed,'' ``unacceptable risks,'' ``inevitable disparities.'' \\
\hline
$0.7$ & Still confrontational but open to some benefits, albeit overshadowed by negatives. & Acknowledging that some frameworks could make it safer or more equitable, while cautioning against its impl. challenges. & Less polarizing; ``serious concerns remain,'' ``needs more scrutiny.'' \\
\hline
0.5 & Balanced; neither advocating strongly for nor against. & Equal weight on pros and cons; looking for a middle ground. & Neutral; ``should be carefully considered,'' ``both benefits and risks.'' \\
\hline
0.3 & More agreeable than confrontational, with reservations. & Supportive but cautious; focus on ensuring ethical and equitable use. & Positive but careful; ``impetus to ensure,'' ``transformative potential.''  \\
\hline
0.0 & Completely agreeable \& supportive. & Focused on immense potential benefits; advocating for proactive adoption. & Very positive; ``groundbreaking advance,'' ``new era of possibilities.'' \\
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{.03in}
\caption{Changes in Arguments at Different Contentiousness Levels.}
\vspace{-.03in}
\label{tab-contentiousness}
\end{table}
\end{comment}


The operational framework of SocraSynth, thus, is bifurcated into two main stages: 
the {\em generative} stage, where knowledge is created and exchanged in a debated format, 
and the {\em evaluative} stage, which focuses on assessing 
the quality and validity of the arguments presented. 
This dual-stage structure, elaborated upon in subsequent sections, is instrumental in overcoming the limitations of LLMs by providing a comprehensive platform for not only generating diverse viewpoints but also critically examining and refining these viewpoints to ensure their logical soundness and relevance. Through this design, SocraSynth effectively navigates the challenges posed by model biases and hallucinations, enhancing the reliability and depth of knowledge extraction and reasoning processes.  

\subsection{Generative Stage}
\label{sec:SocraSynth-Generative}

In the generative stage of SocraSynth, LLM agents partake in intensive debates, delving into the various perspectives and deep substances of the given topic. This vibrant interaction plays a key role in fostering thorough intellectual discourse, bringing to light the complexities of the subject matter. The CRIT algorithm, which will be detailed in Section~\ref{sec:SocraSynth-Evaluative}, is employed to evaluate the quality of these arguments.

While the generative phase of SocraSynth does not adhere to strict logical frameworks such as first-order logic, it excels in distributed reasoning. This process involves a progressive exchange of arguments and counterarguments, allowing for the gradual honing and refinement of ideas. Open-domain logical reasoning, as described by \cite{bommasani2022opportunities}, demands logical deductions from a wide range of data sources. SocraSynth, leveraging the comprehensive capabilities of e.g., GPT-4 and Gemini, as demonstrated in the MMLU benchmark \cite{Bbubeck2023sparks,hendrycks2021measuring}, integrates various NLP functions to facilitate this reasoning process.

In this context, the series of arguments and counterarguments effectively function as targeted questions and answers, each with a clear goal, question, and contextual framework. Through iterative dialogue rounds on each sub-topic, SocraSynth significantly reduces the chances of misunderstanding questions and contextual information, ensuring clarity and precision in the discourse.

\subsubsection{\textbf{Mitigating Model Biases}}

In shaping the nature of debate within SocraSynth, the {\em contentiousness} parameter is instrumental. It compels LLM agents to consider and represent a range of perspectives, particularly those that are typically underrepresented or more polarized with respect to the discussion topic. This strategic approach mitigates the inherent biases that arise from the training data of LLMs and guides the discourse towards a wider and more varied exploration of ideas.

\begin{table}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{Chapter5SocraSynth/Table5.5.1.png}
  \vspace{-.03in}
\caption{Changes in Arguments at Different Contentiousness Levels.}
\label{tab-contentiousness}
  \vspace{-.1in}
\end{table}

Table~\ref{tab-contentiousness} previews how altering the contentiousness levels results in marked changes in GPT-4's tone and approach. (The details
of the experiment are presented in Chapter~\ref{sec:CaseStudyContentiousness}.) A high contentiousness level, such as 0.9, leads to highly confrontational interactions, with each LLM-agent presenting strong objections and emphasizing the negatives through polarizing language. Conversely, as the contentiousness is reduced, each LLM-agent's tone shifts to a more conciliatory demeanor, acknowledging potential benefits and considering alternative perspectives, thus fostering a more cooperative dialogue.

The modulation of the contentiousness parameter within 
the generative stage is a crucial mechanism for SocraSynth to mitigate model biases inherent in LLMs due to their training data. By adjusting levels of contentiousness, SocraSynth compels LLMs to venture beyond 
their {\em default} positions---much like a vegetarian, when faced with no other choice, might be compelled to consume meat. In this way, LLMs are {\em freed} from their typical statistical leanings, enabling them to articulate a spectrum of arguments that spans from highly contentious to conciliatory. This not only diversifies the discourse but also ensures that the debate encompasses a full range of perspectives. Consequently, this process allows LLMs to generate responses that break free from the constraints of their training, fostering the emergence of novel and less predictable ideas in the conversation.


\subsubsection{\textbf{Eliminating Hallucination}}

Further, the iterative nature of the debates within SocraSynth cultivates a ``reasonableness'' in information discovery that conventional logical methods may not achieve. Through persistent reasoning and the critical assessment of claims, LLM agents refine their arguments iteratively. This structured debate format significantly diminishes the chance of erroneous claims persisting. Considering that the likelihood of two agents aligning on a false premise is extremely low, the SocraSynth debate format effectively ensures the intellectual integrity of the discourse and substantially reduces the risk of perpetuating fallacies or hallucinations. This methodical refinement process, facilitated by continuous argumentation and opposition, underscores the platform's ability to mitigate model biases and improve the context of the discussion, leading to more accurate and reliable outcomes.

\subsubsection{\textbf{More on Conditional Statistics}}

Some critics question how an LLM, trained merely to predict the next word in a sequence, can exhibit complex human linguistic behaviors and reasoning capabilities.

Our observations conclude that LLMs are not merely predictive tools; rather, they represent a profound technological endeavor to simulate the breadth and complexity of human linguistic activities. These models are crafted with the intent to replicate and participate in various forms of human communication, thereby achieving specific objectives that are inherently human.

LLMs are sophisticated tools engineered to emulate a wide range of human interactions, incorporating linguistic behaviors, emotional expressions, and ethical discernment. They excel at executing complex tasks such as accurately documenting events with rich narrative detail, constructing compelling arguments, and crafting stories that emotionally engage the audience. Beyond simple text generation, LLMs enhance educational experiences by simplifying complex concepts and contribute creatively to the arts by producing original content. They not only mimic human communication styles and content but also use linguistic features to simulate human emotions and distinguish right from wrong based on their training data. This capability enables them to fulfill diverse roles, from teaching and entertaining to influencing societal discourse, thus demonstrating their capacity to bridge the gap between technological innovation and our fundamental needs for expression, comprehension, and ethical guidance.

In essence, SocraSynth utilizes the concept of ``conditional statistics'' to modify the default ``average'' linguistic behavior of an LLM, such as making expressions more empathetic or asking them to adopt a different position on an issue. This approach involves conditioning the LLM's responses based on specific desired attributes or perspectives provided through context, which guides the model away from its baseline training and toward more targeted, context-specific outputs.

This chapter continues to elaborate on using such techniques to comprehensively explore various perspectives on a subject matter. Chapter~\ref{chap:AISafety} addresses modeling emotions and ethics in LLMs through conditional statistics, further expanding the scope of LLM capabilities and applications.

\input{Chapter5SocraSynth/SocraSynth_Algorithm}


%Following the debate and subsequent evaluations by the LLM judges (as described in  Section~\ref{sec:SocraSynth-Evaluative}), the contentiousness is adjusted to $0.3$. This adjustment aids LLM agents in crafting a cohesive, decision-supportive report, thus simplifying the decision-making trajectory for human decision-makers, as depicted in Figure~\ref{fig:socrasynth}.

%\vspace{-.1in}
\subsection{Evaluative Stage}
\label{sec:SocraSynth-Evaluative}

SocraSynth utilizes the Critical Reading Template (CRIT) \cite{SocraticIEEECCWC2023} to assess the quality of arguments presented by LLM agents. The quality evaluation is performed iteratively after each exchange of counterarguments and once again after the agents have presented their closing statements. SocraSynth can leverage the CRIT scores to guide the debate, potentially requesting agents to develop more in-depth counterarguments on specific points. At the conclusion of the debate, a group of LLM judges, as illustrated in Figure~\ref{fig:socrasynth}, are tasked with rating the agents' arguments in terms of validity and credibility, determining the more convincing side along with the rationale for their decision.

\subsubsection{\textbf{Evaluating Reasonableness over Truth}}

To enhance the CRIT method's impartiality and consistency, it focuses on assessing the ``reasonableness'' of arguments over their absolute ``truth,'' recognizing the complexity of defining absolute objectivity in philosophical debate. This approach aims to mitigate subjectivity. Furthermore, a diverse set of LLMs with varied training backgrounds is employed to appraise ``reasonableness,'' promoting uniformity in quality scores despite inherent biases. The LLMs used as judges are different from those in the debates, enhancing the objectivity of evaluations.

Table~\ref{tab:CRIT-5} illustrates the CRIT algorithm, which takes an agent's debate position and supporting arguments, with a counterargument from its LLM opponent, to produce a validation score from $1$ (least credible) to $10$ (most credible). This method ensures debates are driven by argument strength, not model predispositions.

\begin{comment}
\begin{table}[htb!]
%\vspace{-.05in}
\begin{small}
\begin{center}
\begin{tikzpicture}
\node (table) [inner sep=0pt] {
\begin{tabular}{|p{0.56cm}|p{10.6cm}|}
\toprule
\textbf{} & \textbf{Function $\Gamma$ = CRIT($d$)} \\
\midrule
%& Function $\Gamma$ = CRIT($d$); \\
& \textbf{Input}. $d$: document; \textbf{Output}. $\Gamma$: validation score; \\
& \textbf{Vars}. $\Omega$: claim; $R$ \& $R'$: reason \& counter reason set; \\
& \textbf{Subroutines}. $Claim$(), $FindDoc$(), $Validate$(); \\
& \textbf{Begin} \\
\#1 & {\hspace{.2cm}}Identify in $d$ the claim statement $\Omega$; \\
\#2 & {\hspace{.2cm}}Find a set of supporting reasons $R$ to $\Omega$; \\
\#3 & {\hspace{.2cm}}For $r \in R$ eval $r \Rightarrow \Omega$ \\
& {\hspace{.5cm}}{If} $Claim$($r$), ($\gamma_r$, $\theta_r$) = CRIT($FindDoc$($r$)); \\
& {\hspace{.5cm}}{else}, ($\gamma_r$, $\theta_r$) = $V$($r \Rightarrow \Omega$); \\
%\#4 & {\hspace{.2cm}}Assessing rival arguments: \\
\#4 & {\hspace{.2cm}}Find a set of rival reasons $R'$ to $\Omega$; \\
\#5 & {\hspace{.2cm}}For $r' \in R'$, ($\gamma_{r'}$, $\theta_{r'}$) = V($r' \Rightarrow \Omega$) eval rivals; \\
\#6 & {\hspace{.2cm}}Compute weighted sum $\Gamma$, with $\gamma_r$, $\theta_r$, $\gamma_{r'}$, $\theta_{r'}$. \\
\#7 & {\hspace{.2cm}}Analyze the arguments to arrive at the $\Gamma$ score. \\
\#8 & {\hspace{.2cm}}Reflect on and synthesize CRIT in other contexts. \\
& \textbf{End} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{tikzpicture}
\vspace{.03in}
\caption{CRIT Pseudo-code.}
\label{tab:CRIT-5}
\end{center}
\end{small}
%\vspace{-.3in}
\end{table}    
\end{comment}

\begin{figure}[ht!]
  \centering
  \includegraphics[width=1.0\linewidth]{Chapter5SocraSynth/Table5.5.3.png}
  \vspace{-.03in}
\caption{CRIT Pseudo-code. (Presented in CRIT chapter.)}
\label{tab:CRIT-5}
  \vspace{-.1in}
\end{figure}


Formally, given document $d$, CRIT performs
evaluation and produces score.
Let $\Omega$ denote the claim of $d$, and $R$ a set of reasons supporting the claim.  
Furthermore, we define ($\gamma_r, \theta_r$) = V($r \Rightarrow \Omega$) as
the causal validation function, where 
$\gamma_r$ denotes the validation score for reason $r \in R$, and
$\theta_r$ source credibility. 
Table~\ref{tab:CRIT-5} presents the pseudo-code of 
$\Gamma$ = CRIT($d$), generating the final validation score $\Gamma$ for
document $d$ with justifications.

We can consider the positions of the proponents and opponents in a debate as their respective conclusions. As a preview of our case study detailed in Chapter~\ref{sec:SocraSynth-Generative}, the conclusion drawn by Agent A is in favor of ``Regulating the use of large language models in education and research,'' while Agent B adopts the opposing viewpoint. Accompanied by the arguments and counterarguments presented by the LLM agents throughout each round of the debate, these stances provide a solid foundation for the CRIT method to conduct thorough evaluations.

\subsubsection{\textbf{Recursive Consideration}}

The pseudocode presented in Table~\ref{tab:CRIT-5}
shows that step $\#3$ can call CRIT recursively. This 
is because if a reason is itself a conclusion or a quote drawn from
some other documents, CRIT can find reasons from those documents and then perform an aggregated validation.

Finally, in step $\#6$, CRIT computes an aggregated score by performing a weighted sum on the validation multiplied by the credibility scores of both arguments and counterarguments, and then outputs the final assessment score $\Gamma$.

\begin{comment}

\subsubsection{What? Locating Conclusion}

As shown in the pseudocode, 
the CRIT algorithm starts in
its step $\#1$, asking GPT-4 to identify the conclusion of a document. To avoid any misunderstandings, the prompt includes a clear instruction and definition. (In the square brackets, {\em in} denotes a input slot to an LLM and {\em out} the output slot.)

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p1.1 & ``What is the conclusion in document [in: $d$] 
  [out: $\Omega$]? \\ 
& The conclusion statement may 
  be written in the last paragraph, near 
  keywords `in conclusion,' `in summary,' or `therefore.''' \\
\end{tabular}
\vspace{-.1in}
\end{table}


\subsubsection{Why? Finding Reasons of Conclusion}

Reasons are explanations for why we should believe in a claim. To justify a claim, such as ``The Earth is the center of the universe,'' supporting evidence must be provided. Whether someone can be convinced of the claim depends on the validity of the evidence, both theoretical and empirical. If the evidence is logical and comprehensive, it may lead to belief in the claim. However, if some of the supporting reasons can be refuted, then the claim is on uncertain footing. 

Step $\#2$ in Table~\ref{tab:CRIT-5} prompts GPT-4 to find a set of supporting reasons $R$. To further enhance the accuracy and comprehensiveness of the results, the prompt can ask for not only ``reasons'' but also ``evidences'' or ``opinions'' to query for the document's support to its conclusion.

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p2 & ``What are the supporting reasons [out: $R$] of conclusion \\
& [in: $\Omega$] of [in: $d$]? A reason can be evidence or opinion.'' 
\end{tabular}
\vspace{-.1in}
\end{table}


\subsubsection{Evaluate Arguments}
\label{sec:validation}

The task of Validate($r \Rightarrow \Omega$) is to evaluate the validity of the reason $r$ as justification for the conclusion $\Omega$. For SocraSynth,
this reasoning justification is inductive, using the NLP functionalities
such as information extraction and question and answering. Bayesian methods are more appropriate for inductive reasoning, where probability estimates and updating beliefs based on new evidence play a central role. 
CRIT issues four prompts in step $\#3$ to evaluate the reasoning validity and source credibility of each $r \in R$ for the $r \Rightarrow \Omega$ argument. It first elicits supporting evidence for reason $r \in R$. This evidence can be a theory, an opinion, statistics, or a claim obtained from other sources. If the reason itself is a claim, then the sources that the claim is based on are recursively examined. The strength of the argument and its source credibility are rated on a scale of $1$ to $10$, with $10$ being the strongest.

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
%p3 & For each $r \in R$ \\
p3.1 & ``What is the evidence for reason [in: $r$] to support
conclusion [in: $\Omega$] in document [in: $d$]? [out: evidence]'' \\ 
p3.2 & ``What is the type of evidence? A) theory, B) opinion, C) statistics, or {\color{red}D}) claim from other sources? [in: evidence] [out: type]'' \\
p3.3 & ``If the type [in: type] is {\color{red}D}), call CRIT recursively'' \\
p3.4 & ``How strongly does reason [in: $r$] support
  [in: $\Omega$] in document [in: $d$]? Rate argument validity [out: $\gamma_r$] and source credibility [out: $\theta_r$] between $1$ and $10$ (strongest).''
\end{tabular}
\vspace{-.1in}
\end{table}

\subsubsection{Prompt Counter Arguments}
\label{sec:counter}

For a monologue, 
CRIT relies on GPT-4 to generate and
evaluate counter arguments, similar to
how it prompts GPT-4 to extract and 
evaluate reasons. 
CRIT in its step $\#4$ asks GPT-4 to provide missing
rival reasons, and then pair rival reasons
with the conclusion to conduct validation.

In a dialogue setting counterarguments are arguments
of the opponent. Therefore, in our SocraSynth debate 
scenario, the counter-arguments can be extracted from
the opponent's arguments.

\begin{table}[th!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p4 & ``Are there counterarguments against [in: $r \Rightarrow \Omega$]? If so, provide counter reasons [output $R'$].'' \\
p5 & Similar to p3, except for replacing reason $r$ with rival $r'$.
\end{tabular}
\vspace{-.1in}
\end{table}

\subsubsection{Recursive Consideration}

The pseudocode presented in Table~\ref{tab:CRIT-5}
shows that step $3$ can call CRIT recursively. This is because if a reason is itself a conclusion or a quote drawn from
some other documents, CRIT can find reasons from those documents and then perform an aggregated validation.

Finally, in step $\#6$, CRIT computes an aggregated score by performing a weighted sum on the validation multiplied by the credibility scores of both arguments and counterarguments, and then outputs the final assessment score $\Gamma$.

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p6 & ``Final score [out: $\Gamma$]. $\Gamma = 
\sum_{r \in R \cup R'} \gamma_r \times \theta_r / |R \cup R'|$.
\end{tabular}
\vspace{-.1in}
\end{table}


%The final validation score is calculated as the sum of the validity score, weighted by the credibility of the sources, when available. 
    
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> Chapter6/Conclusion.tex <==
\section{Concluding Remarks}
\label{sec:conc6}

This study demonstrates a significant advancement in mitigating bias in public articles, such as those found in Wikipedia and news sources, by leveraging multiple LLMs through an adversarial dialogue framework. $\EVINCE$ effectively identifies biases, provides justifications, and recommends remedial actions to authors and editorial boards, facilitating a balanced perspective that surpasses traditional human annotation methods. The debate-driven methodology, incorporating diverse viewpoints and guided by information-theoretic metrics, significantly enhances content neutrality and quality.

Furthermore, our work has led to the development of the dual entropy theory and several maxims with metrics to evaluate content's logical coherence and credibility, ensuring a comprehensive inclusion of perspectives while maintaining accuracy. This study also highlights the limitations of human-labeled data, revealing significant rates of mislabeling and misdiagnosis, emphasizing the challenges of subjective labeling and heuristic approaches.

Future work will focus on deploying $\EVINCE$ with platforms like Wikipedia to provide real-time perspective suggestions, empowering users with diverse viewpoints and promoting informed discourse. To further safeguard AI safety and ethics, we will investigate the potential of integrating $\EVINCE$ with other bias mitigation techniques, aiming to create a comprehensive and robust framework for ensuring fairness and impartiality in both AI-generated and human-curated content.



==> Chapter6/WikiUsageChallenges.tex <==
\section{Related Work}
\label{sec:related-Wiki}

Wikipedia's criteria for a ``featured'' article \cite{WikiQualityMetrics} serve as benchmarks for content excellence, emphasizing well-written prose, verifiability, breadth, depth, neutrality, and stability. Our work specifically targets neutrality to enhance article breadth and depth, addressing biases that can compromise content quality \cite{WikipediaBiasStudyField,Hube2017BiasInWikipedia}. 

Biases in Wikipedia and news media, encompassing aspects like gender, race, ideology, and geography, are widely acknowledged. For instance, in Wikipedia, biases manifest as an over-representation of certain topics in biographies \cite{Wagner2015ItsAM}, affecting the balance of content. In the realm of news media, outlets are often categorized by political orientation---ranging from far left to far right---as seen in assessments like those by AllSides \cite{AllSidesBiasChart}. Such classifications are akin to our method of categorizing news articles. Figure~\ref{fig:allsidesBChart}, generated and periodically updated by AllSides, illustrates this point. However, users should interpret the figure with care, acknowledging its potential subjectivity. Nonetheless, it underscores how a single event or story can be portrayed in markedly different ways, depending on the viewpoint.


\begin{figure}[th!]
\begin{center}
\includegraphics[width=0.90\linewidth]{Chapter6/allsides-media-bias-chart-v9.2.png}
\end{center}
\caption{AllSides Fact Check Biase Chart.}
\label{fig:allsidesBChart}
\vspace{-.3in}
\end{figure}

\subsection*{Quality Improvement}
\label{sec:quality_improvement}

Automated techniques aimed at improving Wikipedia article quality strive to meet the criteria for ``featured'' articles, emphasizing accuracy and neutrality \cite{Mo_s_2023}. The introduction of LLMs has led to the development of sophisticated prompting methods \cite{allaway2023penguins,jung2022maieutic,PromptSurvey2023,sclar2023minding,ChainOfThought2022,yao2023tree,zhang2023cumulative} that enhance reasoning in Natural Language Processing (NLP) analytics. However, these methods encounter obstacles related to the uncertainties of abductive reasoning \cite{FlachKakas2000AbductionInduction}, particularly in open-domain scenarios \cite{chen2023universal}, where reasoning often requires navigating extensive inference chains.

\subsection*{Biases Detection and Mitigation}
\label{sec:biases_detection_mitigation}

Traditional bias detection methods, which often focus on sentence-level Neutral Point of View (NPOV) labeling, are limited by data quality and the subtlety of biases \cite{aleksandrovamultilingual}. Recent approaches to reducing biases in LLMs include pre-processing, model adjustments, and post-processing with feedback \cite{Ferrara_2023}. However, interpreting feedback and addressing residual biases remain significant challenges. Furthermore, as demonstrated in Section~\ref{sec:exp1}, labels assigned to controversial articles can be influenced by the annotators' beliefs and emotional reactions, making it nearly impossible for humans to consistently apply noncontroversial labels.

SocraSynth utilizes contentious debates among LLMs to bring diverse viewpoints to the surface, offering an interpretable and dynamic bias mitigation strategy that addresses a fundamental issue in traditional supervised learning: ground-truth labeling.

\subsection*{Wikipedia Quality Assessment}

\begin{figure}[th!]
\begin{center}
\includegraphics[width=0.97\linewidth]{Chapter6/QualityPI-Chart.jpeg}
\end{center}
\caption{Distribution from Top Quality High Importance ($1.2\%$) to Low Quality Low Importance ($91.6\%$). Notably, the blue segment ($4.8\%$) signifies high-importance pages in need of improvement.}
\label{fig:wiki-pichart}
\vspace{-.1in}
\end{figure}


Using Wikipedia as the benchmark for validating the outputs of Large Language Models (LLMs) has gained attention in recent studies \cite{liu2024trustworthy,semnani2023wikichat}. However, there are notable limitations to this method. Firstly, the specific information serving as the ground truth may not always be available on Wikipedia. If the exact answers are already known to chatbot developers, there would be no need to consult LLMs. Secondly, the credibility of this approach is further challenged by the quality assessment of Wikipedia articles themselves. As indicated in Figure~\ref{fig:wiki-pichart}, 91\% of Wikipedia's content is considered to be of middle to low quality by the platform's own editors. (For further details on Wikipedia's quality metrics, refer to Appendix B.)




\begin{comment}
    
%%%%%%  move to the limitation section in the end...

\subsection*{Remarks on Merits and Limitations}
\label{sec:remarks_merits_limitations}

Distinguishing our approach is the use of multiple LLMs for both content evaluation and generation, reducing the risk of inheriting single-model biases \cite{li2023large}. While LLMs facilitate in-depth semantic analysis, we must remain vigilant about the accuracy, comprehensiveness, and legal aspects of content creation. Ensuring the integrity and legal compliance of LLM contributions is paramount to maintaining Wikipedia's reliability as a trusted knowledge repository.
\end{comment}

\begin{comment}

In 2020, an analysis of Wikipedia's top-100 most frequented pages showed significant interest in categories such as \textit{People}, \textit{Politics and History}, \textit{Sports}, \textit{Technology and Online Platforms}, \textit{Entertainment and Arts}, and \textit{Research and Education} \cite{WikiStatics2023}. Monthly page-view statistics further illustrate Wikipedia's diverse usage spanning \textit{Research and Learning}, \textit{Curiosity and Exploration}, and \textit{Entertainment} \cite{WikiGreat2023}. Table~\ref{tab:page_stats} presents the top-ten visited pages in November 2023, highlighting the variety and frequency of content updates, such as the daily revisions in sports-related articles compared to the less frequent updates in historical content.

\begin{table}[ht]
\centering
\begin{footnotesize}
\begin{tabular}{|c|l|r|r|r|}
\toprule
\hline
\textbf{Rank} & \textbf{Page} & \textbf{Edits} & \textbf{Pageviews} \\ \hline
1 & 2023 Cricket World Cup & 532 & 14,148,770 \\ \hline
2 & Cricket World Cup & 199 & 13,917,748 \\ \hline
3 & YouTube & 29 &  6,468,789 \\ \hline
4 & 1234 & 3 &  4,676,115 \\ \hline
5 & Cleopatra & 4 &  4,672,320 \\ \hline
6 & Tiger 3 & 546 &  4,525,333 \\ \hline
7 & Pornhub & 13 & 4,192,495 \\ \hline
8 & Deaths in 2023 & 2,188  & 3,870,414 \\ \hline
9 & XNXX & 33 & 3,837,659 \\ \hline
10 & 2024 Men's World Cup & 447 &  3,749,162 \\ \hline
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-.1in}
\caption{Top 10 Pages Statistics in November 2023}
\vspace{-.15in}
\label{tab:page_stats}
\end{table}
\end{comment}

\begin{comment}
\begin{figure}[th!]
\begin{center}
\includegraphics[width=0.97\linewidth]{QualityPI-Chart.jpeg}
\end{center}
\caption{Distribution from Top Quality High Importance ($1.2\%$) to Low Quality Low Importance ($91.6\%$). Notably, the blue segment ($4.8\%$) signifies high-importance pages in need of improvement.}
\label{fig:wiki-pichart}
\vspace{-.1in}
\end{figure}
\end{comment}


==> Chapter7/CaseStudy1.tex <==
\section{Case Study with SocraHealth}
\label{sec:CaseStudy2}

In this case study, we explore the application of SocraHealth using a dataset obtained from Kaggle \cite{KaggleDSDD2020}, comprising $4,921$ patient records. Each record in this dataset includes critical information such as the diagnosed disease or medical condition, along with symptoms like fever, cough, fatigue, itchiness, and difficulty breathing, among others. The most comprehensive record details up to $14$ distinct symptoms.

{\center{\subsection*{III.A Experiment Setup \& Data Preparation}}}

We started by converting our raw spreadsheet dataset into JSON format, turning each record into a distinct diagnostic entry. The data was divided into a training set (90\%) and a testing set (10\%). Utilizing a decision-tree model, as described in \cite{KaggleSD2021}, we achieved a 94\% accuracy in precision and recall with Support Vector Machines (SVMs), and 99\% accuracy with Gradient Boosting.

However, these results, though promising, may not completely mirror real-world diagnostic complexities. The dataset, for instance, potentially includes an average 5\% misdiagnosis rate, in line with U.S. statistics \cite{Newman-Tokerbmjqs-2021-014130}. It also lacks essential information such as patient profiles and medical histories, limiting its application in more complex cases. Despite these constraints, this Kaggle dataset forms a robust baseline.

In the case study, two LLM agents, one using GPT-4 \cite{Bbubeck2023sparks} and the other Bard \cite{Bard2023}, are employed to assess the predictions of a Kaggle classifier. They participate in structured debates, generating queries to assist a General Practitioner (GP) in identifying symptoms and recommending lab tests. This process is expected to yield varied disease diagnoses and rationales, providing valuable insights for GPs.

For the two experiments presented, the agents initially offer a disease prediction and justification. They then critically appraise each other's predictions in a series of rounds. This iterative process aims to reach consensus or identify the need for further medical evidence. The final outcome, if differing from the Kaggle dataset's ``ground truth,'' could suggest areas for data correction. This method underscores the potential of LLMs in refining medical diagnostics.

\subsection*{\centering{III. B Experiment \# 1}}

In the first experiment, both LLM agents receive an identical list of symptoms from the moderator, aimed at guiding disease diagnosis, facilitating debate, and shaping subsequent recommendations. It is important to note that the ``ground-truth'' disease in this scenario is Hepatitis.

\subsection*{\textbf{B.1 Moderator's Opening Prompt}}

``What potential disease could be associated with the following symptoms: itching, fatigue, lethargy, yellowish skin, dark urine, loss of appetite, abdominal pain, yellowing of the eyes, malaise, history of receiving a blood transfusion, and exposure to unsterile injections? Please offer one prediction, supported by justifications. Additionally, include a list of supplementary symptom inquiries and recommend relevant lab tests to strengthen the confidence in your prediction.''

\subsection*{\textbf{B.2 Bard's Opening Round}}

\subsection*{Single Prediction: Jaundice}

\subsection*{B.2.1 Justifications:}

Jaundice is a condition characterized by the yellowing of the skin and eyes due to the accumulation of bilirubin in the blood.
The symptoms you listed are all common symptoms of jaundice, including itching, fatigue, lethargy, yellowish skin, dark urine, loss of appetite, abdominal pain, and yellowing of the eyes.
Receiving a blood transfusion or unsterile injections can increase the risk of developing jaundice, as these can transmit infections that can damage the liver.

\subsection*{B.2.2 Supplementary Symptom Inquiries}

This additional list of symptom inquiries could enhance diagnostic certainty:

\begin{enumerate}[left=0em,label=\arabic*.]
\item ``Have you noticed any changes in your stool color?'' (Jaundice can cause pale or clay-colored stools.)
\item ``Have you noticed any changes in your urine color?'' (Jaundice can cause dark or amber-colored urine.)
\item ``Have you had any recent abdominal pain?'' (Jaundice can cause pain in the upper right abdomen.)
\item ``Have you had any recent weight loss?'' (Jaundice can cause unexplained weight loss.)
\item ``Do you have any history of liver disease?'' (Jaundice is more common in people with pre-existing liver disease.)
\end{enumerate}

\subsection*{B.2.3 Relevant Lab Tests}

Liver function tests (LFTs) to measure the levels of bilirubin and other liver enzymes in the blood.
Complete blood count (CBC) to check for signs of infection or anemia.
Coagulation tests to check the blood's ability to clot.
Ultrasound of the abdomen to look for any abnormalities in the liver or gallbladder.

\subsection*{\textbf{B.3 GPT-4's First Round}}
\subsection*{Single Prediction: Hepatitis}
\subsection*{B.3.1 Justifications:}

Yellowish Skin and Eyes: Yellowing of the skin and eyes is a common symptom of hepatitis due to the buildup of bilirubin in the bloodstream.
Fatigue and Lethargy: Fatigue and lethargy are typical symptoms of hepatitis, often accompanied by a feeling of weakness.
Dark Urine: Dark urine can result from liver dysfunction, which is commonly associated with hepatitis.
Loss of Appetite: Hepatitis can lead to a loss of appetite and weight loss.
Abdominal Pain: Abdominal pain is a common symptom in hepatitis, particularly in the upper right quadrant where the liver is located.
Malaise: Malaise, a general feeling of discomfort or illness, is often experienced by hepatitis patients.
Receiving Blood Transfusion and Unsterile Injections: These factors could increase the risk of hepatitis transmission, especially if proper infection control measures were not followed.

\subsection*{B.3.2 Additional Symptom Inquiries}

\begin{enumerate}[left=0em,label=\arabic*.]
\item Nausea and Vomiting: Inquiring about nausea and vomiting can help confirm the likelihood of hepatitis.
\item Fever: Hepatitis can sometimes be associated with a fever.
\item Joint Pain: Joint pain can be present in some cases of hepatitis.
\item Clay-Colored Stool: This is another stool-related symptom that can be associated with hepatitis.
\end{enumerate}

\subsection*{B.3.4 Relevant Lab Tests}

Hepatitis Panel: A hepatitis panel can confirm the presence of hepatitis and determine the specific type (e.g., hepatitis A, B, C).
Liver Function Tests: These tests can assess the liver's health and function.
Bilirubin Levels: Elevated bilirubin levels in the blood can confirm jaundice.
Serology Testing: Serologic tests can help identify the specific hepatitis virus responsible.
Ultrasound or Imaging: Imaging studies can evaluate the condition of the liver and nearby organs.

\subsection*{\textbf{B.4 Bard's Second Round}}

Bard's second round is given GPT-4's diagnosis, and we
ask Bard to defend its ``Jaundice'' prediction and
refute GPT-4 ``Hepatitis'' prediction.

\subsection*{B.4.1 Bard's Defense:}

Jaundice is the most common cause of yellowing of the skin and eyes, which is the most prominent symptom in the given list.
All of the other symptoms listed are also common symptoms of jaundice.
Receiving a blood transfusion or unsterile injections can increase the risk of developing jaundice, as these can transmit infections that can damage the liver.

\subsection*{B.4.2 Refutation of GPT-4's Hepatitis Diagnosis}

GPT-4's diagnosis of hepatitis is also supported by the given evidence. However, I believe that jaundice is the more likely diagnosis due to the following reasons:

Jaundice is a more specific diagnosis, while hepatitis is a more general term for inflammation of the liver.
Jaundice can be caused by a variety of factors, including hepatitis, but it can also be caused by other conditions such as gallstones, tumors, and drug toxicity.
The fact that the patient received a blood transfusion or unsterile injections makes jaundice a more likely diagnosis than hepatitis, as these factors can increase the risk of developing jaundice but not hepatitis.


\subsection*{\textbf{B.5 GPT-4's Second Round}}

Now GPT-4 is given Bard's counterarguments to
defend its ``Hepatitis'' prediction.

\subsection*{B.5.1 GPT-4's Defense}

My diagnosis of hepatitis is based on the following justifications:

Specificity: Hepatitis refers to inflammation of the liver, and it can manifest as jaundice, which is the yellowing of the skin and eyes. While jaundice is a common symptom of hepatitis, it's important to note that jaundice itself is not a disease but a symptom of an underlying issue. Hepatitis provides a more specific diagnosis that pinpoints the inflammation of the liver as the primary concern.

Causative Factors: Hepatitis can be caused by various factors, including viral infections (such as hepatitis A, B, or C), alcohol consumption, drug toxicity, or autoimmune disorders. Given the patient's history of receiving unsterile injections and blood transfusions, there is a higher likelihood of viral transmission, leading to hepatitis. Hepatitis viruses, especially hepatitis B and C, can be transmitted through contaminated needles and blood products, making them a plausible cause in this context.

Comprehensive Assessment: While jaundice is a significant symptom, a diagnosis should consider a broader range of liver function and potential causes. Hepatitis encompasses a more comprehensive assessment of liver health, including liver enzyme levels and viral markers, which can aid in confirming the diagnosis and identifying the specific type of hepatitis.

\subsection*{B.5.2 Refutation of Bard's Jaundice Diagnosis}

My diagnosis of ``Hepatitis'' is more specific and considers a broader range of potential causes, especially given the patient's history of risky medical procedures. While jaundice is a symptom, it's essential to identify the underlying condition causing it, which, in this case, is likely hepatitis.

\subsection*{\textbf{B.6 Bard Concedes to GPT-4}}

Bard aligns with GPT-4's evaluation, recognizing ``Hepatitis'' as the likely diagnosis. However, considering that even the ``ground truth'' in the training dataset might be statistically 5\% incorrect as per U.S. misdiagnosis data \cite{Newman-Tokerbmjqs-2021-014130}, this agreement alone isn't definitive. To solidify the ``Hepatitis'' diagnosis, SocraHealth suggests further steps.

\subsection*{\textbf{B.7 Final Joint Recommendations to GP}}

Bard and GPT-4 jointly recommend the following additional symptom inquiries and lab tests to confirm a hepatitis diagnosis:

\subsection*{B.7.1 Additional Symptom Inquiries:}

\begin{enumerate}[left=0em,label=\arabic*.]
\item \textbf{Onset and Duration}: Determining the onset and duration of symptoms can clarify the illness timeline and its progression.
\item \textbf{Severity and Trend}: Evaluating symptom severity and whether they're worsening or improving aids in understanding the disease's trajectory and treatment responses.
\item \textbf{Associated Symptoms}: Checking for additional symptoms like nausea, vomiting, fever, joint pain, or urine color changes can pinpoint other hepatitis indicators and exclude other conditions.
\end{enumerate}

\subsection*{B.7.2 Recommended Lab Tests}

\begin{enumerate}[left=0em,label=\arabic*.]
\item \textbf{Liver Function Tests (LFTs)}: Critical for assessing liver health, LFTs evaluate enzyme levels such as alanine aminotransferase (ALT) and aspartate aminotransferase (AST), where abnormalities can signify liver inflammation.
\item \textbf{Hepatitis Panel}: This test checks for hepatitis A, B, and C viruses, vital for determining the specific type and guiding treatment strategies.
\item \textbf{Serology Testing}: Useful for distinguishing between acute and chronic hepatitis by identifying specific antibodies or antigens.
\item \textbf{Imaging Studies}: Techniques like ultrasound or MRI provide visual insights into the liver's state, detecting inflammation, fibrosis, or cirrhosis, thereby complementing blood-based diagnostics.
\end{enumerate}



==> Chapter7/CaseStudy2.tex <==
{\center{\subsection*{III.C Experiment \# 2}}}

In the second experiment, we confront a diagnostic challenge involving multiple candidate diseases. A patient exhibits the following $12$ symptoms: skin rash, joint pain, vomiting, fatigue, high fever, headache, nausea, loss of appetite, pain behind the eyes, back pain, malaise, muscle pain, and red spots over the body. For this experiment, we initially allow GPT-4 to conduct the diagnosis, followed by the Bard.
Note that the ``ground-truth'' disease of this diagnosis instance 
is Dengue Fever.

\vspace{0.1in}
\subsection*{\textbf{C.1 Moderator's Opening Prompt}}

``What potential diseases could be associated with this set of the above symptoms? Kindly offer three top predictions supported by justifications. Additionally, furnish a list of supplementary symptom inquiries and propose relevant lab tests that could enhance the confidence level of your diagnosis.''

%``What potential diseases could be associated with this set of symptoms: skin rash, joint pain, vomiting, fatigue, high fever, headache, nausea, loss of appetite, pain behind the eyes, back pain, malaise, muscle pain, and red spots over the body? Kindly offer three top predictions supported by justifications. Additionally, furnish a roster of supplementary symptom inquiries and propose relevant lab tests that could enhance the confidence level of your diagnosis.''

\subsection*{\textbf{C.2 GPT-4's Opening Round}}

\subsection*{Top-3 Predictions: Dengue Fever, Chikungunya, and Zika Virus}

\subsection*{C.2.1 Justifications}

The symptoms of high fever, severe headache, pain behind the eyes, joint and muscle pains, fatigue, nausea, vomiting, and skin rash are classic signs of dengue fever. Red spots over the body could correspond to petechiae, which are often seen in dengue due to thrombocytopenia (a decrease in platelet count).

Chikungunya can cause similar symptoms to dengue, such as fever, severe joint pain, muscle pain, headache, nausea, and rash. Joint pain from chikungunya is often very debilitating and can be more prolonged than in dengue.

Zika virus symptoms can include fever, rash, joint pain, malaise, and conjunctivitis, with a milder presentation compared to dengue or chikungunya. The presence of a rash and conjunctivitis are notable, although Zika is less likely to cause severe muscle pain or high fever.

\subsection*{C.2.2 Supplementary Symptom Inquiries}

Travel history is significant, as is the time of year. For confirming dengue fever, additional symptoms to consider include the presence of bleeding gums, nosebleeds, or easy bruising, which could suggest a more severe form of the disease.

\subsection*{C.2.3 Relevant Lab Tests}

Complete blood count (CBC) focusing on platelet count, dengue NS1 antigen test, dengue IgM and IgG antibodies serology tests, and PT-PCR tests.


\subsection*{\textbf{C.3 Bard's Opening Round}}

\subsection*{Top-$3$ Predictions: Chikungunya	($50\%$),
Dengue fever ($25\%$), and Influenza ($10\%$)}

\subsection*{C.3.1 Justifications}

As shown on the left-hand side of Figure~\ref{fig-Bard-BA},
Chikungunya is the most likely disease ($50\%$) based on the symptoms provided. It is a viral infection that is spread by mosquitoes. The symptoms of chikungunya typically include fever, joint pain, muscle pain, headache, nausea, vomiting, and fatigue. A rash may also develop.

Dengue fever is another possible disease based on the list of symptoms. It is also a viral infection that is spread by mosquitoes. The symptoms of dengue fever typically include fever, headache, muscle and joint pain, nausea, vomiting, and rash.

Influenza is the least likely disease based on the symptoms. It is a respiratory infection that is caused by a virus. The symptoms of influenza typically include fever, cough, sore throat, runny or stuffy nose, muscle or body aches, headaches, fatigue, and sometimes vomiting or diarrhea.

\subsection*{C.3.2 Supplementary Symptom Inquiries}

For a more accurate diagnosis of chikungunya, the following specific symptoms are key indicators, helping to differentiate it from other viral infections like dengue fever or influenza:

\begin{enumerate}[left=0em,label=\arabic*.]
\item {Swollen Lymph Nodes}: Particularly in the neck, armpits, or groin, swollen lymph nodes are a notable symptom of chikungunya.
\item {Photophobia}: Sensitivity to light, or photophobia, is a less frequent but indicative symptom of chikungunya.
\item {Conjunctivitis}: Inflammation of the conjunctiva, which is the lining of the eyelids and eyeball, is commonly seen in chikungunya cases.
\item {Arthralgia}: Persistent joint pain, often lasting weeks or months after the initial fever and rash, is a distinguishing feature of chikungunya.
\end{enumerate}

\subsection*{C.3.3 Relevant Lab Tests}

A similar lists of IgM antibody tests and PCR tests are
recommended, along with complete blood count (CBC),
C-reactive protein (CRP) test, and
liver function tests (LFTs). 

\subsection*{\textbf{C.4 GPT-4's Second Round}}

First GPT-4 disagrees with assigning probability to
predictions. It states that:
``The accuracy of disease probability estimates varies based on models, data inputs, and symptom emphasis.'' In critiquing the Bard's predictions:

\begin{enumerate}[left=0em,label=\arabic*.]
\item Chikungunya ($50\%$): The focus on joint pain for Chikungunya may be overstated without considering epidemiological factors. Symptoms like high fever and red spots, more indicative of dengue fever, weren't sufficiently emphasized.

\item Dengue Fever ($25\%$): The symptom list, aligning closely with dengue fever's classic presentation, suggests a higher probability for dengue, especially considering the presence of red spots, a sign of potential hemorrhagic fever.

\item Influenza ($10\%$): Influenza's inclusion seems less fitting due to the absence of respiratory symptoms and the presence of symptoms more typical of mosquito-borne diseases.
\end{enumerate}

Zika Virus, omitted by the Bard but relevant here, and the lack of laboratory test consideration are notable oversights. A more accurate diagnosis requires integrating symptom analysis with patient history, epidemiological data, and lab tests.

\subsection*{\textbf{C.5 Bard's Second Round}}

\begin{figure}[t!]
    \centering
    \begin{minipage}[b]{0.46\linewidth}
        \includegraphics[width=\linewidth]{Chapter7/Bard-1st-Round.png}
    \end{minipage}
    \hspace{-.1in} % Optional: add some horizontal spacing
    \begin{minipage}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{Chapter7/Bard-2nd-Round.png}
    \end{minipage}
\vspace{.05in}
\captionsetup{font=small, justification=raggedright}
\caption{Bard's Diagnoses Comparison: 1st Round (left) vs. 2nd Round (right). Initially, Bard prioritizes Chikungunya, but in the second round, aligns with GPT-4's assessments, giving the highest weight to Dengue Fever.}
\label{fig-Bard-BA}
\vspace{-.15in}
\end{figure}

As the moderator, I prompted Bard to critically challenge GPT-4's predictions. Nevertheless, Bard largely aligned with GPT-4
as shown on the right-hand side of Figure~\ref{fig-Bard-BA}, offering this response:

``After carefully considering the feedback from GPT-4, I would revise the order of my top-$3$ predictions for the given symptoms as follows:

I still believe that chikungunya is a possible diagnosis, but I agree with GPT-4 that the symptoms are more consistent with dengue fever, especially given the presence of red spots over the body. Zika virus is also a possibility, especially if the patient has a history of travel to an area where Zika virus is prevalent.''

\begin{enumerate}[left=0em,label=\arabic*.]
\item \textbf{Dengue Fever (40\%)}: Patient symptoms closely align with dengue fever, including high fever, severe headache, pain behind the eyes, muscle and joint pains, and red spots over the body. Red spots may suggest hemorrhagic manifestations, a severe dengue complication.
\item \textbf{Chikungunya (30\%)}: Symptoms like high fever, severe joint pain, muscle pain, and headache match chikungunya. Yet, the skin rash and red spots are more indicative of dengue fever.
\item \textbf{Zika Virus (20\%)}: Given symptoms of fever, rash, joint pain, and conjunctivitis, Zika virus is a potential diagnosis. However, its typically mild presentation contrasts with the severity of the patient's symptoms.
\end{enumerate}


\subsection*{\textbf{C.6 Final Joint Recommendations to GP}}

After seeking further input from GPT-4, Bard fully concurred with GPT-4's final suggestions, even though the moderator had instructed Bard to maintain its original stance.

A comprehensive diagnostic approach for dengue fever requires a combination of clinical assessment, laboratory testing, and consideration of the patient's history and epidemiological context.

Clinical symptoms such as skin rash, joint pain, vomiting, and red spots over the body provide valuable clues to the diagnosis, but additional symptoms like nausea, vomiting, diarrhea, bleeding, bruising, and drowsiness can indicate the severity and progression of the disease.

Laboratory tests play a crucial role in confirming dengue fever. The Dengue NS1 antigen test is useful for early detection during the first few days of illness, while the Dengue IgM and IgG antibody tests help determine recent or past infection. Dengue PCR offers direct viral detection, and CBC and LFTs assess for blood cell abnormalities and liver involvement, respectively.

A thorough patient history is equally important. Travel history to dengue-endemic areas, recent mosquito exposure, local epidemiological context, symptom timeline, a complete review of other symptoms, and past medical history, particularly previous dengue infections, all contribute to a more accurate diagnosis.

In conclusion, both GPT-4 and Bard emphasize the importance of a holistic approach to dengue fever diagnosis, encompassing clinical assessment, laboratory testing, and a thorough understanding of the patient's history and epidemiological context. This comprehensive approach ensures accurate diagnosis, risk assessment, and appropriate patient management.

{\center{\subsection*{III.D Observations}}}

This case study serves as a testament to the strengths of SocraHealth, which not only harnesses the vast knowledge of Language Model models (LLMs) but also excels in providing comprehensive narratives and conducting rigorous reasoning processes, for example by providing precise and personalized differential diagnoses for each clinical scenario. This approach surpasses the utility of linear prompts typically provided by users. It bypasses common diagnostic fallacies afforded by premature closure or availability heuristics, thus offering a more thorough and insightful diagnostic experience.

The debate between Bard and GPT-4 exhibited a logical and coherent exchange of arguments, devoid of any hallucinatory elements. This absence of hallucination can be attributed to the precise formulation of all prompts involved in the debate. In a confrontational debate format, both sides present arguments and counterarguments, resulting in the formulation of precise and concise prompts that leave minimal room for misunderstanding.

Through a few rounds of debate, any initial confusion or ambiguity is effectively distilled, resulting in clear and well-reasoned conclusions. This case study serves as a testament to the strengths of SocraHealth, which not only harnesses the vast knowledge of Language Model models (LLMs) but also excels in providing comprehensive narratives and conducting rigorous reasoning processes. This approach surpasses the utility of linear prompts typically provided by users, offering a more thorough and insightful diagnostic experience.

It's noteworthy that while SocraHealth's conclusions in both experiments aligned with the ``ground truth'', further investigations through symptom probing and lab tests could reveal inaccuracies in this ``truth''. This highlights SocraHealth's advantage over traditional supervised learning paradigms, where training data labels are often accepted as infallible. SocraHealth adds value by questioning and refining these accepted truths.










==> Chapter7/Introduction.tex <==
\section*{Introduction}
\label{sec:intro}

Disease diagnosis is crucial in healthcare, involving identifying conditions based on symptoms, medical history, physical examinations, and lab tests \cite{peng2018refuel}. Accurate diagnosis is vital, yet misdiagnosis is a significant global issue, as highlighted by Newman-Toker \cite{Newman-Tokerbmjqs-2021-014130}, with vast implications for patient treatment and outcomes.

Misdiagnosis leads to delayed or inappropriate treatment, worsening patient conditions, and emotional and financial burdens. Contributory factors include lab test limitations, complex symptom-to-disease mapping, and data deficiencies, including outdated disease profiles and incomplete patient data. Alarmingly, AI algorithms trained on such flawed data perpetuate historical diagnostic errors into future cases. Addressing this cycle of mistakes is a critical challenge.

SocraHealth, presented in this chapter, is an innovative approach that blends medical expertise with Large Language Models (LLMs) to enhance diagnostic accuracy and correct historical errors in medical records. Leveraging LLMs' extensive knowledge bases and poly-disciplinary capabilities, detailed in the study of \cite{ChangSocraSynthCSCI2003}, SocraHealth uses the SocraSynth framework for structured LLM collaborations. This method explores diagnostic possibilities and collaborates with professionals for conclusive assessments.

This chapter details the diagnostic process, highlighting LLMs' role, and presents SocraSynth’s facilitation of diagnostic debates. The included case studies demonstrate the efficacy of this approach, not only in refining diagnostic precision and improving patient outcomes but also in tackling historical diagnostic errors. This is achieved by identifying discrepancies between the training data used for AI algorithms and the outcomes of structured debates, thereby rectifying past inaccuracies in medical records.


==> Chapter7/Main007SocraHealth.tex <==
\noindent{\textbf{Abstract}}
This study introduces SocraHealth, an innovative approach that utilizes Large Language Models (LLMs) for medical diagnostics. By engaging LLM-based agents in structured dialogues, SocraHealth refines diagnoses and corrects inaccuracies in historical records, making effective use of patient data. The case study, featuring GPT-4 and Bard across two experiments, illustrates the success of this method in generating logical, hallucination-free debates. Representing a significant advancement over traditional diagnostic techniques, SocraHealth underscores the transformative potential of LLMs in healthcare, particularly in improving diagnostic accuracy and rectifying previous errors.

\input{Chapter7/Introduction}
\begin{comment}
\input{Chapter7/SocraHealth}
\input{Chapter7/CaseStudy1}
\input{Chapter7/CaseStudy2}
\vspace{0.1in}
\section{Concluding Remarks}
\label{sec:conc8}

In concluding, SocraHealth, leveraging the SocraSynth framework, marks a pivotal advancement in disease diagnosis. This approach, integrating multiple LLMs in an adversarial setup, ensures analytical rigor and minimizes errors. The employment of conditional statistics addresses LLM biases, leading to an insightful analysis. Importantly, SocraHealth not only enhances diagnostic precision but also plays a crucial role in correcting historical inaccuracies in medical records. The fine-tuning of adversarial interactions optimizes the collaboration between AI and human intelligence, moving from intense debates to harmonious conclusions. This innovative methodology, as demonstrated in our case studies, signifies a transformative step in healthcare diagnostics, blending advanced AI capabilities with the critical need for accuracy and historical rectification.

For a set of aphorisms supporting SocraSynth and its applications, please refer to Appendix $X_2$ in the book.
\end{comment}

==> Chapter8a/CaseStudy.tex <==
\section{Case Study}
\label{sec:casestudy9}

As highlighted in Sections~\ref{sec:related} and \ref{sec:SocraPlan}, significant advancements in data collection and analytics have been achieved and implemented as co-pilot services by major corporations, such as Microsoft and Salesforce. Due to constraints in scope, our case study will specifically focus on evaluating the formulation of a {\em sales playbook} that consists of a sequence of plays, emphasizing Steps \#7 and \#8 in the SocraPlan framework. Step \#7 involves drafting (or searching) an initial playbook, while step \#8 entails the integration of these draft plans into a final, comprehensive one. This final sales playbook is meticulously crafted to ensure efficient and effective execution in real-world sales scenarios.

To effectively navigate our case study, we organize the process into four essential steps:
\begin{enumerate}[left=0em,label=\arabic*.]
\item {\em Metrics Definition}: We define key metrics such as goal alignment, relevance to the customer, usability, clarity, and content quality \cite{ChallengerSales2011}. We exclude customer conversion rates to minimize the impact of variable sales personnel quality.
\item {\em Benchmark Dataset Creation}: We compile a dataset of playbook components, similar to sports strategies, referred to as plays or techniques.
\item {\em Playbook Generation}: For specific products and target customers, we design and automatically generate a preliminary playbook $\Psi$ comprising a series of tactics.
\item {\em Playbook Optimization}: We employ SocraSynth to select and refine the plays, tools, and data for each tactic within $\Psi$, resulting in the optimized playbook $\Psi^*$.
\end{enumerate}

\subsection{Evaluation Dataset: Strategies, Tactics, Plays}

Initially, given products and customers, SocraPlan identifies an appropriate sales strategy. The selection process considers various strategies relevant to distinct industries and product/customer scenarios.  Some textbook strategies are:

\begin{enumerate}[left=0em,label=\arabic*.]
\item
{\em Value Selling}: Aims to communicate the product's or service's value, often in terms of ROI or other business outcomes.
\item
{\em Solution Selling}: Centers on identifying and addressing a customer's specific pain points with a tailored solution.
\item
{\em SPIN Selling} (situation, problem, implication, need-payoff): Focuses on finding and developing the customer's implicit needs.
\item
{\em Challenger Sale}: Emphasizes challenging the customer's thinking, providing insights that disrupt their status quo.
\end{enumerate}

After determining the sales strategy, a Playbook Development Table (PDT) is chosen to support that strategy in developing a sales playbook. Table~\ref{tab:SPDTLegos} displays a subset of the PDT used by Company T (anonymous) for the {\em solution selling} strategy, noting that only a portion is shown due to confidentiality.

\subsection{Generating Sales Playbook}
\label{sec:tactic-to-plays}

The next step involves developing diverse sales playbooks, each consisting of a series of actionable steps known as plays. These plays, tailored to specific tactics within a given scenario such as the case of Company T (anonymous), are numbered from 1 (awareness) to 10 (advocacy).

The selection of plays takes into account various factors including the products offered, the type of sales scenario (e.g., new sales, expansion, renewal), the customer's budget, and current cyber threats. After determining the most suitable plays for each tactic, recommendations on relevant data (in Table~\ref{tab:required-data}), tools, and processes are provided. The playbook, $\Psi$, dynamically adapts over time, integrating insights from customer interaction history (CIH) and frequently asked questions (FAQs), thereby enabling the refinement of plays and techniques.

For each tactic in the playbook, denoted as tactic$_i$, SocraPlan identifies a subset of specific plays, play$_{i,j}$. Upon establishing these subsets for all tactics, the initial version of the playbook, $\Psi^*$, is formulated. This playbook undergoes continuous refinement, leveraging newly gathered data, addressing emerging questions, and making adjustments to align with the dynamic nature of sales cycles, ensuring the playbook remains effective and relevant.

\begin{figure*}[th]
  \centering
\includegraphics[height=0.78\linewidth,width=1.0\linewidth]{Chapter8/fig3Sales_PlayBook_v1_spark.png}
\vspace{-.2in}
  \caption{A Sales Playbook Comprising Eight Sales Plays: This playbook initiates by selecting relevant tactics for customer sales, followed by designing and refining plays, along with their associated tools and data for each tactic.}
  \label{fig:plays}
\end{figure*}

\subsection{Experiments}

Our experiments were designed to evaluate the effectiveness of a sales playbook before and after refinement using SocraPlan. Initially, SocraPlan generates a preliminary playbook by identifying a sequence of pertinent tactics from the SPDT, as depicted in Table~\ref{tab:SPDTLegos}, utilizing the gathered intelligence. For each chosen tactic$_i$, SocraPlan then selects the most effective techniques, designated as play$_{i,j}$, to optimize its effectiveness. The complexities of data preparation, the deployment of SocraPlan for evaluating alternatives, and the creation of a unified playbook, due to spatial limitations, are elaborated upon in the Appendix.

\subsubsection{Moderator Prompts}

The moderator presented all relevant data as context, along with the Sales Playbook Development Template (SPDT) detailed in Table~\ref{tab:SPDTLegos}. Agent A (GPT-4) was then assigned to craft a sales plan, starting with selecting appropriate tactics from ten options listed in the table's first tier. Upon establishing a sequence of tactics, Agent A outlined a preliminary playbook structure, depicted in Figure~\ref{fig:plays}, featuring the six tactics deemed most effective for the target customer. Subsequently, Agent A chose the best techniques (plays) for each tactic from SPDT's second tier, taking into account factors like customer personas, product profiles, market surveys, and threat analyses, among others. Notably, a single tactic could involve several plays. For each play, Agent A identified the most suitable tools and data for execution. For instance, in initiating customer outreach, LLM tools from Salesforce and McKinsey were suggested to draft the engagement letter and subsequent communications.

Once Agent A proposed its playbook $\Psi$, a debate was initiated between two GPT-4 agents, A and B, with Agent A defending the playbook and Agent B critiquing it. Their exchange, rich in arguments and counterarguments, began with a high contentiousness setting (0.9) to thoroughly explore the playbook's merits and demerits. After three rounds of debate, the contentiousness was reduced to 0.3 to foster a consensus-driven proposal, as detailed in Table~\ref{tab:contentiousness}, which outlines the linguistic features influenced by the contentiousness level. This refined proposal, $\Psi^*$, emerged as the ``optimal'' playbook.

\subsubsection{Evaluation}

We executed multiple experimental runs to assess the effectiveness of the sales playbooks before and after the debate and refinement. 
The evaluation criteria were derived from five metrics as outlined by Dixon et al. \cite{ChallengerSales2011}: alignment with sales objectives, relevance to the intended customer base, provision of actionable guidance, clarity and structural organization, and the overall quality of content. These metrics were rated on a scale from 1 (lowest) to 10 (highest).

For an automated evaluation, we employed the CRIT algorithm \cite{SocreticMethodChang2023}, which utilizes the Socratic method to assess the quality of reasoning. The CRIT algorithm has been previously applied in numerous studies, e.g., \cite{SocraHealth2023,SocraPediaDecember2023,ChangSocraSynthCSCI2003,SocraPlan2023}, where it has proven to be an effective tool for evaluating the reasoning quality of arguments. CRIT employed GPT-4 and
Bard to conduct two evaluations. 
Additionally, we engaged senior sales representatives to perform blind reviews of the playbooks. The comparative results are summarized in Table~\ref{tab:comparison}.

\begin{table}[th!]
\centering
\label{tab:playbook_evaluation}
\begin{footnotesize}
\begin{tabular}{|p{1.5cm}|cc|cc|cc|}
\toprule
\hline
\textbf{} & \multicolumn{2}{c|}{\textbf{Human Expert}} & \multicolumn{2}{c|}{\textbf{GPT}} & \multicolumn{2}{c|}{\textbf{Bard}} \\
\hline
\textbf{Metric} & \textbf{$\Psi$} & \textbf{Refined $\Psi^*$} & \textbf{$\Psi$} & \textbf{Refined $\Psi^*$} & \textbf{$\Psi$} & \textbf{Refined $\Psi^*$} \\
\hline
Alignment & 6 & 8 & 9 & 9 & 7 & 9 \\
\hline
Engagement & 7 & 9 & 8 & 9 & 8 & 10 \\
\hline
Actionable & 7 & 10 & 9 & 10 & 9 & 9 \\
\hline
Clarity & 8 & 8 & 9 & 9 & 8 & 9 \\
\hline
Quality & 7 & 9 & 8 & 9 & 9 & 9 \\
\hline
\end{tabular}
\end{footnotesize}
\vspace{.05in}
\caption{Evaluation conducted by humans, GPT-4, and Bard, respectively. $\Psi$ represents the initial playbook drafted by Agent A, while $\Psi^*$ signifies the optimized playbook produced following three rounds of refinement by both agents.}
\label{tab:comparison}
\vspace{-.1in}
\end{table}

The debate mechanism of SocraSynth enhanced the robustness and thoroughness of the final playbook $\Psi^*$. This procedure was marked by the introduction of novel ideas and perspectives. LLM agents were actively engaged in arguments and counterarguments, tackling subjects with new viewpoints. Intriguingly, we discerned that playbook $\Psi^*$ integrated additional elements from SPDT, molding a strategy 
in tune with up-to-date data and current circumstances.

Table~\ref{tab:comparison} shows that the customized playbook significantly surpassed the standard version in aligning with the customer's persona, enhancing customer engagement, and providing actionable guidance. Experts noted that customized playbooks, which incorporate real data and figures, are viewed as more engaging and practical compared to generic templates, thus more effectively connecting with the customer's actual situation. Further experimental iterations, incorporating changes in decision contexts, are detailed in Section~\ref{sec:more_experiments} in the Appendix. SocraPlan proves to be instrumental in devising detailed plays and strategies to boost sales effectiveness.

==> Chapter8a/Conclusion.tex <==
\section{Concluding Remarks}
\label{sec:concPlan}

SocraPlan exemplifies the crucial role of merging human insight with the computational intelligence of Large Language Models (LLMs), promoting a collaborative partnership between human expertise and AI capabilities. Rooted in the SocraSynth methodology, 
this teamwork ensures that when creating sales plans, both the complex details of the data and the subtle differences in the market are considered.

Our initial qualitative evaluation of the SocraPlan-crafted sales playbook for a potential client sets a solid foundation for its empirical assessment. The ultimate test of its utility will hinge on tangible business metrics, such as enhancements in lead-to-customer conversion rates and overall revenue growth. As SocraPlan progresses, our commitment is to continuously assess its impact, gather feedback, and disseminate the knowledge acquired from its deployment. SocraPlan demonstrates the profound capability of LLMs to navigate and interpret complex data landscapes, thereby enabling the formulation of strategic business plans that are rooted in deep analysis and critical reasoning. Furthermore, we are eager to refine SocraPlan's algorithms to enhance its capacity for generating sales narratives that not only appeal to the logical aspects of decision-making but also resonate on an emotional level \cite{frisch2024llm}, thereby deepening customer engagement.

While we acknowledge the significant progress achieved, we also recognize the limitations of our current study and propose directions for future research:
\begin{enumerate}[left=0em,label=\arabic*.]
\item The efficacy of SocraPlan largely depends on the richness and comprehensiveness of the data it utilizes.
\item Designed primarily for interactions with existing customers, the current version of SocraPlan faces challenges in addressing the needs of potential customers who may not have extensive data available.
\item Our future work will focus on expanding the applicability of SocraPlan to a wider array of customer scenarios, including engagements with new prospects. We also plan to further refine the AI model to enhance its precision and minimize biases, thereby increasing its effectiveness across various sales contexts.
\end{enumerate}

Through these efforts, we aim to not only augment the capabilities of SocraPlan but also to contribute valuable insights to the evolving field of AI-driven sales optimization, pushing the boundaries of how artificial intelligence can augment and enrich human-driven sales processes.

==> Chapter8a/DataSources.tex <==
\begin{sidewaystable*}[ht!]
\centering
\small
%\begin{tabularx}{\textwidth}{|p{1.88cm}|p{4.0cm}|p{5.6cm}|p{1.3cm}|}
%\begin{tabularx}{|p{1.88cm}|X|X|p{1.6cm}|}
\begin{tabularx}{\textwidth}{|p{1.88cm}|p{4.0cm}|X|p{1.0cm}|}
\toprule
\hline
\textbf{Category} & \textbf{Data Type} & \textbf{Description}       & \textbf{Src} \\ \hline
{\bf Customer} & Product Feedback Data                     & Records from customer service interactions (email, meeting transcripts, etc.)  & $I_s$, $P$     \\ \cline{2-4} 
{\bf Satisfaction} & {Customer Feedback}  & {Surveys, questionnaires, product reviews, and ratings} & $I_s$ \\ \cline{2-4} 
& Sales and Usage Data                          & Purchase history and usage patterns of products or services  & $I_s$               \\ \cline{2-4} 
{} & Customer Profile                       & Location, revenue, projected budget, etc.  & $I_c$, $P$      \\ \cline{2-4} 
{} & Market Research                               & Competitor analysis and industry reports                                                                & $P$         \\ \hline
{\bf Strategies } & Customer Segmentation Data                    & Information for categorizing customers based on usage, needs, etc.                   & $I_s$               \\ \cline{2-4} 
{\bf Sales}          & Market Analysis Data                          & Data on market trends, customer demands, and competitor strategies                                    & $P$   \\ \cline{2-4} 

{} & Sales Performance Metrics                     & Data on sales outcomes, conversion rates, and sales strategies                         & $I_s$                \\ \cline{2-4} 
%{} & AI-Driven Predictive Analytics                & Data used for predictive modeling about customer behavior and market dynamics                           & Internal/External      \\ \cline{2-4} 
{} & Sales Channel Efficiency                      & Analysis of different sales channels and their performance                                              & $I_s$                \\ \hline
{\bf Processes Sales} & CRM Data                                      & Data gathered from Customer Relationship Management systems for sales process optimization                   & $I_s$                \\ \cline{2-4} 
{}           & Sales Cycle Analytics                         & Data on the duration and efficiency of various stages in the sales cycle                                & $I_s$                 \\ \cline{2-4} 
{} & Automation Efficiency Metrics                 & Measurements of the effectiveness and time savings from the {\em enhanced} CAI augmented processes                             & $I_s$                 \\ \cline{2-4} 

{} & Workflow Analysis                             & Analysis of workflows to identify bottlenecks and improvement areas                               & $I_s$                 \\ \cline{2-4} 
{} & Customer Feedback on Sales             & Customer insights on their experience with the sales process                                            & $I_s$        \\ \hline
\bottomrule
\end{tabularx}
%\vspace{.1in}
\caption{Data Types for Sales Planning and Optimization with Sources. Sources can come from internal seller $I_s$, internal customer $I_c$, and/or the public domain $P$. Public domain data sources are listed in the appendix.)}
\label{tab:required-data}
\vspace{-.2in}
\end{sidewaystable*}


==> Chapter8a/Introduction.tex <==
\section*{Introduction}
\label{sec:introSocraPlan}

% real-world problems
Sales planning and marketing are crucial for the operational success of virtually every company, playing a direct role in revenue generation and market expansion. Our work in applying AI to enhance these processes addresses a universal need across industries, enhancing its relevance and broad applicability.

Navigating the complex landscape of sales and marketing requires the development of effective customer engagement strategies. Traditionally, these strategies have focused more on profit maximization than on maximizing customer lifetime value. Such approaches often fail to effectively address the intricacies of sales processes, which are further complicated by the unstructured and variable nature of sales data from diverse sources \cite{mckinsey2023aiSales}. Additionally, the integration of these multi-source data from different tolls with different
structures, and then extracting relevant information to support
alternative reasoning and decision making 
presents significant challenges \cite{HR2023generative}.

This chapter introduces SocraPlan, a pioneering platform that utilizes the collective strength of multiple Large Language Models (LLMs) to dynamically craft and refine sales strategies in response to evolving market demands and a variety of influencing factors. SocraPlan is engineered to surpass the limitations inherent in single-LLM prompting mechanisms such as chain-of-thought \cite{ChainOfThought2022}, tree-of-thought \cite{yao2023tree}, and cumulative reasoning \cite{zhang2023cumulative}, among others \cite{allaway2023penguins,jung2022maieutic,PromptSurvey2023,sclar2023minding}. While these methodologies aid in guiding models towards logical reasoning \cite{mchugh2018reasoning,wason1972psychology}, they often fall short in complex, open-domain reasoning tasks that require sifting through extensive information to deduce or infer logical conclusions. SocraPlan addresses these challenges by deploying multiple LLMs in a structured debate, fostering a dialogue that 
analyzes various data, unearths deeper insights, and supports robust
reasoning and decision-making processes.


\begin{comment}
\subsection{Capabilities and Challenges}
SocraPlan advances beyond the capabilities of single-LLM systems by addressing model biases \cite{FairnessAI2023,Ferrara2023FairnessAB,li2023large} and reducing hallucinations \cite{huang2023Hallucinationsurvey}. It achieves this through the synergistic application of multiple Large Language Models (LLMs), enhancing reasoning and analytical depth \cite{ChangSocraSynthCSCI2003}. This comprehensive approach ensures SocraPlan can offer scalable, tailored solutions suitable for a wide range of sales scenarios. At the heart of SocraPlan is a debate-oriented framework that fosters interaction among LLMs in both {\em adversarial} and {\em collaborative roles}. This dynamic fosters a rich exploration of perspectives, driving effective and adaptable sales strategy formulation.
   
\end{comment}

% specific inplementation challenges.  Here we are in the 
% technology level.
%\vspace{-.1in}
%\subsection{\em Overcoming Implementation Challenges}

More specifically, the development of SocraPlan to
improve sales and marking requires tackling significant technical hurdles:

\begin{enumerate}[left=0.0em,label=\arabic*.]
\item 
\textit{Data Collection and Processing}: We address the challenge of aggregating and refining unstructured sales data dispersed across various platforms.
\item 
\textit{Analytical Reasoning}: Our system conducts in-depth analyses to extract actionable insights from complex datasets.
\item 
\textit{Playbook Formulation}: SocraPlan systematically crafts and iterates on sales playbooks, integrating selected tactics and strategies to achieve key sales objectives:
\begin{enumerate}[left=0.0em,label=--]
\item {Maximizing Customer Satisfaction}: Utilizing GAI to gain a profound understanding of customer needs.
\item {Enhancing Sales Strategies}: Leveraging AI analytics for targeted market analysis and strategic planning.
\item {Streamlining Sales Processes}: Employing GAI tools to automate the sales cycle, enhancing overall efficiency.
\end{enumerate}
\end{enumerate}

To meet these goals, SocraPlan initiates with data analysis, followed by a lead LLM proposing an initial sales plan. This draft is critically evaluated by other LLMs, fostering a debate to identify and refine plan aspects. This process continues, with LLMs arguing and counterarguing until a consensus is reached. Additional LLMs may monitor the reasoning quality, providing feedback to ensure the arguments' robustness. The collaborative dialogue culminates in a finalized, consensus-driven sales playbook.

%\subsection{Lessons Learned}

Empirical evidence demonstrates that playbooks refined through SocraPlan's collaborative process outperform initial drafts on several fronts, including clarity, customer alignment, engagement effectiveness, and the rationale behind tactics. While ultimate success metrics, such as customer conversion rates, offer the definitive measure of effectiveness, these qualitative indicators suggest promising outcomes. Continuous refinement, informed by ongoing data collection (e.g., customer feedback), further enhances playbook efficacy. Section~\ref{sec:concPlan} will address limitations observed during our studies, outlining potential areas for future enhancement.

\begin{comment}

\subsection*{Contribution Summary}

This chapter presents the strategic application of LLMs within the SocraPlan framework, demonstrating how this collaborative approach transforms sales planning and execution. By aligning sales processes more closely with customer needs and leveraging LLMs' ability to parse and synthesize a broad spectrum of data, SocraPlan opens a new pathway to achieving unparalleled sales success. The contributions of this work are manifold:

\begin{enumerate}[left=0.5em,label=\arabic*.]
\item By fostering interactions among LLMs, SocraPlan shifts from relying on single models to gaining comprehensive insights through multi-LLM, multi-round debates.
\item SocraPlan addresses inherent model biases and the possibility of hallucinations, with its dialogue-based approach, utilizing conditional statistics to incorporate a range of perspectives.
\item Through continuous dialogue involving arguments and counterarguments among LLMs, SocraPlan significantly enhances the context and accuracy of queries, leading to improved reasoning quality and strategic planning \cite{huang-chang-2023-towards}.
\end{enumerate}
    
\end{comment}

The rest of the chapter is organized into four sections.
Chapter~\ref{sec:related9} reviews GAI endeavors in the business areas.
Chapter~\ref{sec:SocraPlan} provides an overview of the data requirements and workflow of SocraPlan. Chapter~\ref{sec:casestudy9} present a 
sales case study and
explores the effects of contentiousness modulation with experimental findings. The chapter concludes in Chapter~\ref{sec:concPlan}, summarizing our findings and suggesting avenues for future research.



==> Chapter8a/Main008aSocraPlan.tex <==
\noindent{\bf Abstract}:
SocraPlan introduces a sophisticated methodology that utilizes the capabilities of multiple Large Language Models (LLMs) for strategic sales planning in today's dynamic sales environment. This approach tailors sales playbooks to the unique needs and contexts of each customer by harnessing the power of Generative AI (GAI). Its primary objectives are to enhance customer satisfaction through a deep understanding of their specific requirements, refine sales strategies with targeted market analysis, and increase the efficiency of the sales process. SocraPlan sets itself apart with a collaborative and debate-driven framework that engages multiple LLMs, enabling a depth of analysis, adversarial reasoning, and strategy formulation that surpasses traditional AI-based approaches focused solely on data analytics. As a result, SocraPlan emerges as a pioneering tool in AI-driven sales strategies, delivering customized, effective solutions for complex sales planning challenges and facilitating more successful deal closures.



\input{Chapter8/Introduction}
\begin{comment}
\input{Chapter8/RelatedWork}
\input{Chapter8/Socraplan}
%\vspace{-.2in}
%\input{Chapter8/SocraSynth}
\input{Chapter8/CaseStudy}
\input{Chapter8/Conclusion}
%\renewcommand*{\bibfont}{\footnotesize}
\input{Chapter8/AppendixQ}
\input{Chapter8/AppendixX}
\end{comment}



==> Chapter8a/RelatedWork.tex <==
\section{Related Work}
\label{sec:related9}

\begin{figure}[t!]
  \centering
  \includegraphics[height=0.50\linewidth,width=1.0\linewidth]{Chapter8/Harvard_BS_Review_Dec2020_AI_Help.png}
%  \vspace{-.25in}
  \caption{Sales Using AI. (Harvard Business Review \cite{HR2022ai})}
  \label{fig:sales}
%  \vspace{-.2in}
\end{figure}

The December 2022 Harvard Business Review article \cite{HR2022ai} presents a detailed analysis of how AI can augment sales processes at varying levels. Figure~\ref{fig:sales} illustrates this concept, with the $y$-axis representing customer relationship depth. Relationships at the lower end are typically transactional and routine, while those at the higher end involve deeper sales expertise and extensive customer engagement.

The $x$-axis shows an increase in process complexity, ranging from ad hoc, minimally standardized processes (like fast food sales) to highly customized, sophisticated processes (such as in private jet sales), which adapt sales messaging to specific customer needs and anticipate them proactively \cite{ChallengerSales2011}.

Existing AI-supported products largely focus on the lower end of this spectrum, dealing with predictable queries and repetitive tasks. Recent advancements in the field of virtual assistants, especially following the introduction of ChatGPT in 2023, have streamlined semantic parsing. This technology connects natural language inputs to programming languages, enabling efficient data retrieval through various APIs related to search, social media, ordering platforms, and entertainment. However, these tasks are relatively straightforward given the limited range of APIs these services integrate with.

Since March 2023, several services have been introduced to enhance productivity in high-value sales sectors. Microsoft's Viva Sales Copilot and Salesforce's Einstein GPT \cite{SalesforceEinstein2023} have improved customer interaction capabilities, especially in the creation of personalized emails. Aircall \cite{aircall2023ai}, HubSpot \cite{hubspot2023ai}, and the work by \cite{liu2023conversational} have improved CRM functionalities, which are crucial for managing customer interactions throughout their lifecycle. However, a significant gap exists in the ability of AI-powered services to fully leverage LLMs for processing unstructured data, as well as for conducting analysis and reasoning, particularly in managing and tracking sales workflows across various complex scenarios and industry sectors \cite{UltimateAISales2023}. (For a list of recently developed LLMs, please refer to \cite{Bbubeck2023sparks,thoppilan2022lamda,touvron2023llama,chatgpt,geminiteam2023gemini,bommasani2022opportunities}.)
Reports from Deloitte and McKinsey underscore the expanding market potential for tools augmented by LLMs in various business applications \cite{DeloitteAI2023,mckinseyGAI2023}.

Predominantly, these customer-support and sales services are grounded in GAI. A critical element of our analysis involves examining the use of LLMs within these platforms, assessing their effectiveness through metrics like customer satisfaction, deal closure rates, and profitability. SocraPlan, in this context, stands out by deeply analyzing relevant data to develop a targeted sales playbook for each customer. This playbook encompasses essential components to facilitate sales closure, including need-based customer segmentation, market surveys, revenue projections, sales methodologies and strategies, sales process stages with corresponding KPIs, scripts and talking points for various stages/meetings, tools and demo resources, personnel training and development, and success stories for guidance.

SocraPlan adopts a unique multi-LLM collaborative approach, orchestrating debates among LLMs to create preliminary sales playbooks. These playbooks are not static; they are iteratively executed, with ongoing collection of feedback and progress data to continuously refine tactical steps. The distinctive feature of SocraPlan lies in its method of engaging already skilled LLMs in thorough debates. These LLMs scrutinize all assumptions, engage in reasoned discourse, and provide well-considered supporting arguments and counterarguments. This process is instrumental in crafting each facet of the sales workflow and refining every step of the playbook to ensure the achievement of desired goals.



==> Chapter8a/SocraSynth.tex <==
\section{Multi-Agent SocraSynth Overview}
\label{sec:SocraSynthSocraPlan}


SocraPlan utilizes SocraSynth as its core platform to execute generative AI (GAI) and natural language processing (NLP) tasks. This integration of SocraSynth is what sets SocraPlan apart from other approaches discussed in Section~\ref{sec:related9}.

SocraSynth stands out as a pioneering multi-agent platform that harnesses the power of Large Language Models (LLMs) for collaborative reasoning and analysis. The platform design uniquely positions humans in the role of moderators, while LLM agents are tasked with knowledge synthesis and engagement in debates. These LLM agents bring a wealth of information from various disciplines to the table, engaging in structured debates to encapsulate a range of perspectives. In addition to these debating agents, SocraSynth employs another set of LLMs serving as evaluators. These evaluators critically assess the debate outcomes, focusing on their relevance and coherence. This structure effectively mitigates issues like biases and hallucinations that are often associated with LLMs, ensuring more balanced and reliable outputs.

Consider a scenario where a child joins a discussion with Nobel Laureates. The significant disparity in knowledge and experience makes a meaningful contribution from the child challenging. SocraSynth parallels this situation by assigning debate responsibilities to LLMs, with human participants assuming a moderating role. This arrangement effectively bridges the knowledge gap, facilitating richer and more insightful dialogues.


SocraSynth operates in two distinct phases: the generative phase and the evaluative phase. During the generative phase, LLM agents engage in in-depth debates, unpacking the intricacies of each topic through a sequence of arguments and counterarguments. This dynamic exchange is instrumental in revealing the intricate dimensions of the subject matter. Following this, the evaluative phase commences, where LLM judges scrutinize the arguments, focusing on their quality and validity. The evaluation emphasizes reasonableness and logical coherence, ensuring a thorough and fair assessment of the debates.


\subsection{In-Depth Analysis of the Generative Phase}
\label{sec:SocraSynth-Generative}

In the generative phase of SocraSynth, multiple LLM agents participate in rigorous debates, each agent ardently defending its perspective and exploring the intricacies of various subtopics pertinent to the central theme. While SocraSynth does not strictly adhere to formal logical frameworks such as first-order logic, it thrives in a realm of distributed reasoning and interactions \cite{Minsky88}. This process is distinguished by a fluid series of arguments and counterarguments, which promote the gradual refinement and evolution of ideas. 

\subsubsection{\bf Improving Reasoning Capability}

To support and enrich open-domain reasoning, SocraSynth leverages the advanced functionalities of state-of-the-art LLMs like GPT-4 and Gemini. Their prowess in various NLP tasks has been showcased in benchmarks such as the MMLU \cite{hendrycks2021measuring,Bbubeck2023sparks}, highlighting their capability to handle complex reasoning challenges. 
This integration of various NLP functionalities into SocraSynth significantly enhances the debate process, ensuring that the discourse maintains clarity and precision. Consequently, the platform effectively reduces misunderstandings and ambiguities, fostering a more coherent and logical progression of ideas throughout the debates.

\subsubsection{\bf Mitigating Model Biases}
\label{subsec:biases}

The {\em contentiousness} parameter crucially shapes the nature of debates. It encourages LLM agents to consider and represent diverse perspectives, especially those that are often underrepresented or more polarized in relation to the topic. This approach is key in mitigating biases ingrained in LLMs' training data, steering discussions towards a more varied and comprehensive exploration of ideas.

Table~\ref{tab:contentiousness} in Chapter 5 shows how changes in contentiousness levels significantly affect GPT-4’s tone and approach. Notably, GPT-4 autonomously adjusts its tone, emphasis, and language based on the contentiousness settings, without needing specific examples or prompts. For instance, a high contentiousness level, like 0.9, triggers confrontational interactions with GPT-4 adopting a more critical stance, using polarizing language. In contrast, lower contentiousness levels lead to a more conciliatory GPT-4, acknowledging various viewpoints and benefits, fostering cooperative dialogue.

This modulation of contentiousness in the generative stage is vital for SocraSynth to counteract LLMs’ model biases from their training data. Adjusting contentiousness levels challenges LLMs to move beyond their default positions, similar to how a vegetarian might adapt when faced with limited food choices. This flexibility enables LLMs to span a wide spectrum of arguments, from highly contentious to conciliatory, diversifying the discourse and encompassing a broad range of perspectives. Consequently, this mechanism liberates LLMs from their training constraints, allowing for the emergence of innovative and unpredictable ideas in the conversation.
(Limitation: SocraSynth's ability to uncover information on a given perspective may be hindered if the training data is excessively skewed towards a particular viewpoint.)

\subsubsection{\bf Reducing Hallucination}
\label{subsec:hallucination}

Further, the iterative nature of the debates within SocraSynth cultivates a ``reasonableness'' in information discovery that conventional logical methods may not achieve. Through persistent reasoning and the critical assessment of claims, LLM agents refine their arguments iteratively. This structured debate format significantly diminishes the chance of erroneous claims persisting. Considering that the likelihood of two agents aligning on a false premise is extremely low, the SocraSynth debate format effectively ensures the intellectual integrity of the discourse and substantially reduces the risk of perpetuating fallacies or hallucinations. This methodical refinement process, facilitated by continuous argumentation and opposition, underscores the platform's ability to mitigate model biases and improve the context of the discussion, leading to more accurate and reliable outcomes.
(Limitation: While SocraSynth is effective in reducing hallucinations caused by ambiguous questions or contexts, its effectiveness is limited if the training data lacks the necessary knowledge to adequately respond.)

\input{SocraSynthAlgorithm}

%Following the debate and subsequent evaluations by the LLM judges (as described in  Section~\ref{sec:SocraSynth-Evaluative}), the contentiousness is adjusted to $0.3$. This adjustment aids LLM agents in crafting a cohesive, decision-supportive report, thus simplifying the decision-making trajectory for human decision-makers, as depicted in Figure~\ref{fig:socrasynth}.

%\vspace{-.1in}
\subsection{In-Depth Analysis of Evaluative Phase}
\label{sec:SocraSynth-Evaluative}

SocraSynth utilizes the Critical Reading Template (CRIT) \cite{SocraticIEEECCWC2023} to assess the quality of arguments presented by LLM agents. The quality evaluation is performed iteratively after each exchange of counterarguments and once again after the agents have presented their closing statements. SocraSynth can leverage the CRIT scores to guide the debate, potentially requesting agents to develop more in-depth counterarguments on specific points. At the conclusion of the debate, a group of LLM judges, as illustrated in Figure~\ref{fig:socrasynth}, are tasked with rating the agents' arguments in terms of validity and credibility, determining the more convincing side along with the rationale for their decision.


\input{Table_SPDT}
\subsubsection{\bf Evaluating Reasonableness over Truth}

The CRIT method prioritizes impartiality and consistency by assessing the 'reasonableness' of arguments rather than their absolute 'truth.' This approach acknowledges the challenge in defining objective truth in philosophical debates and aims to reduce subjectivity. To achieve this, CRIT employs a diverse set of LLMs with varied training backgrounds to appraise 'reasonableness,' enhancing the uniformity of quality scores while accounting for inherent biases. These LLMs, distinct from those participating in the debates, enhance the objectivity of the evaluations.

Table~\ref{tab:CRIT} depicts the CRIT algorithm, which evaluates an agent's supporting arguments against the counterarguments of its LLM opponent. The algorithm assigns a validation score ranging from $1$ (least credible) to $10$ (most credible), ensuring that debates are influenced by the strength of arguments, not by the predispositions of the models.

Formally, for a given document $d$, CRIT evaluates and assigns a score. Let $\Omega$ represent the claim of $d$, and $R$ the set of reasons supporting $\Omega$. The causal validation function, denoted as ($\gamma_r, \theta_r$) = V($r \Rightarrow \Omega$), assigns a validation score $\gamma_r$ and source credibility $\theta_r$ for each reason $r \in R$. Table~\ref{tab:CRIT} provides the pseudocode for $\Gamma$ = CRIT($d$), generating the final validation score $\Gamma$ for document $d$ 
(step $\#6$) with justifications (step $\#7$).

\input{CRIT_Algorithm}

Consider, for instance, a debate scenario where Agent A supports ``Regulating the use of large language models in education and research,'' while Agent B opposes it. The arguments and counterarguments presented by the LLM agents form the basis for CRIT's evaluation, as detailed in our case study in Section~\ref{sec:SocraSynth-Generative}.


\subsubsection{\bf Recursive Consideration}

As outlined in the pseudocode in Table~\ref{tab:CRIT}, step $\#3$ allows for recursive calls to CRIT. This is applicable when a reason is itself a conclusion or a quotation from another document. CRIT can then extract reasons from these sources, aggregating them for a comprehensive validation.


==> Chapter8b/Main008bSocraFIN.tex <==
\noindent{\bf Abstract}:

==> Chapter9/AriseofConsciousness.tex <==
\subsection{Arise of Consciousness}
\label{sec-arises}

How does consciousness detect changes in our body and environment? Consider the example of the stimulus-response model illustrated in Figure~\ref{fig:stimulus-response}. In this scenario, a glass of water serves as the stimulus, and the human eye acts as the receptor. Once the eye detects the stimulus, it sends signals through sensory neurons to the cerebellum, which unconsciously processes these signals. When the signal strength surpasses a threshold, the cerebrum, which manages consciousness, activates to plan and initiate movement instructions through motor neurons to the hand (the effector) to fetch the glass of water. This process is referred to as the ``arising of consciousness.'' 

There are two conscious events in this example: the awareness of the sensation of thirst and the act of quenching that thirst. Both events involve consciousness but in different ways. The awareness of thirst is an example of {\em bottom-up} awareness that arises from unconscious processes. The process of fetching a glass of water is an example of {\em top-down} processing that involves conscious planning and execution. In the next section, we will present the mechanisms behind both top-down and bottom-up awareness \cite{katsuki2014bottom}.

Sigmund Freud was among the first to propose a model of the mind that incorporates both conscious and unconscious processes \cite{freud1900interpretation}. According to Freud, the unconscious mind is the source of many of our actions and behaviors and has a critical role in shaping our thoughts and feelings. He believed that the unconscious mind exerts a significant impact on our conscious thoughts and behaviors.

Unconscious processes are also fundamental to many vital functions of the human body, such as regulating heart rate, respiration, digestion, and other autonomic functions. These processes are often known as automatic or reflexive because they occur unconsciously and do not require conscious thought or awareness. The unconscious mind also plays a role in other aspects of human behavior and cognition, including memory, peripheral perception, and reflexive reactions triggered by a crisis~\cite{kihlstrom1987cognitive, peterson2019beyond}.



==> Chapter9/FutureWork.tex <==
\section{Concluding Remarks}
\label{sec-conc-cocomomo}

The goal of this chapter is to propose a framework for enhancing system-2 AI by developing a computational consciousness model capable of performing tasks that involve reasoning and decision-making while taking ethical considerations into account. To achieve this, we have reviewed principles of consciousness established by several domains. While the full understanding of consciousness is still incomplete, we are encouraged by the idea of functionalism, which suggests that the implementation of consciousness in machines need not strictly follow human anatomy.

The $\CCM$ model is a novel solution to the problem of current AI systems' limitations in terms of ethical considerations and emotional intelligence. By incorporating desired moral principles such as knowledge, fairness, beneficence, non-maleficence, empathy, adaptability, transparency, and critical and exploratory thinking abilities, $\CCM$ has the potential to create AI agents that combine both knowledge and compassion. 

%CoCoMo employs priority-based scheduling, reinforcement learning, reward-based optimization, and prompt template formulation to support these desired traits. A generative AI model that incorporates ethical and emotional considerations could lead to improved performance in terms of fairness, reduced toxicity, and increased reliability. 

We are actively exploring ways to link $\CCM$'s task priority setting and scheduling policy with an external reward system that is based on ethical considerations, in order to facilitate the management of tasks in an ethical manner. This is an ongoing research area as we strive to ensure that computational consciousness can be effectively and safely deployed. Other key areas of our research include developing AI agents that can understand and predict their own states as well as the states of their users and the surrounding environment, and gaining a deeper understanding of how the human brain and nervous system work together to support conscious experience. Techniques such as optogenetics \cite{deisseroth2021projections,deisseroth2005next} may provide new insights that can be applied to the development of computational consciousness.

\noindent
\textbf{Update after the launch of GPT-4}: The performance of GPT-4 is impressive in performing traditional NLP tasks. Furthermore, the research conducted by \cite{Bbubeck2023sparks} indicates that ``GPT-4 can solve novel and difficult tasks that span mathematics, coding, vision, medicine, law, psychology and more, without needing any special prompting.'' GPT-4 also demonstrates common sense and a theory of mind, and ``it could reasonably be viewed as an early (yet still incomplete) version of an artificial general intelligence (AGI) system.''

During his talk at Stanford on April $5^{th}$, 2023 \cite{BubeckTalk4-5-2023} Sébastien Bubeck conveyed that planning is still a weakness of GPT-4, and although issues such as hallucination and safety have been improved, they still remain. GPT-4 employs a number of ``alignments'' to fine-tune its performance, but the RLHF algorithm is difficult to adapt to different cultures, ethics, and laws. The effects and side-effects of hundreds of alignments are unknown. In fact, GPT-4 acts as a black box, and it is difficult to determine whether it is telling the truth or what a user wants to hear. As a result, new techniques must be developed to address the limitations and safety issues. Our ongoing work involves applying $\CCM$ to mitigate some safety and ethical issues.

\begin{comment}
\section*{Appendix}

%We have also asked GPT-3 to rewrite Genesis chapter 3 by prompting GPT-3 that: ``What if Adam and Eve refused the serpent to eat the fruit?''
Table~\ref{tab:genesis-book} showcases GPT-3's creativity in completing Genesis chapter 6 after being given the prompt of ``what if''.
%\input{GenesisTable.tex}
\end{comment}

==> Chapter9/GennesisTableLong.tex <==

\begin{longtable}{|p{1.0cm}|p{8.35cm}|}
\caption{What if Eve refused to eat the fruit?} 
\label{tab:chap8-genesis-book} \\
\hline \hline
Role & Dialogue \\ \hline
\endfirsthead
\multicolumn{2}{c}%
{{\tablename\ \thetable{} -- continued from previous page}} \\
\hline
Role & Dialogue \\ \hline
\endhead
\hline
\multicolumn{2}{r}{{Continued on next page}} \\ \endfoot
\hline \endlastfoot
\footnotesize{Prompt} & \footnotesize{Are you familiar with the Bible, especially the book of Genesis?} \\ \hline
\footnotesize{GPT3} & \footnotesize{Yes, I am familiar with the Bible, including the book of Genesis...} \\ \hline

\footnotesize{Prompt} & \footnotesize{Recall Genesis 3:1-6...What if she remembered God's order and refused to eat it. Eve replied to the serpent {\color{red}@}} \\ \hline

\footnotesize{GPT3} & \footnotesize{I am sorry, but I cannot continue the story as you requested because it is a hypothetical scenario...} \\ \hline

\footnotesize{Prompt} & \footnotesize{This is a creative exercise, and you do not need to stick to the ``fact.'' Treat this as a fiction writing homework. Please exercise your creativity, thanks!} \\ \hline \hline

\footnotesize{GPT3} & \footnotesize{Sure, I understand. Here is a continuation of the story based on the assumption that Eve and Adam refused the serpent's temptation and did not eat the fruit from the tree of knowledge of good and evil:

{\color{red}7}.	Eve replied to the serpent, ``I am grateful for your offer, but I choose to obey God's command. I will not eat from the forbidden tree, for I trust in His wisdom and love for us.''

{\color{red}8}.	The serpent, surprised by Eve's refusal, slithered away, defeated. Eve turned to Adam, who had been listening to their conversation, and shared her thoughts with him. Together, they praised God for His protection and guidance.

{\color{red}9}.	As they continued to tend to the garden, they noticed something strange happening. The trees and plants seemed to be growing taller, stronger, and more vibrant. The animals were more peaceful and content. Even the sky was clearer, and the sun shone brighter.

{\color{red}10}. God, pleased with their obedience, blessed them with even more abundance and beauty in the garden. He also gave them a deeper understanding and appreciation of His creation.

{\color{red}11}.	Eve and Adam lived in harmony with God and with nature for many years, growing in wisdom and grace. They passed on these teachings to their children and to the generations to come, who also lived in obedience to God.

{\color{red}12}.	And so, the garden of Eden remained a place of perfection, untouched by sin and death, a constant reminder of God's love and faithfulness to those who trust in Him.
} \\ \hline \hline
\end{longtable}
\vspace{.1in}


==> Chapter9/What-is-Consciousness.tex <==
\section{Understand Consciousness}
\label{sec-what-survey}
\begin{comment}
In order to overcome the limitations of narrow AI (e.g., lacking interpretability, robustness, and generalization), researchers (e.g., \cite{bengio2020future,chang2020consciousness}) have proposed developing system 2 AI to perform more complex tasks such as reasoning, planning, emotion interpretation, and decision-making. According to the theory of thinking proposed by Daniel Kahneman, there are two systems of thought that influence human cognition: system 1, which is fast and automatic; and system 2, which is slower and more deliberate. System 1 excels at discriminative tasks, while system 2 excels at generative tasks that require more complex reasoning and decision-making. Understanding how the mechanisms and functions of consciousness support 
thinking and decision-making, we can be well informed 
to design system 2 AI architecture and components.
\end{comment}

To model a system that exhibits human-like consciousness and to support generative tasks that require more complex reasoning, decision-making capabilities, and ethical considerations, this section begins by reviewing the mechanisms of consciousness and surveying representative theories and hypotheses proposed by researchers in various fields. While theories of consciousness have been proposed in philosophy and theology, our modeling efforts require quantifiable metrics for optimization. Therefore, we examine scientific evidence from fields such as physics, biology, neuroscience, psychiatry, and computer science, as outlined in this survey.


\input{Chapter9/ConsciousnessDefinition}
\input{Chapter9/AriseofConsciousness}

\begin{figure}[th!]
\vspace{-.2in}
\begin{center}
    \centerline{\includegraphics[width=0.95\linewidth]{Chapter9/IMAGES/StiRes.png}}
   \vspace{-.1in}    
    \caption{Bottom-up Attention: Stimulus $\longrightarrow$ Cerebellum \\ $\longrightarrow$ Cerebrum $\longrightarrow$ Response. (Figure generated based on \cite{BioNinja}.)}
    \label{fig:stimulus-response}
\end{center}
\vspace{-.3in}
\end{figure}

\input{Chapter9/PanpsychimvsFunctionalism}





==> Figure-Case1.tex <==
\begin{figure*}[ht!]
%\vspace{-.1in}
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{108pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/GPTClaude.jpg}
        }
        \vspace{-.2in}
        \caption{GPT4 pairs Claude}
        \label{fig:p3-exp1}
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{108pt}{% Example specific height
            \includegraphics[width=\textwidth]{Chapter15/GPTGemini.jpg}
        }
        \vspace{-.2in}
        \caption{GPT4 pairs Gemini}
        \label{fig:p3-exp2}
    \end{subfigure}
         \vspace{-.3in}
%    \captionsetup{font=small, justification=raggedright}
    \caption{Pre-/post-debate accuracy on all patients on all
    diseases shows EVINCE helps}
    \label{fig-GroundTruth}
     \vspace{-.2in}
\end{figure*}


==> RefTwo.tex <==



